AI-Driven Research for Databases

As the complexity of modern workloads and hardware increasingly outpaces human research and engineering capacity, existing methods for database performance optimization struggle to keep pace. To address this gap, a new class of techniques, termed AI-Driven Research for Systems (ADRS), uses large language models to automate solution discovery. This approach shifts optimization from manual system design to automated code generation. The key obstacle, however, in applying ADRS is the evaluation pipeline. Since these frameworks rapidly generate hundreds of candidates without human supervision, they depend on fast and accurate feedback from evaluators to converge on effective solutions. Building such evaluators is especially difficult for complex database systems. To enable the practical application of ADRS in this domain, we propose automating the design of evaluators by co-evolving them with the solutions. We demonstrate the effectiveness of this approach through three case studies optimizing buffer management, query rewriting, and index selection. Our automated evaluators enable the discovery of novel algorithms that outperform state-of-the-art baselines (e.g., a deterministic query rewrite policy that achieves up to 6.8x lower latency), demonstrating that addressing the evaluation bottleneck unlocks the potential of ADRS to generate highly optimized, deployable code for next-generation data systems.

==> figures/1.5-intro.tex <==
different optimization problems have different evaluation
challenges (e.g., simulation may be need for optimizing a system component but evolve in full system in another case), the techniques we apply are 
we illustrate how to use AI to  we apply it across three ``classic'' database problems, co-evolving the evaluation process alongside the candidate solutions.

\accheng{specificity is confusing
need to do something different for every approach?

we are looking at the space of cost-reductive techniques. it is spanned by these potential optimization techniques. we are looking at applying ADRS to these techniques to do things we might not be able to do otherwise

3 different things seem to disparate

theme of techniques is unclear
lacking structural guidance to tie these techniques together

can we add a Fig 1? what differs with AI-driven stuff vs. AI in the name?
Ex: chat bot solved the last mile problem of being in natural language
Is there something about ADRS that enables us to make search space smaller and evaluation faster that was not possible before?

Why now? big problem
Here are the taxonomy of solutions

Previous ad-hoc manual approach
Maybe separate tiers: no AI, ADRS for solution, ADRS for evaluator

Be very clear that there has been work on other parts of ADRS, evaluator is currently manual
Our big step is that we we are addressing the evaluator problem
And it is particularly challenging for databases
}

[For entire paragraph: Be very clear Our big step is that we we are addressing the evaluator problem
we are applying ADRS to evaluator techniques listed before 
Make sure we answer this implicitly: Is there something about ADRS that enables us to make search space smaller and evaluation faster that was not possible before?
we are looking at applying ADRS to these techniques to do things we might not be able to do otherwise
since different problems need different techniques, we look at three ``classic'' database problems 
make read better and flow better
]
In this paper, we illustrate how to use AI to design effective evolution techniques to address these various challenges. Specifically, we consider three ``classic'' database problems and \textit{co-evolve} their evaluation process alongside the candidate solutions.
In the buffer manager, we co-evolve the \textit{simulator} to automatically discover a caching algorithm that outperforms the SOTA. For index selection, we co-evolve our \textit{model of end-to-end behavior} to discover a new algorithm that enables both better cost estimation and latency (30\% improvement) compared to existing methods. For query rewrites, we co-evolve the \textit{subset of workloads and search techniques} to generate a novel, deterministic policy that results in [2.0$\times$] lower latency and runs in over four orders of magnitude faster (<200ms vs. 80 minutes) than the SOTA approach, which makes LLM calls per query. Beyond raw performance, these results highlight the practical advantage of evolving white-box code: the discovered solutions are interpretable, predictable, and deployable without specialized inference infrastructure.

\accheng{evaluation is problem
what is solution?
for different problems, you have different techniques
}

While standard techniques exist to mitigate evaluation and search costs, each introduces significant trade-offs and requires considerable manual effort. (1) One method is to employ simulators~\cite{}, but constructing high-fidelity models of complex database internals is notoriously difficult and time-consuming. Low-fidelity alternatives risk misleading the optimization process, requiring careful manual tuning to ensure validity. (2) Another approach is to model end-to-end performance (e.g., via learned cost models~\cite{}), but this requires significant effort in feature engineering and data collection. (3) Evaluation can also be accelerated by running only a subset of workloads~\cite{}, but manually selecting representative queries is challenging and risks overfitting, which limits the solution's applicability. (4) Finally, limiting the search space to a subset of optimization techniques can reduce the number of iterations needed but requires expert analysis to ensure critical opportunities are not excluded~\cite{}. \ion{(1) The evaluation is hard. (2)Why is the evaluation harder in the case of DBSs vs other systems? (3) There are different techniques to reduce the evaluation cost but they are problem specific. (4) We illustrate how to design efficient evaluations by considering three "classic"problems in databases.}

\accheng{don't emphasize trade-offs because would expect me to mention how to navigate

Just say there are different techniques to apply and different effectiveness for different problems
We illustrate how to use AI to design effective evolution techniques
}

\accheng{need to set the stage for the following:
different tradeoffs for different problems
given a problem, how to identify these tradeoffs

need to setup the problem
}

\accheng{(2) why evaluation is hard?
need to make why clear this is a DB thing
not super clear what is difference with DB that you can't do with ADRS and OE already
cross-component coupling, database cost model (noisy signal, can we say something about input for cost model is helpful?), playing up simulator, workload dependent}

In this paper, we demonstrate how we can automate these evaluation techniques to effectively apply ADRS to a range of database performance problems. Our key insight is to \textit{co-evolve} the evaluation process alongside the solutions. Rather than treating evaluation components as static artifacts, we leverage the evolutionary loop to simultaneously refine simulators, performance models, workload subsets, and the space of optimization strategies. By framing evaluation fidelity as an evolvable objective, we demonstrate how to effectively apply ADRS to complex database systems.

\accheng{too much setup, not enough insight
need to address what we setup in detail}

% the immense complexity of these systems makes applying this approach challenging. Effective ADRS deployment requires researchers to first address two difficult research stages: (i) \textbf{problem formulation} and (ii) \textbf{evaluation setup}.

% Problem formulation entails defining goals, setting constraints, understanding related work, and providing sufficient context to develop a solution. Optimizing database performance requires specialized knowledge of internal system intricacies, which LLMs often lack this context by default and generating the necessary data may require various exploratory experiments. \accheng{do we just say defining goals is a human effort?}

% Evaluation setup involves providing a target system or simulator, defining performance objectives (such as workloads and metrics), and implementing baselines. In the database context, there are  bottlenecks in securing rapid feedback and selecting appropriate evaluation objectives.
% ADRS frameworks usually must execute many iterations (e.g., tens to hundreds~\cite{}), so the evaluation in each iteration must be \textit{fast} and \textit{accurate}. Direct evaluation on a full database is usually prohibitively expensive, as recompilation, data loading, and benchmark execution take too long for each iteration. To make search feasible, researchers must rely on \textit{simulators}, but this introduces a fundamental trade-off: high-fidelity simulators are difficult to build, while low-fidelity simulators risk guiding the LLM toward invalid optimizations.
% Furthermore, determining the correct metrics and workloads for evaluation is challenging. Running all workloads against end-to-end metrics may be too expensive, yet running a subset with estimation metrics risks overfitting and failing to optimize for the full system.

% In this paper, we demonstrate how to effectively apply ADRS to a range of database performance problems. Our key insight is that we should \textit{co-evolve} the missing pieces in problem formulation and evaluation setup alongside the solutions. Concretely, we leverage the evolutionary loop to not just to discover solutions but also to generate better simulators, context, and evaluation objectives. 
% \textit{By treating problem formulation and evaluation as evolvable problems, we optimize the entire process of applying ADRS to databases.}

% \accheng{Overall insight: evolution processes
% multiple challenges: evolution takes too long, search space too large
% Here's we take three use cases, we are going to address some of these challenges
% Using an outer evolutionary method
% First one: too slow, develop faster than e2e
% Second one: devleop model to do e2e
% third one: subset of tests, guiding the search
% }

\accheng{do we focus only on performance in this paper?}% \accheng{yes we should}

\accheng{don't say heuristics, just say algs}

We demonstrate this approach by applying it to three case studies to demonstrate its potential for this domain. In the buffer manager, we co-evolve the \textit{simulator} to automatically discover a caching algorithm that outperforms the SOTA. For index selection, we co-evolve our \textit{model of end-to-end behavior} to discover a new algorithm that enables both better cost estimation and latency (30\% improvement) compared to existing methods. For query rewrites, we co-evolve the \textit{subset of workloads and search techniques} to generate a novel, deterministic policy that results in [2.0$\times$] lower latency and runs in over four orders of magnitude faster (<200ms vs. 80 minutes) than the SOTA approach, which makes LLM calls per query. Beyond raw performance, these results highlight the practical advantage of evolving white-box code: the discovered solutions are interpretable, predictable, and deployable without specialized inference infrastructure.


% In this paper, we apply ADRS to a variety of database performance problems to demonstrate its potential for this domain. In the buffer manager, we automatically discover a caching algorithm that outperforms the SOTA by X\%. For query rewrites, we evolve a novel, deterministic policy that results in [X.Y$\times$] lower latency and runs in over four orders of magnitude faster (<200ms vs. 80 minutes) than the SOTA approach, which makes LLM calls per query. For index selection, we discover a new algorithm that enables both better cost estimation and latency (X\% improvement) compared to existing methods. \lma{Optional: we've been primarily talking about perf numbers. But if there's space, maybe call back the benefit of white-box optimization again.}

% Despite this promise, applying ADRS to database systems is uniquely challenging because these systems are complex and must satisfy a wide range of operational guarantees. First, databases are \textit{stateful} systems that must uphold a range \textit{correctness guarantees} across state changes while simultaneously optimizing for varied and often conflicting \textit{performance objectives}. \lma{Slightly difficult to parse. Maybe have a one-sentence example.} Formulating the optimization goals by specifying correctness constraints and defining workload-dependent performance goals constitutes a significant challenge in practice. 

% \lma{``Second,''?} Databases have \textit{immense complexity}. These systems comprised of multiple, intricate layers that are usually individually optimized. The interactions between these components create a vast and noisy search space that is difficult to model accurately. For instance, the end-to-end performance of a novel concurrency control protocol arises from its interactions with the transaction manager, logger, and buffer pool. \lma{This makes sense, but we didn't solve this problem. Maybe use a problem we solved as an example. Unless you want to phrase this as future work?} This intricate web of dependencies makes building a fast, high-fidelity evaluation framework a primary obstacle, as simple component-level tests are often insufficient to predict end-to-end system impact.

% \lma{``Third,''?} Evaluation is challenging on databases due to their complexity. Each modification on the full system requires a re-compilation, loading the database state, and execution of benchmarks. This makes each iterative loop too expensive, so the standard solution is to evaluate solutions on a \textit{simulator} to make evaluation feasible. As such, a key challenge in using ADRS is building a fast and high-fidelity simulator. Our approach is to implement a cascade of simulators.

% We present a number of preliminary solutions and insights in applying ADRS to databases. \lma{Do we want to call this "preliminary"? For a full research paper, we might not want to use "preliminary". We could say this is the "first attempt" at XYZ if you want to tone down expectations a bit.} First, to address the challenge of simulation, we propose automatically evolving simulators via ADRS. Crucially, we find that ``more is more'': more baseline implementations and metrics on the full system result in more effective simulator evolution. 

% Second, databases may required domain-specialized data that are not present in LLMs. 
% We propose bridging the context gap by incorporating agents to construct the missing ground truth data (``construct the context you need'') to enable the discovery of high-performance optimizations.

% Finally, we discuss how to ``hone the signal'': successful evolution requires us to carefully select the workload to evolve on. \lma{Seems a bit thin. Add one sentence?}

% However, realizing this potential requires navigating the unique complexities inherent to stateful database architectures. In the rest of the paper, we elaborate on these challenges, outline our proposed solutions, and evaluate the research implications of this new paradigm.

\accheng{rename
before, designed things assuming writing code was bottleneck
now that is not the case

code review is the number one problem now
bottleneck shift: software designed to spend a lot of time generating code and review is much faster
People don't have as much ownership
Now code is cheap, 1\% code generation, 99\% everything else
This shift means that everything else is the bottleneck
Here, the bottleneck is evaluation
Higher fidelity becomes directly relevant to how we can create solutions
}

\accheng{this should just be challenges of ADRS for evaluation specific to database}

\accheng{every technique has tradeoff and tradeoff is tunable
}
Despite the exciting potential of applying ADRS to databases, there are significant hurdles due to the difficulty of end-to-end evaluation. ADRS frameworks are only as effective as the evaluators guiding them, as successful discovery requires fast, accurate, and detailed feedback from the evaluator. However, there is an inherent trade-off between speed and three other critical properties (fidelity, generality, and coverage) that we need.
\textbf{Speed} is key for evaluation, as ADRS frameworks generally need a substantial number of iterations to find good solutions~\cite{}. On the other hand, the evaluator must maintain \textbf{fidelity} by capturing the salient system behaviors for the problem being solved. Moreover, we should have \textbf{generality}: evaluators must support diverse workloads to provide robust feedback signals and prevent overfitting to a single configuration or dataset. Finally, the evaluation should enable sufficient \textbf{coverage} of the search space to avoid missing out on further improvements. Achieving high fidelity, generality, and coverage increases evaluation latency, and balancing these competing objectives is particularly difficult in databases due to their complexity and vast problem spaces.
\accheng{coverage relates to number of iterations rather than faster iterations

end state as a convergence metric

maybe frame as: one other reason the evaluator is slow is because of the search space, here's the technique for that

convergence and fidelity in reasonable time
we want to converge to X result in Y time
generality is form of fidelity
main properties are speed, fidelity, convergence

evaluation is the most important unsolved problem in this space
need to prove this is the problem to solve
these tradeoffs are non-trivial (speed vs. fidelity), this is manual and hard
we can now intelligently navigate this tradeoff with AI
need to prove this is a real problem (can't just run on real system) and our solution is feasible
3-way tradeoff between properties
speed vs. quality of solution tradeoff, mention quality means different things (fidelity, convergence, reality is navigating curve)

now that code is cheap, navigating this non-trivial tradeoff can be cheap
we can optimize/automate something that we could not before
easy to sacrifice convergence
there is direct tradeoff between fidelity and convergence

mention research on solution selector 
}

\accheng{need to make clear what is reasonable time
DBs are not vibe-codeable so longer things 
One week is not inherently prohibitive but we should be clear for evaluation

need to make clear what is the bottleneck and why in minutes rather than days

need to be clearer that the bottleneck is the evaluator so this needs to be fast
before, would not manually run 10-100s of ideas but now you can so different/more pressing challenge to make evaluation faster
}
First, databases have high evaluation costs due to their complex and stateful nature. For example, directly applying an existing ADRS framework to optimize PostgreSQL's buffer replacement policy would require modifying C++ source code, recompiling the database (X mins), loading data for standard benchmarks (e.g., Y mins for TPC-H SF=10), and executing the full workload (e.g., Z mins). A single iteration could take over X+ minutes, making the tens to hundreds of iterations required for convergence prohibitively slow. 
This example shows how database researchers to navigate complex trade-offs between the evaluator properties we need for ADRS frameworks.

Furthermore, search space can be extremely large for database performance problems, complicating coverage. For instance, identifying the optimal set of query rewrite rules is a combinatorial problem. When applying ADRS directly, the framework often becomes ineffective as it wastes resources (e.g., searching through vast numbers of ineffective rule combinations), struggling to identify and focus on the most promising regions of the problem space.

While standard techniques exist to accelerate evaluation, each prioritizes speed at the expense of fidelity, generality, or coverage.
(1) Researchers often employ simulators to avoid expensive full-system evaluation. However, this sacrifices \textbf{fidelity}. Accurately modeling database internals is difficult as complex interactions between different components create a noisy environment that is hard to capture. Low-fidelity models risk guiding the LLM toward invalid optimizations.
(2) Similarly, relying on proxy metrics and using a model to predict end-to-end behavior favors speed over \textbf{fidelity}. Simplified metrics (e.g., cost estimation rather than actual query latency) are easier to measure but often fail to reflect true performance in complex systems.
(3) To improve speed, one can run a subset of workloads. This approach can compromise \textbf{generality}: optimizing for a narrow subset risks overfitting and the loss of signals required for the full system.
(4) Finally, limiting exploration to a subset of optimization techniques can reduce the number of iterations needed in the evolution loop but reduces \textbf{coverage}. This technique requires significant domain expertise to ensure critical opportunities are not discarded.

Navigating the trade-offs introduced by these techniques requires painstaking manual effort and can be as difficult as developing the solutions themselves. To address this, we present our co-evolutionary approach in the next section, which automates parts of the evaluation process to more effectively apply ADRS to databases.

\accheng{how does ADRS relate to prior ML techniques? could combine them in theory

both manual research loop and ML learned technique are bootstrapping pieces for "one ring to rule them all" so we don't have to put down prior work

need to convey hype and urgency: we are at a precipice

the evaluation is the bridge to the land of dreams}

\accheng{
1. more and more complexity, harder workloads, etc. 
research currently takes too long

2. there is shift with LLMs. think about where learned approach comes in: both takes awhile to custom-train a model to tune parameters and also can only tune parameters of existing implementations. use as example to solidfy the two points.
having LLM generate code gives you deeper level of optimization? not feasible for grad students/profs to try out hundreds of algorithms. this kind of capability is not feasible before

3. we believe ADRS is rapidly becoming the norm.
ADRS will eventually become the norm
People need to believe this will be the future to care about this paper

4. bottleneck is evaluation. if we can solve evaluation, we get even more amazing thing than ADRS.

5. evaluation is hard for databases.

6. here are the standard/existing techniques to make eval cheaper. why applying them directly is insufficient. just mention techniques by name, central point is that doing these is as hard as solving problems themselves

7. topic sentence: we address this critical evaluation bottleneck by [more detail than use AI, co-evolution is good but be clear]. we demonstrate using three classic DB problems
ADRS was replacing some pieces with bot loop. we are replacing some more pieces.
use feedback from inner loop to feed outer loop

8. just high level overview of case studies
have section reference to insights

9. reminder about vision
}
The design of high-performance database systems traditionally relies on manual algorithm development, which requires substantial time to adapt to new workloads and hardware.
Recent research integrates machine learning (ML) to automate  performance optimization. However, these methods largely treat the underlying engine as a black box, focusing on knob tuning or replacing components with learned models that perform inference at query time. Consequently, learned approaches remain difficult to deploy~\cite{} due to run-time inference overhead, unpredictable worst-case behavior, and the need for specialized ML infrastructure.

A new class of AI-driven techniques is emerging to address these practical limitations while automating system design. Specifically, Large Language Models (LLMs) are enabling a phase shift toward white-box optimization. Instead of executing models at runtime, these techniques use LLMs to generate optimized code directly. This new approach, termed AI-Driven Research for Systems (ADRS), shows promising results in automated algorithm discovery by finding solutions that match or exceed the performance of state-of-the-art, human-designed algorithms on various systems problems~\cite{} (e.g., 13$\times$ faster load balancing algorithm, 10$\times$ faster code for Datadog). %(e.g., yielding significant performance gains in load balancing algorithms and production monitoring infrastructure).

\accheng{we're explaining what is hard, too much focus on what

instead should focus on north-star what and sell why solving this problem will be important

need to sell ADRS more

we think the future of DB research is ADRS, this is what's blocking that dream

need to layout vision about how DB research will be done in 5/10 years
1. most DB researchers don't know about ADRS
2. people don't know what it will evolve into
b/c people don't understand this dream yet, we should add some of the argument from our other paper

need sense of "upending systems research"
"how fixing evaluation unblocks the future of DB researcher"

needs 1-2 paragraphs restating what we said previously: ADRS will eventually become the norm
People need to believe this will be the future to care about this paper
}

ADRS frameworks evolve interpretable source code, yielding solutions that are debuggable, deployable, and free of runtime inference overheads. 
The framework operates through an LLM-driven feedback loop.  
In each iteration, the LLM generates a candidate solution (e.g., executable code), which is evaluated against a predefined benchmark. Promising solutions and their performance metrics are then incorporated into the prompt for the subsequent iteration, guiding the search toward better programs.  

\accheng{this should be topic sentence, paragraph below does not emphasize evaluation is hard clearly}

Crucially, the success of this approach depends on a robust, user-provided \textit{evaluation setup} to accurately measures the performance of candidate solutions.
While recent research focuses on improving the solution generation capabilities of ADRS~\cite{}, the evaluation pipeline remains a manual endeavor, one that is especially challenging for database systems. Databases are stateful, complex, and made up of tightly coupled components, making direct evaluation prohibitively slow. The overhead of recompiling, loading data, and benchmarking during each ADRS step often makes the hundreds of iterations required for convergence infeasible~\cite{}. \accheng{be careful about saying this and cite some things, recent research has shown cost models insufficient} Standard cost models in databases offer a faster proxy, but they frequently fail to accurately reflect end-to-end performance due to the intricate interactions between different system components. Furthermore, performance is highly workload-dependent, requiring candidate solutions to be tested against diverse benchmarks. These evaluation bottlenecks are exacerbated by massive search spaces of problems in this domain (e.g., finding the optimal set of SQL query rewrite rules is NP-Hard~\cite{}), making discovery of effective solutions difficult within a reasonable timeframe.

\begin{table}[t!]
    \centering
    \caption{Techniques for reducing evaluation costs. \accheng{move to 2.3, if we have figure in intro, should highlight our contributions}}
    \label{tab:evaluation_techniques}
    \vspace{-1em}
    \begin{tabular}{ll}
        \toprule
        \textbf{Technique} & \textbf{Description} \\
        \midrule
        Simulator & Approximates system logic. \\
        E2E performance model & Predicts e2e metrics faster. \\
        Workload subset & Measures subset of benchmarks. \\
        Search space reduction & Limits scope of optimization. \\
        \bottomrule
    \end{tabular}
    \vspace{-1.6em}
\end{table}

% \accheng{ADRS uses these techniques so mention they are good techniques, just hard to use
% Not that they are bad techniques}

 % overhead of end-to-end evaluation and massive design spaces
To overcome these overheads, database researchers reduce evaluation costs by employing several standard techniques (Table~\ref{tab:evaluation_techniques}), which can also be applied to ADRS evaluators. These methods navigate the trade-off between evaluation speed and quality. While effective, they are problem-specific and require considerable manual effort to implement. For instance, when optimizing localized components (e.g. buffer cache), hand-crafted simulators can approximate behavior without running the full system~\cite{}. However, constructing high-fidelity simulators is notoriously difficult while low-fidelity alternatives risk misleading the optimization process. Alternatively, we can model end-to-end performance (e.g., via learned models mapping cost estimation to query latency~\cite{}), but this requires significant effort in feature engineering and data collection. When dealing with large benchmarks, evaluation can also be accelerated by running only a subset of the workload~\cite{}.
This reduces evaluation time, but manually selecting representative queries is challenging and requires careful tuning to avoid overfitting. Finally, limiting the search space to a subset of optimization techniques can reduce the required iterations (e.g., ~\cite{}) but requires expert analysis to ensure critical opportunities are not excluded~\cite{}. Ultimately, these traditional approaches are powerful tools, but they rely heavily on human intuition to balance evaluation speed and quality, highlighting the need for a way to automate their application.

In this paper, we address this critical evaluation bottleneck. We apply ADRS directly to the traditional evaluation techniques described above, leveraging LLMs to automate this previously manual process. Rather than relying on a static, hand-written evaluator, we propose \textit{co-evolution}: the LLM iteratively refines both the candidate algorithm and the evaluator itself. 
Since evaluation techniques are problem-specific, we illustrate how we use AI to design efficient evaluations by considering  three ``classic'' database problems. In the buffer manager, we co-evolve the \textit{simulator} alongside the caching policy to automatically discover an algorithm that outperforms the state-of-the-art. For index selection, we co-evolve our \textit{model of end-to-end behavior} to discover a new algorithm that enables both better cost estimation and latency (30\% improvement) compared to existing methods. For query rewrites, we co-evolve the \textit{subset of workloads and search techniques} to generate a novel, deterministic policy that results in [2.0$\times$] lower latency and runs in over four orders of magnitude faster (<200ms vs. 80 minutes) than the state-of-the-art approach, which makes LLM calls per query. Beyond raw performance, these results highlight the practical advantage of evolving white-box code: the discovered solutions are interpretable, predictable, and deployable without specialized inference infrastructure.

First, to address the challenge of simulation, we propose automatically evolving simulators via ADRS. Crucially, we find that ``more is more'': more baseline implementations and metrics on the full system result in more effective simulator evolution. 

Second, databases may required domain-specialized data that are not present in LLMs. We propose bridging the context gap by ``constructing the context you need'' by co-evolve the context alongside the actual solution.
to enable the discovery of high-performance optimizations.

Finally, we discuss how to ``hone the signal'': successful discovery requires us to co-evolve what workloads and metrics to use in the evaluation setup.

\begin{figure}[t!]
  \centering
  \vspace{-0.7em}
    \includegraphics[width=0.48\textwidth]{figures/simulator.pdf}
  %\vspace{-1.2em}
  \caption{We implement a co-evolutionary loop to design both the simulator and solutions.}
  \vspace{-0.5em}
  \label{fig:buffer-cache}
\end{figure}

\begin{figure}[t!]
  \centering
  \vspace{-0.7em}
    \includegraphics[width=0.37\textwidth]{figures/query-rewrite.pdf}
  %\vspace{-1.2em}
  \caption{We co-evolve the context alongside the solution.}
  \vspace{-0.5em}
  \label{fig:query-rewrite}
\end{figure}

\begin{figure}[t!]
  \centering
  \vspace{-0.7em}
    \includegraphics[width=0.37\textwidth]{figures/index-selection.pdf}
  %\vspace{-1.2em}
  \caption{We co-evolve the evaluation objectives alongside the solution.}
  \vspace{-0.5em}
  \label{fig:index-selection}
\end{figure}

==> figures/2.8-overflow.tex <==

\accheng{needs to be substantial enough that people will want to read it

needs to come across as what is the vision rather than matter-of-fact, this is how it's gonna be

steer it towards a certain direction}

\accheng{where will finding better solutions matter the most?

use amdhal's law
bottleneck analysis

researchers now defined by their problem identification skills
}


4.2, 5.1

\subsection{Case Study \#2: Index Selection}

add challenge: noisy eval, eval is too expensive/noisy
5.2

\accheng{since we are AI-driven, not idea-driven, evaluation noise matters more with these iterative loops}

\accheng{Evolution Needs Discovery}

\section{Third Insight and Case Study...}

4.3: abstraction layer
4.4
Data-driven evolution

\accheng{Evolve in More Than One Dimension / Evolution is Not One-Dimensional}

\subsection{Case Study \#4: Txn Isolation}
4.1

\subsection{Case Study \#5: Anti-Pattern?}

\accheng{
3.0: all the insights
For each case study, describe how we arrived at this insight
Buffer: 
Insight 1. more is more: show one baseline
}

\accheng{
I arrived at this insight by doing this case study rather than the other way around

How should we use ADRS for DBs? My insights are solutions for these questions
}


To demonstrate the capability of ADRS in solving database performance problems, we investigate three diverse tasks. [reword, reads awk: Each case study follows a common schema that captures the problem setup, environment, evolutionary process, model usage, and final outcome, as detailed in Table~\ref{tab:expanded-schema} in the Appendix.]

In this section, we present a subset of representative case studies selected to highlight insights to guide future research. These examples illustrate both the limitations of current frameworks and new research directions under ADRS (detailed further in Section~\ref{sec:best-practices}). 
\accheng{We evaluate three open-source ADRS frameworks (GEPA, OpenEvolve, and ShinkaEvolve) using their default configurations. To ensure a fair comparison, we equalize the generation budget by capping each run at 100 iterations using the GPT-5 and Gemini-3.0-Pro-Preview models. We repeat each experiment three times. The specific configs are provided in Appendix \ref{sec:config_files}.}

The three case studies cover different DB components, summarized as follows:

\accheng{
\begin{itemize}

\item \emph{\textbf{CBL} - Optimizing Spot Instance Savings under Deadlines (Single Region):} Given a job with a deadline, the solution aims to maximize the use of cheaper spot instances in a public cloud without violating the deadline. ADRS improves the SOTA result by up to 35\% for a single region. 


\item \emph{\textbf{CBL-Multi} - Optimizing Spot Instance Savings under Deadlines for Multi-Region:} An extension of the single-region spot instance scheduling problem to multiple regions, where the policy must also choose migration timing and region placement. ADRS achieves 17\% improvements over a strong baseline in a multi-region setting. 

\item \emph{\textbf{EPLB} - Optimizing Expert Placement in MoE Inference:} The solution seeks to balance the load across GPUs by mapping the expert replicas across GPUs. ADRS provides a fivefold improvement in the time it takes to rebalance experts compared with the best-known proprietary implementation.

\end{itemize}
}

\textbf{Automated Simulation and Metric Discovery}
Constructing a faithful evaluation environment for the buffer manager presented a dilemma: full-system PostgreSQL emulation is too slow for the thousands of iterations required by evolutionary search, while abstract analytical models lack the fidelity to capture complex interactions like ``ring buffer'' strategies or dirty page write-back costs.

[emphasize key part: learning from some baselines!!]
To resolve this tension, we developed a trace-driven Python simulator that isolates the buffer management logic from the broader storage stack. Rather than manually re-implementing the system, we utilized the agentic framework to translate core C data structures—specifically buffer descriptors, block groups, and locking semantics—into a lightweight execution harness. This allowed us to replay real workload traces (TPC-H, TPC-C) orders of magnitude faster than wall-clock time while preserving the causal dependencies of eviction decisions. This isolation enabled the agent to explore the solution space rapidly, validating candidates against the simulator before promoting them to the full system.

Defining the optimization objective proved equally critical. Initial evolution runs targeted buffer hit rate, the standard proxy for cache performance. However, our analysis revealed a significant decoupling between hit rate and actual query latency; policies maximizing hit rate often evicted cheap-to-refetch sequential pages in favor of expensive random-access pages, or ignored the high cost of writing out dirty pages. To align the search with real-world performance, we evolved the metric itself into a latency score—a composite function weighting misses by their physical I/O cost (e.g., penalizing dirty evictions and random reads). This shift steered the search toward policies that minimized total system stall time rather than merely maximizing cache residency.

\textbf{Generalizing Simulator Construction}
This case study implies a broader methodology for database optimization. Instead of relying on monolithic, hand-tuned simulators, we envision an agentic framework capable of automatically extracting component-specific micro-simulators directly from the database source code. By isolating specific state spaces—such as the lock manager or query optimizer—and driving them with production traces, an agent can generate high-fidelity models that capture complex internal behaviors (like lock contention or cache thrashing) while remaining computationally tractable for iterative search.

Similarly, determining the correct optimization metric requires moving beyond single-dimensional proxies. As observed with the disconnect between hit rate and latency, the "right" metric is often a dynamic function of the workload’s physical constraints. Future frameworks should automate this discovery by correlating internal simulator states (e.g., WAL flush rates, IOPS, CPU usage) with external performance indicators. By treating the metric definition as part of the search space, the agent can learn a surrogate utility function that aligns the evolutionary process with the user's true performance goals, whether that be throughput, tail latency, or resource efficiency.

\subsection{Automatically Building Simulator and Determining Evolution Goals}

\textbf{Simulator evolution.} To automate the discovery of buffer replacement policies, we needed a simulator that balances fidelity to PostgreSQL internals with the flexibility for an LLM to experiment. We iterated through six versions to find this balance. Initial attempts (V1–V4) failed because they focused on the wrong constraints: V1 used Abstract Syntax Tree (AST) analysis to penalize code complexity, which stifled the emergence of novel strategies by constraining the form rather than the function. Conversely, V2–V4 strictly replicated PostgreSQL’s C implementation in Python; while accurate, this approach failed to expose high-level runtime metadata to the evolving policies. Without explicit awareness of active table scans or future access estimates, the evolved policies could not distinguish between sequential scans (cheap) and random point lookups (expensive), resulting in sub-optimal performance on mixed workloads.

\textbf{Providing sufficient context.} Our breakthrough (V5) came from identifying the correct abstraction layer: rather than constraining algorithms, we exposed rich runtime information—specifically scan contexts, estimated access times, and block groups. This visibility shifts the focus from guessing based on history to making intelligent decisions based on why a page is being accessed. Critical to this success was the integration of multiple ground-truth baselines (Clock-Sweep, PBM-PQ, PBM-Sampling). These served as "few-shot examples," allowing us to calibrate the simulator against known PostgreSQL behaviors and debug discrepancies between simulated and actual performance. By validating the simulator against these baselines, we ensured the infrastructure was realistic enough for the ADRS to synthesize robust strategies that adapt to different workload requirements without violating hard PostgreSQL constraints.

\textbf{Latency modeling.} We observed that early evolved policies achieved high hit rates in the simulator but failed to improve throughput in the actual database (V6). We traced this discrepancy to the simulator’s initial reliance on standard cache metrics, which treat all evictions equally. In reality, a synchronous dirty write (requiring a flush to disk before eviction) costs nearly $10\times$ more than a sequential read. To bridge this reality gap, we calibrated the simulator using NVMe latency profiles, assigning specific penalties to high-latency operations (e.g., 200µs for dirty writes vs. 20µs for sequential reads). This forced the evolutionary process to optimize for end-to-end throughput rather than simple cache residency, leading to the discovery of the \texttt{3WAY\_POLICY} which prioritizes the eviction of clean pages to preserve I/O bandwidth.

\textbf{Failure of strict constraints (V1–V4).} Initial attempts failed by focusing on the wrong optimization bounds. V1 used Abstract Syntax Tree (AST) analysis to penalize code complexity, which incorrectly constrained form over function and stifled novel strategies. Conversely, V2–V4 strictly replicated PostgreSQL’s C implementation. While functionally accurate, this approach obscured high-level runtime metadata. Without explicit awareness of active table scans or future access estimates, evolved policies could not distinguish between cheap sequential scans and expensive random lookups, resulting in sub-optimal performance.
\accheng{
1. we have cheap sequential scans vs. expensive random lookups

2. Equally critical was the integration of multiple ground-truth baselines

add table to summarize results
}

\textbf{Injecting sufficient context (V5).} Our breakthrough came from adopting a "more is more" abstraction strategy. We exposed rich runtime metadata—specifically scan contexts and access estimates—enabling decision-making based on why a page is accessed. Equally critical was the integration of multiple ground-truth baselines (Clock-Sweep, PBM-PQ, PBM-Sampling) to explicitly define the boundaries of the search space. These baselines served as anchors, demonstrating the range of realistic performance achievable within PostgreSQL's architectural limits. By calibrating against this known "feasible set," we ensured the simulator guided the agent toward strategies that were not only theoretically optimal but also valid within hard system constraints.

\textbf{Latency modeling (V6).} Early policies achieved high simulator hit rates but failed to improve real-world throughput. We traced this to the simulator’s reliance on abstract cache metrics, which treat all evictions equally, ignoring the "more is more" reality that physical context dictates performance. In practice, a synchronous dirty write costs nearly 10$\times$ more than a sequential read. To bridge this gap, we calibrated the objective function using NVMe latency profiles, assigning specific penalties to high-latency operations (e.g., 200µs for dirty writes vs. 20µs for sequential reads). This hardware-enriched context forced the evolutionary process to optimize for end-to-end throughput rather than simple cache residency, leading our final policy, which prioritizes evicting clean pages to preserve I/O bandwidth.


==> figures/3-problem.tex <==

\section{Problem Formulation}
\label{sec:prob}
A core challenge in applying ADRS to database systems is translating ambiguous, high-level requirements into a precise problem formulation that can guide an automated search. A complete formulation requires specifying not only what constitutes a \textit{correct} solution, but also what makes a solution \textit{good}, and what background knowledge is needed to find it. Accordingly, this section explores the three essential components of problem formulation for databases: extracting correctness constraints from application semantics, defining performance objectives, and providing the necessary operational and domain-specific context to the ADRS framework. \accheng{update this}

\subsection{Extracting Constraints}
For an ADRS framework to discover valid new algorithms, we must provide it with the appropriate correctness guarantees to define the search space of acceptable solutions. For databases, these guarantees can be broadly categorized into data consistency, transaction isolation, and database integrity constraints. Crucially, these constraints depend on application semantics, and developers often leave these rules implicit. Therefore, a critical research question is how we can infer (ideally automatically) these semantic requirements to establish the correctness constraints for applying ADRS framework.

We propose applying AI agents to extract and formalize these constraints. A promising  approach is to use a coding agent interface (e.g., Cursor) that allows the application developer to provide feedback as the agent constructs a comprehensive set of formal constraints. It could employ a combination of techniques, including static analysis of application source code to identify data invariants, monitoring runtime behavior to infer transactional boundaries, and engaging in an interactive dialogue with the developer to disambiguate requirements. The final output of this process is a set of specification that can be directly used by the ADRS framework, serving as the ground truth for verifying the correctness of any generated algorithm.

\accheng{show solutions, otherwise proposals}

\textbf{Data consistency.} Data consistency rules ensure that the database remains in a valid state. For example, in a banking application, a transfer of funds must debit one account and credit another by the same amount, ensuring money is not created or destroyed. Developers typically encode these rules in application logic (e.g., within an if-then-else block) rather than as a formal declaration. An AI agent could extract these semantics by analyzing application source code or through an interactive, multi-turn dialogue where the framework poses hypothetical scenarios to the developer to disambiguate the required invariants.

\textbf{Transaction isolation.} Transaction isolation guarantees protect concurrent operations from interfering with each other. For instance, a flight reservation application needs to determine the minimum isolation level required to preventing two users from booking the last seat on a flight. An AI agent could leverage existing transactional code if present or ask the developer a series of questions and provide suggestions to infer the precise isolation guarantees. Leverage concurrency anomaly testing is another promising route~\cite{jepsen}. We describe an initial framework in Section~\ref{sec:eval}.

\textbf{Database integrity constraints.} While declared integrity constraints like \texttt{PRIMARY KEY} or \texttt{UNIQUE} are already explicit in the database schema, many others are hidden within application logic (e.g., a manual check that a value must be positive). For the ADRS framework to operate with complete specifications, an AI agent must identify these implicit rules and formalize them. 

These specifications can serve as the ``ground truth'' for the ADRS framework, ensuring that the automated search is strictly confined to the space of correct algorithms.
% In summary, before an ADRS framework can begin its search for performant algorithms, it requires a formal specification of application correctness. Since these requirements are often undefined, a critical preliminary step is to deploy an AI agent to build this specification. This agent must actively extract implicit rules from source code and interactive dialogue, transforming them into a set of formal constraints. 

\subsection{Defining Objectives}
\label{subsec:objectives}
Beyond correctness, an ADRS framework requires well-defined objectives to guide its optimization search. While these frameworks excel at systematically exploring a solution space to find a Pareto frontier of optimal trade-offs, a key challenge is defining the utility function that represents a user's desired performance. \accheng{do we want to focus only on performance objectives here?} \accheng{cite Cosine for pareto frontier}

For databases, a primary challenge is articulating complex performance goals. Users, particularly on multi-tenant systems, often cannot define the precise trade-offs between competing metrics. While there are existing constructs like SLOs/SLAs for many database workloads, there is no principled way to define the relative importance of competing metrics, such as weighting throughput at 80\% and 99th percentile latency at 20\%. Furthermore, any such static weighting is inherently brittle, as workload characteristics and performance priorities can change over time. Towards this end, a more expressive framework to articulate complex performance goals could be an interesting direction of future research.

As a starting point, we propose a human-in-the-loop feedback mechanism that helps users identify acceptable objectives. 
Rather than requiring a user to specify a complete utility function upfront, a more practical goal is to first extract the key performance metrics and then allow a user to specify acceptable ranges along these different axes. We can leverage prior work on reproducing key workload characteristics~\cite{taobench} and work towards automating this with an agentic framework. Once these metrics are identified, the ADRS framework can be used to discover and present different points on the Pareto frontier. Each point represents a concrete performance trade-off (e.g., higher throughput for increased tail latency), allowing the user to provide feedback on which outcomes are preferable. This iterative process allows the framework to refine its understanding of the desired performance profile, effectively disambiguating the optimization objective over time.

\subsection{Determining the Optimization Target}
A crucial aspect of problem formulation is defining the nature of the desired solution artifact, as this shapes the entire search process. Many database optimization problems can be categorized as either ``offline,'' where extensive analysis is permissible, or ``online,'' where decisions must be made under strict, sub-second latency constraints. While the asynchronous, iterative model of ADRS is a natural fit for offline tasks, its application to online scenarios is more challenging.

Many database problems already have well-established offline formulations. For these, ADRS can be applied directly to search for a superior solution.
\begin{itemize}
% \item \textbf{Index tuning}: The classic offline problem is to select an optimal, fixed set of indexes for a static workload. This has been a long-standing challenge where heuristic-based greedy algorithms have been the state-of-the-art for decades~\cite{MS_greedy_index_tuning}.
\item \textbf{Query rewrite}: The search for novel rewrite rules or better algorithms for rule ordering is an offline process. The goal is to discover a new, static set of rules or a better heuristic that can be integrated into an existing query optimizer like Calcite, a direction already explored by recent LLM-based approaches~\cite{GenRewrite}.
\item \textbf{Workload tuning}: In the zero-shot setting, the goal is to produce a single, static set of knob configurations based on workload and hardware characteristics. This is the model used by both well-known rule-based tools like PGTune~\cite{pgtune} and recent learning-based systems~\cite{E2ETune_VLDB25}.
% \item \textbf{Plan-hint tuning}: This problem focuses on  deciding which hint sets to explore for a given query in tuning the best hint set for a query plan. ADRS frameworks can be used to improve upon learning-based approaches like Bao~\cite{Bao_SIGMOD21}.
\end{itemize}

However, many critical database challenges are online, which makes the direct application of ADRS infeasible. 
For online scenarios, we must shift the abstraction layer at which ADRS operates. The search for a solution remains an offline, iterative process, but the artifact being discovered is not a static configuration. Instead, it is a efficient \textit{policy} designed to be deployed into the live system to make decisions in real time.
\begin{itemize}
\item \textbf{Index tuning}: As workloads evolve, indexes must be adjusted. One potential formulation is to have ADRS discover a control policy that monitors query patterns and decides when to create or drop indexes based on real-time telemetry.
% \item \textbf{Workload tuning}: Iterative knob tuning in a live environment requires real-time adjustments. The ADRS optimization target should not be a single set of knobs, but a closed-loop control policy that dynamically adjusts system parameters based on observed workload behavior.
\item \textbf{Plan-hint tuning}: Deciding on the best hint set for a query as it arrives requires a decision in milliseconds. Rather than relying on a complex and slow ML model to predict execution time for each hint set, ADRS could be tasked with generating a more efficient, end-to-end decision-making strategy, perhaps a compact set of rules or a lightweight model, that can select the best hints with minimal runtime overhead.
\end{itemize}

\accheng{cases where this formulation is too hard?}

\accheng{ADRS in DBs is a more boring paper, not as surprising}

\subsection{Providing Context}
Moreover, another key research question is how to ground a general-purpose Large Language Model (LLM) with the specialized, stateful context required to reason about database systems. Providing this context effectively is a central challenge, as the ADRS search process is highly sensitive to its inputs. We identify three main categories of context relevant to databases:
\begin{itemize}
    \item \textbf{Live telemetry}: real-time operational data, which often resides in disparate sources like system catalogs, configuration files, and unstructured logs. A critical first step is making this data available in a structured, low-latency format. 
    \item \textbf{System architecture}: specifics about the particular database, such as the available tuning knobs, the concurrency control protocol, and the API primitives of its core components. This architectural context defines the valid action space for the ADRS, ensuring its proposed solutions are compatible with the target system.
    \item \textbf{Cutting-edge research}: the vast corpus of database literature should be used to inform the search for novel solutions.
\end{itemize}

\textbf{Context representation.}
A fundamental challenge is determining the optimal format for provide context to the ADRS. Raw data often cannot be directly inputted into an LLM due to its size, complexity, or format. For example, live telemetry is often too large to fit within model context windows, necessitating real-time summarization techniques. Similarly, academic literature should distilled into key ideas. A promising approach is to leverage Retrieval-Augmented Generation (RAG), where context is stored in a specialized vector database. The agent can then query this database to retrieve only the most relevant snippets of telemetry, documentation, or research papers pertinent to its current line of reasoning. However, this introduces further challenges:
\begin{itemize}
    \item \textbf{Timeliness}: retrieved context should not be stale, which could affect search results.
    \item \textbf{Summarization}: effective summarization techniques are needed for all context types to ensure the most salient information is extracted and presented concisely.
    \item \textbf{Consolidation}: we should synthesize coherent insights from these heterogeneous sources (e.g., combining a theoretical model from a research paper with live performance data).
\end{itemize}

\textbf{Context scope.}
Another critical open question is: how much context is appropriate? Simply providing more information does not guarantee better results. As demonstrated in prior work, an overly constrained or ``guided'' search can stifle the discovery of novel solutions that lie outside existing human knowledge. The challenge is to design abstractions that provide the necessary grounding without prematurely collapsing the search space. This requires navigating a delicate trade-off: the context must be detailed enough to allow for meaningful optimization but abstract enough to avoid constraining the search to only incremental improvements.Furthermore, this optimal level of context is likely not static. Just as a human researcher's focus shifts after reading different papers, the context provided to the agent should evolve as the search progresses. Initially, a broad overview of the problem space might be beneficial to encourage diverse exploration. However, once the agent identifies a promising direction, the context could become more focused, providing technical details about specific techniques to facilitate refinement and exploitation.



==> figures/4-simulator.tex <==
\section{Evaluation Frameworks}
Another core challenge in applying ADRS to database systems is the development of an evaluation framework that guide the search process. Such a framework should not only be \textit{fast} enough for iterative search and \textit{accurate} enough to be trusted but also \textit{comprehensive} enough to enable end-to-end optimization across the entire database stack. This section first the use of a spectrum of simulation to manage the trade-off between evaluation speed and fidelity. We then discuss how a hierarchical optimization model to manage the complexity of database systems.

\subsection{Spectrum of Simulation}



Database performance is notoriously difficult to simulate due to the complex interactions between components like the buffer manager, concurrency protocol, and storage engine, as well as dependencies on the underlying hardware. This creates a critical dilemma for applying ADRS: end-to-end system evaluations are too slow for the iterative feedback loop, while building a single, high-fidelity simulator is a prohibitively difficult.

To resolve this tension, we propose supporting a spectrum of simulation fidelities, ranging from lightweight analytical models to hardware-in-the-loop emulation. Rather than relying on a single simulator, the ADRS agent could begin its search using a fast, low-fidelity model, such as query cost models~\cite{sagedb} or more recent distribution-aware I/O models from auto-tuning frameworks~\cite{}, to rapidly explore the solution space and prune unpromising directions. It could then progressively validate the most promising candidates against slower, more accurate simulators, up to the full system.

\accheng{Writing analytical
models, as we did for I/O in the previous section, that capture in-
memory and hardware effects is extremely complicated and error
prone, even for a single design, as we have found in our prior
work}

A key research opportunity is to leverage the ADRS framework itself to \textit{automatically evolve} the simulator. By using replicating the real system’s performance metrics as the objectives (identified as described in Section~\ref{}), an agent could be tasked with generating models that match this behavior at varying trade-offs between evaluation cost and accuracy. This raises a core research question: what is the \textit{minimal set} of parameters and components required to accurately model a specific workload behavior? The answer is workload-dependent in databases; optimizing OLAP query plan may only require a cost model for I/O and CPU, whereas tuning a storage engine's compaction policies for a write-heavy workload would demand a detailed simulation of the LSM-tree structure, memtable, and block cache.

For database, full simulation is intractable in many cases, such as predicting the system-wide impact of a complex schema change. To deal with these scenarios, we envision an agentic framework 
capable of selectively modeling system behavior to predict performance. To ground this reasoning, the agent would first gather context by analyzing data distributions and query logs, then hypothesize about potential performance impacts, and finally automatically generate a lightweight proof-of-concept or a targeted micro-simulation to verify its hypothesis.

Ultimately, the need for fast, accurate evaluation motivates a broader shift in how data systems are designed. Unpredictable behavior in databases often stems from complex design decisions made to optimize performance and efficiency. We argue that future systems should instead be designed for predictability, as this would directly enable ADRS frameworks to more effectively optimize for other goals.

\accheng{Spanner slows down requests to have predictable latency}

\subsection{Hierarchical Optimization Across the Database Stack}
Looking forward, ADRS can enables end-to-end optimization of the entire database stack, overcoming the limitations of traditional, localized approaches. Current manual optimization of these systems is inherently local due to human bandwidth and organizational boundaries. In practice, large-scale database deployments are managed by siloed teams. For example, at Meta, the TAO, MySQL, and RocksDB teams optimize their respective layers of the stack largely in isolation. This partitioning makes end-to-end optimization difficult, as improvements in one component may be suboptimal or even detrimental when considering the system as a whole. ADRS presents an opportunity to optimize across these boundaries, furthering the vision of ``instance-optimized'' databases. This builds upon prior work in auto-tuning databases. Systems like Cosine were a pioneering step toward instance-optimized storage engines but required the manual construction of complex analytical models and were limited to a fixed template of design abstractions. ADRS can generalize this approach by \textit{automating} the creation of these models (e.g., not just limited to cost and latency~\cite{cosine} and the discovery novel algorithms and data structures that lie outside the predefined design space.

The central challenge we face in realizing this vision with ADRS is how to translate component-level improvements into end-to-end performance gains. A full-system simulation is often computationally intractable, while live end-to-end benchmarks are noisy, capable of obscuring the real impact of a targeted algorithmic improvement. Conversely, while component-level benchmarks provide a clean signal, they may not be representative of the final end-to-end performance.

We propose a hierarchical model where a high-level coordinating agent manages specialized ADRS agents for each database component. This structure allows the low-level agents to focus on well-defined, local optimization targets, providing them with a clean evaluation signal and keeping the problem scope manageable. The high-level agent is then responsible for orchestrating these components, leveraging a spectrum of simulation to progressively build a holistic model of system-wide performance. This approach, presents two primary research challenges:
\begin{itemize}
    \item \textbf{Automatically decomposing simulation}: How can an agent learn to automatically decompose a monolithic system simulation? This would require the agent to identify key sub-components, model their individual behaviors and interactions, and iteratively refine its composite model by comparing its predictions against the behavior of the real system.
    \item \textbf{Conflicting objectives:} How can the coordinating agent resolve the conflicting objectives that naturally arise between different system layers? For example, an aggressive buffer pool policy that maximizes cache hits may increase lock contention. The meta-agent must be able to navigate the system's global Pareto frontier, a task that requires extending the human-in-the-loop feedback mechanisms from Section~\ref{subsec:objectives} to guide the agent's trade-off decisions.
\end{itemize}

Overall, ADRS optimization motivates a shift towards modularity in database systems. We propose extending the notion of storage engine templates for key value stores, which introduced a structured dictionary of design abstractions, from prior work~\cite{cosine} to the general database systems. Database architectures should expose its core components (e.g., the query optimizer, transaction manager, and buffer pool) through clear interfaces. These APIs would make the system a manipulable environment for ADRS frameworks to optimize.

% \subsection{Other Simulation Observations}
\accheng{laoding data between every iteration is very slow and annoying!

TPC-H: ~10mins, TPC-C: 5-10mins, longer if more warehouses

I guess the forking DBs would be useful here}

==> figures/5-solution.tex <==
\accheng{framing: here's how we tried this new paradigm, good results, new field to explore}

\accheng{other option: this works in industry, clear differentiation from other papers}

\accheng{key problem right now: how to differentiate from previous paper
could make the case: the DB researchers are doing things wrong or DB researchers have lots of problems
}

\accheng{release env for ADRS: Postgres playground, tune postgres workload tuning
postgres setup that's fast to run, only work in memory, as speedy as possible, correctness and performance tests
e.g., Docker image with postgres to load data, etc.
harness to benchmarks, OE, consistency checker}

\accheng{add CacheLib results}

==> figures/6-discussion.tex <==

% \textbf{Spectrum of simulation.} 
% Performance objectives.


\textbf{How can we develop effective simulators?} While we showed a successful example of coevolution in Section~\ref{}, this case study focused on a specific database component. As we extend ADRS to optimize over multiple components, the full system, and even multiple different systems, we will need to build increasingly complex simulators. Building on our approach of co-evolving simulators, one exciting research direction is to support a cascade of simulators ranging from lightweight analytical models to hardware-in-the-loop emulation. Rather than relying on a single simulator, the ADRS agent could begin its search using a fast, low-fidelity model, such as query cost models~\cite{sagedb} or more recent distribution-aware I/O models from auto-tuning frameworks~\cite{}, to rapidly explore the solution space and prune unpromising directions. It could then progressively validate the most promising candidates against slower, more accurate simulators, up to the full system.

For complex changes where full simulation is intractable, such as schema changes, an agentic framework could be used to generate targeted micro-simulations. The agent would gather context from data distributions and query logs to hypothesize performance impacts and then automatically generate a proof-of-concept to verify its reasoning. Ultimately, the need for fast, accurate evaluation motivates a broader shift in how data systems are designed. Unpredictable behavior in databases often stems from complex design decisions made to optimize performance and efficiency. We argue that future systems should instead be designed for predictability, as this would directly enable ADRS frameworks to more effectively optimize for other goals.

% \subsection{Context}

% \textbf{Abstraction layer for optimization.}

% \textbf{Hierarchical optimization.}

% \textbf{RL.}

\subsection{Workloads}

\textbf{Live telemetry.}

How can we ground ADRS with the specialized, stateful context required for problem solving? 

The ADRS search process is highly sensitive to its inputs, so we must carefully manage context for these frameworks. For databases, context falls into three main categories: live telemetry from system catalogs and logs, architectural specifics such as tuning knobs and API primitives, and the vast corpus of database research literature. 

Providing this information effectively is a central challenge. For example, live telemetry often resides in disparate sources and must be structured for low-latency access. Architectural context defines the valid action space to ensure proposed solutions are compatible with the target system, while research literature informs the search for novel algorithmic techniques.

What are the optimal formats for representing and retrieving this context? Raw data is often too large for model context windows, necessitating real-time summarization. A promising direction is to use Retrieval-Augmented Generation (RAG) to store context in specialized vector databases, allowing the agent to query relevant snippets of documentation or performance data. This approach introduces several research problems, including maintaining the timeliness of retrieved context, developing summarization techniques that preserve salient information, and consolidating insights from heterogeneous sources. For instance, an agent may need to synthesize a theoretical model from a research paper with live performance metrics to ground its reasoning.

How much context is appropriate for autonomous discovery? Providing more information does not guarantee better results, as overly constrained searches can stifle the discovery of solutions that lie outside human knowledge. The challenge is to design abstractions that provide necessary grounding without prematurely collapsing the search space. We believe the optimal level of context is likely dynamic. Initially, a broad overview of the problem space may encourage diverse exploration, whereas later stages of the search require focused technical details to facilitate refinement. It remains to be seen how to navigate the trade-off between providing enough detail for meaningful optimization and maintaining the abstraction needed for creative discovery.

% 1. buffer manager: algorithmic and implementation optimizers? Should they be separate?
% want to select workload for technique to evolve

% 3. index: noisy eval

% \accheng{DBs are hard vs. DB research is hard

% writing txns are hard --> should frame this problem from a DB builder/researcher perspective 
% designing architectures is a different kind of problem
% what should we focus on?

% frame each problem from this angle
% then say in future work: this is also applicable to XYZ
% }

% \accheng{what is the best possible simulator? what does best mean?}

\textbf{}

\subsection{Evaluation}

% \textbf{Verification.}
% Verification is hard.

% \textbf{Correctness.}
% Leverage consistency/isolation.


[offline vs. online, just-in-time]
Are general-purpose algorithms becoming obsolete? Database systems historically rely on universal heuristics to ensure robust performance across unpredictable workloads. Instance-optimized designs challenge this by tailoring logic to specific data, but they typically introduce runtime inference overhead or demand heavy manual engineering. ADRS shifts this dynamic by generating and compiling bespoke, workload-specific source code on demand. This creates the possibility of disposable algorithms, where highly specialized components are deployed and then entirely rewritten from scratch as the workload drifts. It remains to be seen whether ADRS will primarily serve as an offline tool to discover better universal rules, or if it will enable databases that continuously rewrite their own core engines in production.


% \accheng{
% future applications
% generalizability vs. instance-optimized: what is the implication of this?
% different types of problems: external to DBs (query rewrite, index selection) vs. some you have to recompile (different application and requirement)

% limitations of performance, what are the implications of expanding to beyond performance
% }

\accheng{1. what is role of human and what level of human guidance

2. correctness: having bots evaluate tests for correctness is simpler than try to evaluate performance, writing better tests
}

\accheng{correctness}

[what is role of human and what level of human guidance]
What is the optimal level of human intervention in automated system design? Traditional database engineering requires developers to manually implement algorithms and construct rigorous benchmarks. While ADRS automates the generation of these components, the framework still relies on humans to define search spaces, constraints, and reward signals. As LLMs become capable of co-evolving both the solution and the evaluator, the role of the database researcher shifts fundamentally from writing low-level system code to specifying high-level invariants and workload semantics. Balancing this guidance is critical, as overly restrictive prompts stifle novel discoveries while unconstrained searches yield impractical results. It remains to be seen whether developers will stay closely in the loop as interactive supervisors or if ADRS frameworks will eventually synthesize production-ready engines entirely from high-level natural language specifications.

[changes in database design]
Ultimately, the need for fast, accurate evaluation motivates a broader shift in how data systems are designed. Unpredictable behavior in databases often stems from complex design decisions made to optimize performance and efficiency. We argue that future systems should instead be designed for predictability, as this would directly enable ADRS frameworks to more effectively optimize for other goals.
Overall, ADRS optimization motivates a shift towards modularity in database systems. We propose extending the notion of storage engine templates for key value stores, which introduced a structured dictionary of design abstractions, from prior work~\cite{cosine} to the general database systems. Database architectures should expose its core components (e.g., the query optimizer, transaction manager, and buffer pool) through clear interfaces. These APIs would make the system a manipulable environment for ADRS frameworks to optimize.

What happens when AI generation expands beyond performance optimizations? Current ADRS applications succeed readily on performance problems, such as caching or query routing, since these algorithms do not alter the underlying semantics of the database. A flawed cache eviction policy only degrades latency, whereas a subtle bug in transaction isolation or logging corrupts data. Applying these frameworks to complex subsystems like concurrency control introduces severe verification challenges. To safely evolve these critical components, the evaluation loop must integrate rigorous correctness checks, such as formal verification or exhaustive fuzzing. It remains to be seen whether automated frameworks can synthesize proven, core transactional logic without rendering the evaluation loop prohibitively slow.

[add paragraph about interesting problems/opportunities related to workload optimization (distinguish from system optimization)]
[formal specs, mention application specs]
\textbf{How can we leverage ADRS to optimize application queries?} Defining and maintaining semantic integrity is a prerequisite key challenge for applications. In database systems, these guarantees include data consistency, transaction isolation, and integrity constraints. However, developers often leave these rules implicit within application logic rather than declaring them formally. For example, a banking application may encode a balance invariant within an if-then-else block, or a reservation system may rely on specific isolation levels to prevent double-booking. Writing correct application code has long been a difficult problem~\cite{}, and safely optimizing it requires an explicit understanding of these often implicit requirements.

One possible direction is to employ AI agents to identify and formalize implicit constraints to serve as the ground truth for the ADRS framework. An agent could analyze application source code with other available context (e.g., example output, documentation, etc.) to identify data invariants or monitor runtime behavior to infer transactional boundaries. For complex semantics, a coding agent interface might allow the developer to disambiguate requirements through interactive dialogue or hypothetical scenarios. The final output of such a process would be a set of formal specifications needed for a particular query. Subsequently, we could leverage an ADRS framework to optimize this code (e.g., rewrite transactions) while leverage these specifications to ensure it preserves the intended behavior. 


==> figures/index-alg-comparison-old.tex <==
\begin{figure}[t!]
\centering
\vspace{-1.0em}
  \caption{Comparison of the Extend baseline with the best evolved index selection policy. Highlighted regions mark the key algorithmic innovations discovered by evolution.}
  \label{fig:extend_comparison}

  \begin{subfigure}{\linewidth}
      \begin{minted}[
          frame=lines,
          fontsize=\small,
          linenos,
          breaklines=true
      ]{python}
def Extend(workload, cands, eval, budget, K):
    sel, cost = [], eval.cost(workload, {})
    # Phase 1: Greedy -- best candidate each round
    while len(sel) < K:
        best, best_c = None, cost
        for idx in cands:
            if idx in sel or over_budget(sel, idx, budget):
                continue
            c = eval.cost(workload, set(sel)|{idx})
            if c < best_c: best, best_c = idx, c
        if not best: break
        sel.append(best); cost = best_c
    # Phase 2: Extend with additional columns
    for i, idx in enumerate(sel):
        for col in all_columns:
            ext = Index(idx.columns + (col,))
            c = eval.cost(workload, swap(sel, i, ext))
            if c < cost: sel[i] = ext; cost = c
    return set(sel)
      \end{minted}
      \caption{Extend~\cite{schlosser2019extend}}
      \label{fig:extend-baseline-code}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}{\linewidth}
      \begin{minted}[
          frame=lines,
          fontsize=\small,
          linenos,
          breaklines=true,
          highlightlines={2-7,9-19},
          highlightcolor=blue!10
      ]{python}
def EvolvedPolicy(workload, cands, eval, budget, K):
    memo = {}  # Memoize cost evaluations
    def get_cost(S):
        k = frozenset(S)
        if k not in memo:
            memo[k] = eval.cost(workload, S)
        return memo[k]
    base = get_cost({})
    # Pre-score: query-cost-weighted efficiency
    q_costs = [cost_per_query(q) for q in workload]
    for idx in cands:
        benefit = base - get_cost({idx})
        help = 1 + 1.5*query_overlap(idx, q_costs)
        score[idx] = (benefit/size(idx)) * help
        if "date" in table(idx): score[idx] *= 2.25
        if "store" in table(idx): score[idx] *= 1.75
    # Prune prefixes; keep top-30 by score
    prune_dominated_prefixes(cands, score)
    seeds = top_k(cands, by=score, k=30)
    # Single-pass greedy in pre-scored order
    sel, cost = [], base
    for idx in seeds:
        if not over_budget(sel, idx, budget):
            c = get_cost(set(sel) | {idx})
            if c < cost:
                sel.append(idx); cost = c
    # Same as Extend, using get_cost, top-20 cols
    ...
    return set(sel)
      \end{minted}
      \caption{Best Evolved Policy}
  \end{subfigure}
  \vspace{-1.0em}
\end{figure}


==> figures/insights-table-old.tex <==
\begin{table*}[t]
    \centering
    \caption{ADRS Framework Analysis}
    \label{tab:case_studies}
    \begin{tabularx}{\linewidth}{
        >{\hsize=1.2\hsize\raggedright\arraybackslash}X  % Column 1: Standard width
        >{\hsize=0.6\hsize\raggedright\arraybackslash}X  % Column 2: Slightly narrower
        >{\hsize=1\hsize\raggedright\arraybackslash}X  % Column 3: Widest (for long numbers)
    }
        \toprule
        \textbf{Insight} & \textbf{Case Study} & \textbf{Improvement Over SOTA} \\
        \midrule
        % Row 2
        \textbf{Co-evolve the workload and search space: \newline \textit{ ``Go off what you know''}} 
        \begin{itemize}[leftmargin=*, nosep]
            \item Exploit prior empirical successes to identify promising directions.
        \end{itemize} &
        Query Rewrite (Section \ref{sec:query-rewrite}) \begin{itemize}[leftmargin=*, nosep]
            \item Technique 3
            \item Technique 4
        \end{itemize} & 5.4$\times$ latency reduction on TPC-H,  6.8$\times$ latency reduction on DSB  \\ \addlinespace
        \midrule
        % Row 1
        \textbf{Co-Evolve the Simulator: \textit{``More is more''}}
        \begin{itemize}[leftmargin=*, nosep]
            \item More baseline implementations and performance data enable evolution to discover algorithms that translate into real improvements.
        \end{itemize} & 
        Buffer Cache (Section \ref{sec:buffer}) \begin{itemize}[leftmargin=*, nosep]
            \item Technique 1
        \end{itemize} 
        & 19.8\% higher hit rate, 11.4\% I/O volume savings \\ \addlinespace
        \midrule
        % Row 3
        \textbf{Co-Evolve the Evaluation Objectives: \textit{``Hone the signal''}} 
        \begin{itemize}[leftmargin=*, nosep]
            \item Balance between estimation and full metrics, adding sanity checks as necessary.
        \end{itemize} & Index Selection (Section~\ref{sec:index}) \begin{itemize}[leftmargin=*, nosep]
            \item Technique 2
        \end{itemize} & 6.3\% latency reduction on TPC-DS, 5.8\% latency reduction on TPC-H,  2.2$\times$ lower selection time on TPC-H \\  %Evolve beyond a single dimension
        \bottomrule
    \end{tabularx}
\end{table*}


==> figures/query-rewrite-latencies.tex <==
\begin{table}[t]
    \centering
    \caption{Latency results on TPC-H and DSB.}
  \label{tab:query-rewrite-latency}  
  \setlength{\tabcolsep}{1.5pt}
  \renewcommand{\arraystretch}{1.1}
  \scriptsize
  \begin{tabular}{@{}l ccc ccc@{}}
  \toprule
  & \multicolumn{3}{c}{TPC-H 10x} & \multicolumn{3}{c}{DSB 10x} \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
  Query Latency (s) & Average & Median & p90 & Average & Median & p90 \\
  \midrule
  PostgreSQL & 47.56 & 5.47 & 300.00 & 19.58 & 2.50 & 13.35 \\
  R-Bot (GPT-4o) & 22.58 ($\downarrow$52.5\%) & 5.47 ($\downarrow$0.0\%) & 28.18 ($\downarrow$90.6\%) & 11.55 ($\downarrow$41.0\%) & 1.86 ($\downarrow$25.6\%) & 12.08 ($\downarrow$9.5\%) \\
  R-Bot (GPT-5) & 22.55 ($\downarrow$52.6\%) & 5.47 ($\downarrow$0.0\%) & 27.70 ($\downarrow$90.8\%) & 11.55 ($\downarrow$41.0\%) & 1.87 ($\downarrow$25.2\%) & 12.08 ($\downarrow$9.5\%) \\
  \textbf{Evolved} & \textbf{8.78} ($\downarrow$\textbf{81.5\%}) & \textbf{4.76} ($\downarrow$\textbf{13.0\%}) & \textbf{21.33} ($\downarrow$\textbf{92.9\%}) & \textbf{2.85} ($\downarrow$\textbf{85.4\%}) & \textbf{1.62} ($\downarrow$\textbf{35.2\%}) & \textbf{7.43} ($\downarrow$\textbf{44.3\%}) \\
  \bottomrule
  \end{tabular}
\end{table}

% \begin{table}[t]                                                                                               
%   \centering                                                
%   \caption{Comparison of Query Latency.}                                                                         
%   \label{tab:query-rewrite-latency}                                                                              
%   \setlength{\tabcolsep}{1.5pt}
%   \renewcommand{\arraystretch}{1.1}
%   \scriptsize
%   \begin{tabular}{@{}l ccc ccc@{}}
%   \toprule
%   & \multicolumn{3}{c}{TPC-H 10x} & \multicolumn{3}{c}{DSB 10x} \\
%   \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%   Query Latency (s) & Average & Median & p90 & Average & Median & p90 \\
%   \midrule
%   \multicolumn{7}{@{}l}{\textit{R-Bot paper (PG14, 128GB, 3.1GHz):}} \\
%   Origin & 104.86 & 10.60 & 300.00 & 37.76 & 5.28 & 300.00 \\
%   R-Bot (GPT-3.5) & 55.71 ($\downarrow$46.9\%) & 10.41 & 300.00 & 26.19 ($\downarrow$30.6\%) & 4.61 & 35.25 \\
%   R-Bot (GPT-4) & 57.60 ($\downarrow$45.1\%) & 10.37 & 300.00 & 25.35 ($\downarrow$32.9\%) & 4.58 & 17.17 \\
%   \midrule
%   \multicolumn{7}{@{}l}{\textit{Ours (PG17, 144GB, 72-core, SSD):}} \\
%   Origin & 47.56 & 5.47 & 300.00 & 19.58 & 2.50 & 13.35 \\
%   R-Bot (GPT-4o) & 22.58 ($\downarrow$52.5\%) & 5.47 ($\downarrow$0.0\%) & 28.18 ($\downarrow$90.6\%) & 11.55
%   ($\downarrow$41.0\%) & 1.86 ($\downarrow$25.6\%) & 12.08 ($\downarrow$9.5\%) \\
%   R-Bot (GPT-5) & 22.55 ($\downarrow$52.6\%) & 5.47 ($\downarrow$0.0\%) & 27.70 ($\downarrow$90.8\%) & 11.55
%   ($\downarrow$41.0\%) & 1.87 ($\downarrow$25.2\%) & 12.08 ($\downarrow$9.5\%) \\
%   \textbf{Evolved} & \textbf{8.78} ($\downarrow$\textbf{81.5\%}) & \textbf{4.76}
%   ($\downarrow$\textbf{13.0\%}) & \textbf{21.33} ($\downarrow$\textbf{92.9\%}) & \textbf{2.85}
%   ($\downarrow$\textbf{85.4\%}) & \textbf{1.62} ($\downarrow$\textbf{35.2\%}) & \textbf{7.43}
%   ($\downarrow$\textbf{44.3\%}) \\
%   \bottomrule
%   \end{tabular}
%   \end{table}


==> figures/z-overflow.tex <==
This paper argues that AI optimization will be a first-class citizen in coming years. We describe how this affects databases, outlining the unique challenges in this area and future research directions.

% What is unique to DBs?
% Start with here’s what different
% Need to store data reliably, manage access, etc.
% Relational alg: many different ways to run same query
% Start with what’s different/challenging with DBs

% ADRS are very promising...

% This brings us to the challenges with applying ADRS to DBs.

, and this cannot be dynamically tuned along the Pareto frontier.

1. lack of framework

For instance, there is no principled way for a user to specify a preference like 80\% importance on throughput and 20\% on 99th percentile latency. Most systems currently only support a single weight between metrics, if at all.

Developers often lack a formal method to articulate the relative importance of competing metrics for a given workload. 

% \section{Searching for Better Solutions}

\accheng{DB research is gonna change.
it's gonna be less about solutions and more about problems.
what's the vision I want to convey?
ADRS already points this out
ADRS has already indicated that role of researchers shifting from solutions to problem solvers. what does this mean for DB researchers? in this paper, we're gonna pinpoint key problems that we need to solve to enable ADRS for DBs
these are: (i) tooling for problems
(ii) simulators
}

For instance, [example].
These systems need to store data reliably, manage concurrent access, optimize declarative queries, etc.
\item This complexity is compounded by the fact that these systems are also comprised on multiple layers and components, each of which is complex and individually optimized.
\item The interactions between these components create a vast and intricate search space for optimization, one that has traditionally required decades of meticulous, human-driven research to navigate.
\item For instance, [example]

    \item These ADRS frameworks leverage LLMs to generate algorithms that match or even exceed the performance of state-of-the-art, human-designed solutions for a range of systems performance problems. 
    \item These frameworks require users to formulate the problem and provide an evaluation framework to score candidate solutions generated by the LLM.
    \item ADRS implements a feedback loop in which LLMs are iteratively called to generate solutions, and these solutions are evaluated and scored to provide feedback for future iterations.
    \item Example of ADRS applied to txn scheduling

\accheng{results}

These rules are well-studied and there is sufficient formal specifications out there. The challenge is how to automatically infer these from application developers.

Databases provide a number of guarantees, which can be broadly categorized into data consistency, transaction isolation, and database integrity constraints. While there is extensive literature providing robust specifications for these guarantees, they are often implicitly defined by application developers in practice. Thus, a core challenge in this area is to automatically infer these semantic requirements to establish the correctness constraints for applying ADRS framework.

Another requirement of ADRS frameworks is the objectives for optimization.
ADRS frameworks enable a systematic search through the space of solutions, which will enable Pareto frontiers to be established. 
[summarize the two challenges/research directions below]

such as weighting throughput versus tail latency.
First, there is a need for a more expressive framework to articulate complex performance goals. 
In general, this is challenging as users may not know exactly how to weigh different performance metrics and how this might change over time. Users, especially on multi-tenant systems, often cannot articulate the precise trade-off between metrics like average throughput and tail latency. 

Since extracting a precise utility function from a user is difficult, a more practical goal is to first extract the key performance parameters and then allow a user to specify acceptable performance ranges along these different axes. We can then use the ADRS framework to generate different points on the Pareto curve and explain the tradeoffs to users. The user can provide feedback that iteratively refines the framework's understanding of their desired performance profile, effectively disambiguating the performance objectives over time.

However, current metrics are insufficient to capture the complex, multi-objective nature of system performance. 
\begin{itemize}
    \item There is no principled way to articulate the relative importance of competing metrics for a given workload for databases.
    \item While constructs like SLOs/SLAs exist, there is no principled framework to express a nuanced goal,, such as ``throughput is weighted at 80\% and 99th percentile latency at 20\%.''
    \item Supporting static weights is insufficient because workloads change over time.
    \item The rise of ADRS frameworks, which can be used to automatically discover performance Pareto frontiers, opens up the need for a model to consider performance tradeoffs systematically.
\end{itemize}

Moreover, another key goal is to automatically identify the key performance metrics.
\begin{itemize}
    \item This comes down to disambiguating specifications: a user might not know how important throughput is compared to tail latency for the many application workloads on a multi-tenant system.
    \item Extracting a precise utility function from a user is challenging. Instead, a more practical goal is to first extract the key performance parameters and then allow a user to specify acceptable performance ranges along these different axes.
    \item We imagine a human-in-the-loop feedback mechanism in which the ADRS framework can present the user with different points on the Pareto curve, allowing them to evaluate concrete trade-offs and provide feedback that iteratively refines the framework's understanding of the desired performance profile.
\end{itemize}

\textbf{How to format the context?} [better rephrasing of question?]
The right format to input context is an open question.
For example, since live telemetry is often too large to be used directly, an open research question is how to best summarize it to extract key insights. [also mention System architecture and Cutting-edge research]
[Mention RAG and storage of context]
[add more challenges about formatting context]

\textbf{How much context?}
Another critical open question is: how much context is appropriate? Simply providing more information does not guarantee better results. As demonstrated in prior work, an overly constrained or ``guided'' search can stifle the discovery of novel solutions. The challenge we face is to design abstractions that provide the necessary grounding without collapsing the search space. This requires navigating a delicate trade-off: [don't talk about APIs, talk about context] the APIs must be expressive enough for meaningful optimization but constrained enough to guide the search effectively. [mention this context should probably change as the search progresses, just like how real humans might change to different ideas after reading diff papers]

An open research question is what is the right context to provide to the LLM to help it find better solutions. bridge gap between a general-purpose Large Language Model and the highly specialized, stateful domain of database systems. The richness of this required context makes this a particularly acute challenge for the database domain.
\begin{itemize}
    \item LLMs are pretrained on a vast breadth of knowledge, but it is important to tailor this knowledge to the problems we are trying to solve.
    \item Furthermore, providing real-time data is a challenge
    \item Providing this context in an effective and timely manner is a central problem, 
    \item Recent work shows that ADRS search process is sensitive to input and feedback
\end{itemize}

There are three main categories of context for DBs: 
\begin{itemize}
    \item First, the agent needs access to the database's live operational telemetry, which currently resides in disparate, hard-to-access sources like system catalogs, configuration files, and unstructured query logs. Making this data available in a structured, low-latency format—for instance, by indexing logs as BigQuery has done—is a critical first step.
    \item Often, this data is too large to directly feed in. Summarizing and presenting the most important points are an open area of research. How to summarize and extract key insights? \accheng{look at monitoring/telemetry research here}
    \item Second, how to provide specifics about existing system architecture: the available tuning knobs, the specific concurrency control protocol in use, or the set of valid transformation rules in the query optimizer. 
    \item Third, how to leverage the decades of rich academic literature in the database field to inform its search for novel solutions?
\end{itemize}

\textbf{Context format.}
We propose the design of formal, agent-facing APIs and abstractions that expose this context in a structured and intentional manner. 
\begin{itemize}
    \item DB components should expose a clear API that allows an agent to query their internal state, propose a change, and receive structured feedback.
\end{itemize}

\textbf{How much context?}
A critical open question is how much context is appropriate? 
\begin{itemize}
    \item Simply providing more information does not guarantee better results. As demonstrated in the original ADRS paper, overly constrained or "guided" search can stifle the discovery of novel solutions that lie outside the scope of existing human knowledge. 
    \item The challenge, therefore, is to design abstractions that provide the necessary grounding without collapsing the search space to only include incremental improvements. 
    \item This involves navigating a delicate trade-off: the APIs must be expressive enough to allow for meaningful optimization but constrained enough to ensure the ADRS finds good solutions.
\end{itemize}

\accheng{mention direct applications and successes}

\accheng{frame this in traditional DB architecture or modern data stack?}

Challenges in DBs today:

Writing txns: correctness

Optimizing for performance

complexity

new workloads

designing new architectures, etc.

similar to software systems, cannot keep up with growing demands?

\accheng{need to differentiate from previous paper
focus here should be DB specific so probably don't need new eval results here
}

A core challenge in applying ADRS in general is formulating the problem precisely. A major part of this is specifying what the constraints are in code. However, problem specifications are often ambiguous or incomplete. 
We focus on two aspects of specifications for databases: application semantics and performance metrics. We also discuss providing sufficient context for the ADRS framework.

\accheng{can structure based on research process or just the steps outside of ADRS?}
% In this paper, we structure our exploration of these challenges by mapping them to the distinct stages of the scientific research process. We begin by examining the critical first step of problem formulation, where ambiguous human intent must be translated into a formal, machine-tractable objective. Next, we address the challenge of simulation and evaluation, a step made uniquely difficult in databases by the complex interplay of their many stateful components. Finally, we explore the complexities of searching for solutions, where the vast, multi-layered design space of a modern database must be navigated efficiently and safely. By systematically dissecting these challenges, we lay out a research agenda for building the next generation of ADRS frameworks capable of reasoning about and evolving these complex systems.

\accheng{need this to be specific so maybe defer for now}
\accheng{what are the types of challenges we want?}

Third, what is the appropriate abstraction layer to apply ADRS? Applying ADRS to DB components is non-trivial.
\begin{itemize}
    \item Online vs. offline
    \item Multiple layers
    \item Hints
\end{itemize}

(i) formalizing ambiguous objectives, (ii) developing sufficient simulators, and (iii) navigating a multi-layered and vast search space.

\accheng{focus on prob + simulation, other part is addressed}

(i) \accheng{problem formulation}, including the development of abstractions and APIs that can translate ambiguous performance goals and implicit application semantics into concrete objectives, and (ii) \accheng{evaluation}, which necessitates a new generation of simulation frameworks capable of providing rapid, high-fidelity verification for AI-generated artifacts. 

\begin{itemize}
    \item To apply ADRS, we need to either build representative simulators or identify the salient points of the problems we want to solve.
    \item 
\end{itemize}

Second, the performance of a database is notoriously difficult to simulate accurately, as it arises from complex interactions between its many components. 


detail the motivation, potential technical designs, and research implications of ADRS.

In the rest of the paper, we discuss the technical challenges and research opportunities in fully adopting ADRS for database systems.
\begin{itemize}
\item We begin by motivating the need for a new, AI-driven methodology for database systems research.
\item We then detail the core challenges in \textbf{problem formulation}, covering the need to automatically extract correctness constraints, define nuanced performance objectives, and provide effective context to the LLM.
\item Next, we address the critical challenge of \textbf{evaluation}, arguing for a new generation of simulation frameworks that can provide rapid, high-fidelity feedback and support hierarchical, end-to-end optimization.
\item Finally, we conclude by outlining a research agenda and discussing the broader implications of ADRS for the future of database systems design, from component-level algorithms to the architecture of the system itself.
\end{itemize}

In this paper, we discuss the technical challenges in fully adopting ADRS for DBs.
\begin{itemize}
    \item In the rest of the paper, we detail the motivation, potential technical designs, and research implications of ADRS. [fill in and add more bullets]
\end{itemize}

% \textbf{.}

% \textbf{.}

% \textbf{.}

To resolve this tension, we propose that a central goal of ADRS should be to automatically construct a spectrum of simulators, ranging from lightweight mathematical models to high-fidelity emulators. 
\begin{itemize}
    \item A range of tools, each giving a more precise semantics to the core abstractions in the system
    \item  The process would begin with a simple model---for instance, using established cost models for analytical workloads as a starting point---and would then be iteratively refined.
    \item \accheng{Mention COSINE cost models}
\end{itemize}

We can leverage the ADRS framework itself to generate this hierarchy of models, each with a different trade-off between fidelity and evaluation cost. 
\begin{itemize}
    \item Using the full system executions as the ground truth, the ADRS framework can generate simulators with the goal of matching the system along various performance metrics.
\end{itemize}

A core research question is: what is the minimal set of parameters and system components required to simulate desired workload behaviors? 
\begin{itemize}
    \item The answer is workload-dependent. For instance, optimizing an OLAP query plan might only require an accurate cost model for I/O and CPU, whereas optimizing an OLTP transaction scheduler needs a detailed simulation of the lock manager and thread pool contention.
\end{itemize}

Another core research question is: can we leverage AI to automatically identify the salient points of a problem?
\begin{itemize}
    \item This ties into our discussion on automatically identifying performance metrics in the previous section.
    \item ...
\end{itemize}

There are many scenarios in databases for which full simulation appears infeasible (e.g., predicting the system-wide impact of a complex schema change, representing all parameters for workload tuning).
\begin{itemize}
    % \item We propose an agentic approach to use LLMs to reason about what are the key metrics and what needs to be simulated.
    \item In these cans, we can use AI agent to reason about these effects, much like a human expert.
    \item To ground this reasoning, the agent would: (1) gather context by analyzing the data distribution, dependent code, and query logs; (2) hypothesize about potential performance impacts; and (3) automatically generate a lightweight proof-of-concept or a targeted simulator sub-component to verify its hypothesis against a defined set of metrics.
\end{itemize}

Ultimately, the advent of ADRS should motivate a broader shift in system design toward predictability. 
\begin{itemize}
    \item Prior work has show that unpredictable behavior in modern databases often stems from design decisions that prioritized performance, efficiency or resilience.
    \item We argue that future systems should instead be designed for predictability: a simpler, more predictable system is inherently easier for an ADRS framework to model and simulate accurately. This then enables ADRS to automatically optimize for performance and other goals.
\end{itemize}

\accheng{add takeaway: more complete simulator is, the solution for ADRS is better at the cost of accuracy and speed}

For these scenarios, we should try to reformulate the problem: instead of having ADRS make the online decision itself, its goal should be to generate a fast, lightweight \textit{policy} that can be deployed to make these decisions in real time.

A key challenge in applying ADRS to databases is the mismatch between its asynchronous, iterative evaluation model and the real-time decision-making required by many core database tasks. While offline problems permit time-consuming analysis, a database's core operational loop involves countless dynamic decisions that demand solutions on microsecond to millisecond timescales. This mismatch requires us to carefully define the right abstraction layer for the ADRS to optimize.

moving from finding static configurations to generating dynamic control policies.

[fill these next paragraphs out, add citations using the latex format ~\cite{}]
Many database problems already have ``offline'' formulations. 
\begin{itemize}
    \item \textbf{Index tuning}: offline (selecting indexes for a static workload
    \item \textbf{Query rewrite}: discovering new rewrite rules, and designing better algorithms for rule ordering/selection
    \item \textbf{Workload tuning}: zero-shot knob tuning
    \item \textbf{Plan-hint tuning}: an algorithm/strategy to decide which sets of hints to explore
\end{itemize}

There are still online challenges that are harder to directly apply ADRS. need way to cleverly formulate problem or otherwise minimize overhead of running ADRS
\begin{itemize}
    \item \textbf{Index tuning}: online (adjusting index selection as queries come)
    \item \textbf{Workload tuning}: iterative knob tuning in online setting, based on real-time workload info
    \item \textbf{Plan-hint tuning}: Directly let AI design an end-to-end strategy for hint tuning. The downside is that deciding on the best hint set without a prediction model might be challenging an ML model to predict execution time for each hint set to select the best plan for the query.
\end{itemize}

For many classic database problems, the optimization target is a static configuration. For instance, in budget-aware index tuning, the goal is to find an optimal, fixed set of indexes for a given workload, a problem where heuristic-based greedy algorithms have long been the state-of-the-art~\cite{MS\_greedy\_index\_tuning}. Similarly, in zero-shot knob tuning, the goal is to produce a single, static set of configuration parameters based on workload and hardware characteristics, a task addressed by well-known rule-based tools like PGTune and more recently by fine-tuned LLMs~\cite{cite:E2ETune_VLDB25}. For these problems, the conventional ADRS model is a natural fit: the framework searches a combinatorial space to find the best static artifact.

However, for the pervasive online challenges in a database, a static configuration is inherently brittle. A fixed queue depth for admission control cannot adapt to fluctuating workloads, nor can a constant deadlock timeout. For these scenarios, the optimization target for ADRS must be elevated from a static set of parameters to a dynamic control policy. The high-level goal is to have ADRS generate a stateful control algorithm that modulates its behavior based on real-time system feedback.
For workload tuning, instead of treating an LLM as an interactive advisor that suggests which of a storage engine's hundreds of knobs a human should turn, ADRS should autonomously generate a closed-loop tuning policy that adjusts these parameters in real time.
For query optimization, the goal is not merely to rewrite a single query or find a static set of plan hints. Instead, ADRS should discover novel rewrite rules, expanding beyond the manually crafted rule sets in systems like Calcite, or generate new hint-selection strategies to improve upon the learning-based approaches pioneered by systems like Bao~\cite{Bao_SIGMOD21}. Recent work has already shown that LLMs can be used to discover new, natural-language rewrite rules, demonstrating the feasibility of this direction~\cite{GenRewrite}.


% \subsection{Problem Setup: Determining the Right Abstraction Layer To Optimize}

\accheng{is online the right framing? complexity is alternative}

Database systems in particular have many ``online'' optimization scenarios that necessitate real-time, adaptive decision-making under strict latency constraints. 
\begin{itemize}
    \item While offline tasks like initial schema design or bulk data loading permit extensive, time-consuming analysis, the core operational loop of a database involves countless dynamic decisions.
    \item These online challenges are pervasive across the database stack, from workload management to transaction execution. [workload tuning example] Even modern adaptive query optimizers make online adjustments, altering a query's execution plan mid-flight based on the actual cardinalities observed, rather than relying on stale, pre-computed statistics.
    \item These problems demand solutions on microsecond to millisecond timescales, rendering the conventional ADRS model of asynchronous, iterative evaluation unsuitable when directly applied. 
\end{itemize}

This fundamental mismatch requires a shift in the abstraction layer at which ADRS operates (e.g., moving from finding static workload configurations to generating dynamic control policies).
\begin{itemize}
    \item For these scenarios, the optimization target for ADRS must be elevated from a static set of parameters to a dynamic policy. 
    \item The high-level goal is to have ADRS generate a stateful control algorithm that modulates its behavior based on real-time system feedback.
    \item A fixed configuration, such as a single queue depth for admission control or a constant deadlock timeout, is inherently brittle and cannot adapt to fluctuating workloads.
    \item Instead, ADRS could produce a novel admission control policy that dynamically adjusts its queue depth based on current CPU utilization and 99th percentile transaction latency, yielding a far more robust and general solution.
    \item For workload tuning, instead of treating the LLM as an interactive advisor that suggests which of RocksDB’s hundreds of knobs a human should turn, ADRS should autonomously generate a closed-loop tuning policy that adjusts these parameters in real time. For query optimization, the goal of ADRS is not to rewrite a single query, but to evolve the query optimizer itself.
\end{itemize}

Towards this end, we can leverage existing work on self-designing DBs. \accheng{could have this part of the motivation or simulator}
\begin{itemize}
    \item They present the essential abstractions that an ADRS framework would require. Specifically, they establish the closed-loop, data-driven feedback mechanisms for iterative improvement; they demonstrate the viability of replacing brittle, human-written heuristics with robust learned models; and most critically, they expose APIs that provide cost and cardinality predictions for hypothetical query plans, enabling rapid, low-cost exploration of the optimization search space.
    \item While these systems represent an advanced integration of learned models to replace heuristic-driven components, ... an ADRS agent could treat these APIs as primitives to rapidly evaluate novel architectural hypotheses, thereby transforming the database from an opaque system into a manipulable environment for automated discovery.
\end{itemize}

To deliver this information, we propose the design of formal, agent-facing APIs. Rather than ad-hoc prompting, database components should expose clear interfaces that allow an agent to query their internal state, propose a change, and receive structured feedback. [expand this paragraph more, how could this look? provide some different proposals]

[add a topic sentence talking about how ADRS enable e2e optimization for DBs]
Manual optimization of databases tends to local, constrained by both human bandwidth and organizational boundaries. In practice, large-scale database deployments are managed by siloed teams. For example, at Meta, the TAO, MySQL, and RocksDB teams optimize their respective layers of the stack largely in isolation. This partitioning makes end-to-end optimization difficult, as improvements in one component may be suboptimal or even detrimental when considering the system as a whole. ADRS presents an opportunity to globally optimize across the stack and tailor the database to the requirements of a given workload.

[make read better and flow well]
As previous work has showed, one size does not fit all for databases and we can more fully pursue the vision of an instance-optimized database that is automatically tailored to the exact requirements of a given workload. ADRS can be seen as the automated, generalized successor to prior work on auto-tuning databases. For example, systems like Cosine were a pioneering step toward instance-optimized storage engines, but required the manual construction of a complex, distribution-aware analytical I/O model and a fixed template of design abstractions. ADRS can automate this process entirely; an agent can be tasked with generating the simulation model, just as it generates the algorithm itself, learning the complex interactions that were previously modeled by hand. It can also come up with \textit{novel} algorithms and data structures, that were manually designed before so could only choose from fixed choices.

We propose a hierarchical model where a high-level coordinating agent manages specialized ADRS agents for each database component. This structure allows the low-level agents to focus on well-defined, local optimization targets, providing them with a clean evaluation signal and keeping the problem scope manageable. The high-level agent is then responsible for orchestrating these components. Leveraging the spectrum of simulation, it can start with low-fidelity models of component interactions and progressively build a more holistic simulation to predict system-wide performance. 
There are two main research challenges here: [frame the below as research questions]
\begin{itemize}
    \item \textbf{Automatically decomposing simulation}: enabling the agent to learn how to automatically decompose the simulation into multiple parts. The agent needs to identifying key sub-components, simulating them, and iteratively refining its model based on how well the composite simulation matches the real system's behavior.
    \item \textbf{Conflicting objectives:} navigating the competing objectives that naturally arise between layers; for example, an aggressive buffer pool policy that maximizes cache hits may increase lock contention. The responsibility of the coordinating meta-agent is to resolve these conflicts by exploring the multi-objective Pareto frontier for the entire system, using the human-in-the-loop feedback mechanisms described in Section~\ref{subsec:objectives} to guide its trade-off decisions.
\end{itemize}

[make read better]
To make this process easier, databases should be built to expose modular APIs that allow ADRS frameworks to more easily search for solutions. We can extending the notion of storage engine templates from prior work~\cite{cosine}. This has been done before for key-value stores where a structured dictionary of design abstractions is introduced. We can generalize database architectures in general, which should expose its core components—the query optimizer, transaction manager, and buffer pool—through similar structured, machine-readable interfaces, transforming the entire system into a manipulable environment for discovery.

This is challenging both from simulation and benchmark perspective. A key research question is how to consider to translate component optimizations into end-to-end performance? [mention challenges with simulation: too complex/expensive to simulate full system and benchmarking: end-to-end benchmarks have a lot of noise but component-wise benchmarks may not be representative of e2e performance]

We propose a hierarchical model (ADRS over ADRS), where a high-level coordinating agent manages a set of specialized ADRS agents, each responsible for a specific database component. 
The low-level agents focus on local optimization targets, to scope the tasks to get good results and stay within the context windows of existing models.
The high-level coordinating agent should consider how these pieces fit together. Can leverage our spectrum of simulation to build more and more complex models to simulate how the overall system will perform. [add more details] 
An interesting question here is can we automatically break down a complex problem into different parts? Can try to frame this problem as one where the agent determines various sub-components and simulates them. then it sees how representative the overall system simulation is compared to the real system.

A key challenge in such a framework is navigating the competing objectives that naturally arise between layers. The goals of individual components are often in direct conflict; for example, an aggressive buffer pool policy that maximizes cache hit rates may increase lock contention within the concurrency control manager. The responsibility of the coordinating meta-ADRS agent is to resolve these conflicts by exploring the multi-objective Pareto frontier for the entire system. We can extend prior work to present different points on the frontier and infer user desires based on the framework we described in Section~\ref{subsec:objectives}. 

To enable this, database components must expose formal, agent-facing APIs that allow the coordinating agent to set objectives, propose changes, and receive structured feedback, transforming the system into a truly manipulable environment for discovery. [write some more based on this: Cosine has storage engine template – a dictionary
of design abstractions to allow structured descriptions of arbitrary
key-value storage engine designs. --> extend this idea for general DBs]

\accheng{expanding the scope of research problem}
A fundamental limitation of human-driven optimization is that it is inherently local, constrained by both cognitive bandwidth and organizational boundaries. 
\begin{itemize}
    \item In practice, large-scale database deployments are managed by siloed teams, each with deep domain expertise in a single component; for example, at Meta, the TAO team, the MySQL team, and the RocksDB team optimize their respective layers of the stack largely in isolation. 
    \item This partitioning makes end-to-end optimization difficult as improvements in one component may be suboptimal or even detrimental when considering the system as a whole. 
\end{itemize}
\accheng{mention this helps contribute to instance-optimized DB vision}

ADRS presents an opportunity to [expand the scope of this optimization] \accheng{what about Harvard self-optimizing DBs?}
\begin{itemize}
    \item This new capability raises a central research question: How should we optimize end-to-end performance?
    \item An end-to-end approach could, in theory, discover globally optimal configurations that are invisible to localized optimizers.
    \item However, it faces a combinatorial explosion of the search space, which may render it intractable for complex systems.
    \item Simulation challenge here as well
\end{itemize}

We propose a hierarchical model (ADRS over ADRS), where a high-level coordinating agent manages a set of specialized ADRS agents, each responsible for a specific database component. 
\begin{itemize}
    \item In this paradigm, the top-level agent does not tune low-level parameters directly. Instead, its role is to define the objectives and constraints for the component-level agents. 
    \item A key research question is the best way to decompose the global optimization problem into a set of more manageable, localized searches.
    \item For instance, it might instruct the storage engine's ADRS to optimize for write amplification, while simultaneously tasking the transaction scheduler's ADRS with minimizing 99th percentile latency.
\end{itemize}

Another key challenge in such a hierarchical framework is navigating the competing objectives that naturally arise between different layers of the system. 
\begin{itemize}
    \item The goals of individual components are often in direct conflict; for example, an aggressive buffer pool policy that maximizes cache hit rates may increase lock contention within the concurrency control manager.
    \item  The responsibility of the coordinating meta-ADRS agent is to resolve these conflicts by exploring the multi-objective Pareto frontier for the entire system.
    \item This requires the principled mechanism described previously for navigating performance trade-offs to guide these AI agents.
\end{itemize}

Things like COSINE are steps towards this but super complex

To deliver this information, we propose the design of formal, agent-facing APIs. Rather than ad-hoc prompting, database components should expose clear interfaces that allow an agent to query their internal state, propose a change, and receive structured feedback. [expand this paragraph more, how could this look? provide some different proposals]

Enabling ADRS to discover these sophisticated policies requires treating the database less like a black box to be configured and more as a manipulable environment for discovery. We can leverage the essential abstractions from prior work on self-designing databases to this end. These systems have already established the necessary closed-loop, data-driven feedback mechanisms and, critically, exposed "what-if" APIs for components like the query optimizer. An ADRS agent can treat these APIs as primitives to rapidly and cheaply evaluate novel architectural hypotheses, making the discovery of complex, dynamic policies a tractable problem.

Cosine has storage engine template – a dictionary
of design abstractions to allow structured descriptions of arbitrary
key-value storage engine designs. --> extend this idea for general DBs

only limit goals of cost and latency

\accheng{DB usually end-to-end benchmarks but there is a lot of noise

on one hand, e2e has a lot of noise but smart alg only shows fraction of improvement

if only evaluate low level component, would see improvements

so what if it doesn't show up e2e

researcher problem: does it show up e2e or needs to be more specific
}

\accheng{pitch ADRS paper as measurement study for OSDI?}

\accheng{arxiv}

Second, building evaluation frameworks for ADRS represents a critical bottleneck. 
\begin{itemize}
\item To apply ADRS effectively, we need evaluation frameworks that can provide feedback orders of magnitude faster than traditional, end-to-end benchmark suites. However, database performance is notoriously difficult to simulate accurately, as it arises from complex interactions between its many components.
\item We argue for a spectrum of simulation that allowing ADRS to trade off speed and accuracy during its search. 
\item An additional challenge is determining the right abstraction layer for optimization; databases have may real-time, latency-constrained problems (e.g., query optimization, workload tuning) that require careful design of ADRS-compatible interfaces.
\item Finally, ADRS frameworks creates the opportunity for holistic, end-to-end optimization across the database stack, which necessitates evaluation frameworks that can manage competing objectives between different components and reason about global performance trade-offs.
\end{itemize}

For decades, the database community has pursued the vision of a self-optimizing system that can automatically adapt to its workload. This has led to a rich history of research in areas like auto-tuning and learned components. We argue that a new class of AI-driven approaches is poised to realize this vision at an unprecedented scale, supplanting the traditional, human-driven heuristic design processes.

This paper argues that AI-driven optimization will become a first-class citizen of database design in the coming years, supplanting the traditional, heuristic-driven approach. We describe how this paradigm shift will affect the database domain, outlining the unique challenges and future research directions in this area.

\accheng{many ppl don't know about ADRS
could also mention auto-optimizing DBs and tie it to that line of work

ADRS in DBs is a more boring paper, not as surprising
On top of that, to apply it to most problems, we need to solve correctness constraints
}

\accheng{assumes we want to apply ADRS directly
need to show potential
need to say that this can work
then say what is fundamental about DBs that is different: consistency, longer term correctness
}

\accheng{motivate that there is challenge}
Databases are elaborate systems that must satisfy a wide range of operational guarantees, making them a uniquely challenging domain for automated algorithm discovery due to two main reasons.
\begin{itemize}
    \item First, there is the challenge of \textit{specifying correctness and performance}. 
    \accheng{big difference between DB and other systems is that DB is stateful
    e.g., loading up data to see performance bottlenecks take a lot of time
    }
    These systems must adhere to strict consistency/isolation guarantees while simultaneously optimizing for multiple and often conflicting (e.g., availability, latency, etc.) performance objectives. This makes defining the optimization target a non-trivial task.
    \item Second, databases have \textit{immense complexity}. These systems are comprised of multiple layers and components, each of which is intricate and individually optimized. The interactions between these components create a vast and intricate search space for optimization, one that has traditionally required decades of meticulous, human-driven research to navigate. 
    \item For instance, developing an optimized concurrency control protocol involves navigating fundamental tradeoffs between throughput and isolation guarantees as well as modifying many components (transaction manager, log, etc.).
\end{itemize}

A new class of AI-driven approaches, called AI-Driven Research for Systems (ADRS), have begun to show promising results in automated algorithm discovery, finding solutions that exceed the performance of state-of-the-art baselines systems performance problems. 
\begin{itemize}
    \item To apply an ADRS framework, users need to formulate the problem by defining the search space (e.g., the set of allowable query rewrites) and providing an evaluation environment, such as a simulator or a testbed, to score candidate solutions generated by a Large Language Model (LLM).
    \item The ADRS framework implements a feedback loop in which LLMs are iteratively prompted to generate new candidate solutions. These solutions are evaluated used to refine the prompt for the next iteration, guiding the search better solutions.
    \item For example, [add txn scheduling use case]
    \item  Unlike prior ML applications to databases, which has primarily focused on black-box tuning by optimizing system parameters or replacing specific components with learned models (e.g., learned query optimizers), ADRS treats the system as a \textit{white-box} to optimize system code. \accheng{ok to say?}
\end{itemize}

While promising, adopting ADRS for database systems requires addressing fundamental challenges around (i) formulating the problem and (ii) constructing an evaluation framework. \accheng{not aligned with challenges before}

\accheng{need to say here what is different about DBs, need clear story for motivation
tension for challenge, what is the big challenge that we want to solve?}
In this paper, we identify the key research challenges in the database domain that must be addressed to enable this transition. We argue that realizing the full potential of ADRS for databases requires new approaches to: 

\ion{and the solution are} is


\textbf{Simulator Evolution.} We iterated through six simulator versions to enable the automatic discovery of buffer replacement policies. Initial attempts (V1–V4) relied on static analysis to enforce constraints or strictly replicated PostgreSQL internals, but these approaches proved either too restrictive or lacked the necessary abstractions for evolution. Specifically, V1 utilized Abstract Syntax Tree (AST) analysis to penalize complexity, which prevented the emergence of novel strategies, while V2–V4 improved the policy interface but failed to expose crucial runtime metadata. Without awareness of active table scans or future access estimates, evolved policies could not distinguish between sequential scans and random point lookups, resulting in sub-optimal performance on mixed workloads.
[say more about why you make these decisions, make sure tehre is enough context for a reader that doesn't know about simualtors before reading this]

\textbf{Information Exposure.} The breakthrough (V5) involved implementing a dedicated scan tracking infrastructure rather than complex algorithmic constraints. We introduced block groups (128 blocks) to track scan progress efficiently and exposed a NextAccessEstimator interface, allowing policies to query the estimated time until a buffer is reused. By passing precise access context (e.g., scan ID, position, and access type) with every request, we enabled the simulator to support diverse workloads such as TPC-H and TPC-C. This rich information interface allowed the evolutionary process to discover the COMBINED\_POLICY, which successfully balances scan resistance for analytical queries with frequency protection for OLTP workloads. [No, the key insight is below. we want to write about HOW we got to V5
Takeaways in trying to build a simulator automatically with Cursor
“Finding the right abstraction layer is key”
V5 succeeds largely because it exposes rich information (scan tracking, access context, estimation interface) that any algorithm can use
By exposing scan contexts, estimated access times, and block groups, the system allows algorithms to make intelligent decisions based on why a page is being accessed, rather than just guessing based on history
This visibility shifts the focus from specific algorithms to the underlying infrastructure, enabling the AI to synthesize strategies that adapt different workload requirements without breaking hard Postgres constraints.
Having multiple ground-truth baselines was critical (“few-shot examples”)
Essentially diverse unit/e2e tests (unit = baseline)
Signal from real evaluation results on the full system is crucial
Having PBM-PQ, PBM-Sampling, and Clock-Sweep (Postgres default) helped identify what data was useful for caching and what directions of improvements were feasible.
Having validated results also enabled Cursor to debug the simulator much faster and reason about flaws between its simulator and the ground truth.
PBM served effectively as a calibration tool to ensure the simulator was realistic. I then did additional prompting based on previous simulators to ensure evolution was not constrained only to PBM-like algorithms.
]

[again, make sure tehre is enough context for a reader that doesn't know about simualtors before reading this and make it understandable and clear. HOW did we come up with the insight we should focus on latency?]
\textbf{Latency Modeling.} To ensure simulated gains translated to real-world performance, we replaced simple hit-rate metrics with latency-aware scoring (V6). Standard metrics fail to capture the high cost of synchronous dirty writes (200µs) and random I/O (100µs) relative to sequential reads (20µs). We calibrated the simulator against NVMe measurements to penalize latency-heavy operations, incentivizing policies that prefer evicting clean pages and preserving random access patterns. This refinement led to the 3WAY\_POLICY, confirming that optimizing for end-to-end throughput produces more robust algorithms than optimizing for cache residency alone.

\#1: Buffer Manager

\textbf{Problem setup.}
The task is to select which pages to evict from a fixed-size buffer pool when new pages must be loaded. PostgreSQL's default CLOCK sweep algorithm uses recency as a heuristic, while PBM uses scan progress predictions to estimate future access times. However, PBM's sampling-based eviction uses a simple scoring function that does not account for page characteristics like dirty state, access frequency, or workload type.
This problem was studied in a VLDB paper~\cite{} and the result was improved in a recent Master's thesis~\cite{vanderkooy2023pbm}, which introduced Predictive Buffer Management (PBM), a sampling-based approach that uses scan progress estimates to approximate Belady's optimal algorithm. 

\textbf{Initial program and baselines.}
The initial program is PBM's sampling-based eviction policy~\cite{vanderkooy2023pbm}, which randomly samples buffers and selects the one with the furthest predicted next access time.
We compare against CLOCK sweep, PostgreSQL's default algorithm, and the original PBM sampling implementation.

\accheng{need to clarify here we are evolving simulator}

strictly replicating PostgreSQL's C implementation at a low level. 

\textbf{Optimization goal.} 

Our goal in this case study is to evolve a new cache eviction algorithm that leads to better throughput and latency. [add a bit more detail, paraphrase completely, do no directly reuse: Buffer management is a critical task in database systems. A database
system’s buffer manager controls memory with the task to limit
the number of buffers in use so that they fit in the main memory of
the machine running the database system.] PostgreSQL's default CLOCK sweep algorithm uses recency as a heuristic [add more details]. The state-of-the-art algorithm is PBM-Sampling, a sampling-based approach that uses scan progress estimates to approximate Belady's optimal algorithm. [add details from paper: 1-2 sentences summarizing key idea of alg and how it gets wins].



This creates a dilemma for ADRS: end-to-end evaluations are too slow for iterative feedback, while simpler simulators often rely on proxy metrics that fail to capture these trade-offs. To address this, we leverage the ADRS framework to co-evolve the simulator. We find that "more is more": accurate simulation relies on ground-truth baselines and performance comparisons on the full system. This approach allows the AI to automatically align the simulator's internal objectives with the full system. We present an example of how this insight applies with a case study on optimizing the caching algorithm for the buffer manager in Postgres to reduce I/O latency. We describe how we use Cursor to automatically evolve a simulator of the buffer manager, apply an ADRS (OpenEvolve) to the simulator, and show how it discovers an algorithm that improve throughput by up to X\% and latency by up to Y\%.

Our goal in this case study is to evolve a new cache eviction algorithm that leads to better throughput and latency. The buffer manager determines which database pages remain resident in the limited memory pool, making eviction decisions that minimize costly disk I/O. PostgreSQL's default CLOCK sweep algorithm uses recency as a heuristic for predicting future page accesses. The algorithm maintains a circular buffer of pages, each with a "usage count" that increments on access. When eviction is needed, the clock hand sweeps through pages, decrementing usage counts until finding a page with zero count to evict. While simple and efficient, this LRU-approximation approach struggles with sequential scan workloads where recently-accessed pages may never be needed again. The state-of-the-art algorithm is PBM-Sampling, a sampling-based approach that uses scan progress estimates to approximate Belady's optimal algorithm. PBM-Sampling tracks the progress of active sequential scans and estimates when each cached page will next be accessed, evicting pages with the furthest predicted reuse distance. By leveraging query-level semantics about scan behavior rather than relying solely on access history, PBM-Sampling achieves throughput improvements on scan-heavy analytical workloads compared to CLOCK.

To automate policy discovery, we need an evaluation framework to measure and compare the effectiveness of different caching policies. Since evolution on the full system is challenging due to implementation complexity and setup time (e.g., compilation, loading data, etc.), we describe our process in first using Cursor to evolve a \textit{simulator} that can accurately capture key characteristics relevant for caching policies. 
used Cursor to develop a simulator that balances execution speed with PostgreSQL fidelity. We iterated through six versions, discovering that we needed to expose more system state, not less, to bridge the gap between the simulator and the full system.

We began with a naive approach by directly prompting Cursor to build a simulator based on Postgres focusing on hit rates. Our first simulator versions attempted to faithfully replicate PostgreSQL's buffer manager implementation. We exposed the same data structures that PostgreSQL uses internally: buffer descriptors with tags, state flags, usage counts, and the buffer hash table. 

While functionally accurate, this approach buried high-level runtime metadata inside opaque data structures. PostgreSQL's buffer manager operates at the wrong abstraction level for intelligent eviction decisions. The buffer manager code can see a buffer's current usage count, whether the page is dirty or pinned, and the page's identity as a relation and block number. However, it cannot see which sequential scans are currently active, where those scans are in their progress through a table, which scans will access a given block in the future, or how fast those scans are progressing through their data. This information does exist somewhere in PostgreSQL (the executor knows about active scans, the storage manager tracks relations), but it is scattered across different subsystems and is not aggregated at the buffer manager level. When we replicated PostgreSQL's structure in our simulator, evolved policies had no way to predict future accesses. They could only react to past behavior, which is exactly what PostgreSQL's built-in clock sweep algorithm already does. The fundamental problem is that you cannot approximate Belady's optimal eviction algorithm without estimates of future access times, and PostgreSQL's buffer manager abstraction does not provide that information.

The key change [for what?] was providing access to multiple \textit{ground-truth baselines}: ClOCK, PBM-PQ (a precursor of PBM-Sampling available in the paper codebase), and PBM-Sampling. These baselines served as [reword, sounds awk] anchors, demonstrating the range of realistic performance achievable within PostgreSQL's architectural constraints. [we should focus on making point that multiple baselines help lay foundation for feasible search space, what kids of tehcniques ] By calibrating against this known feasible set, we ensured the simulator guided evolution toward strategies that were not only theoretically sound but also valid within hard system limits. This calibration revealed what was missing: the simulator needed to expose rich runtime metadata, specifically scan contexts and access estimates—to enable decision-making based on why a page is accessed, not just that it was accessed. This new simulator models the PBM's added abstractions and  exposes the same conceptual information (e.g., scan contexts, block groups, access estimates)

[make read better: there was one more thing we needed to refine.] [add nice transiton. we just assumed we should optimize for hit rate, and this also aligned with the simulator with the original VLDB `26 paper~\cite{}, which computes hit rates. Howeever, this was not accurate for full system performance. Evolved algorithms on the simulator got worse performance on the full system.] 
The final refinement (V6) added latency-aware scoring. Early policies achieved high simulator hit rates but failed to improve real-world throughput. The problem was that the simulator treated all evictions equally, ignoring that physical I/O costs vary dramatically. A synchronous dirty page write costs approximately 200 $\mu$ s, while a sequential read costs only 20$\mu$s, a 10$\times$ difference the hit rate metric completely ignores. Similarly, random index lookups cost approximately 100$\mu$s compared to 20$\mu$s for sequential reads, meaning a "wrong" eviction of an index page is 5$\times$ more expensive to recover from than evicting a scan page. 

Cursor identified this gap by comparing simulator predictions against real PostgreSQL benchmarks: policies with identical hit rates produced vastly different throughput depending on whether their misses triggered sequential reads or random dirty writes. Consequently, we calibrated the objective function using NVMe latency profiles, assigning specific penalties to high-latency operations.  This hardware-grounded context forced evolution to optimize for end-to-end throughput rather than cache residency alone. The resulting policies learned to prioritize evicting clean pages over dirty ones and to favor sequential scan victims over random access pages, not because scan pages are less valuable, but because the cost of being wrong about them is far lower. This cost-aware eviction strategy preserves I/O bandwidth where it matters most.

Simulator fidelity required aligning the optimization objective with physical I/O costs. 

[say something about final version of simulator? need transition] Finally, we needed accurately align the optimization objective of our simulator with full system performance. 

The default baseline is PostgreSQL's native query optimizer executing the unmodified query. This engine uses cost-based estimation and dynamic programming as a heuristic for plan selection. The algorithm generates candidate execution plans based on available statistics and indexes, selecting the one with the lowest estimated cost until the plan space is explored. While highly effective for standard queries, this general-purpose approach struggles with complex analytical queries where structural rewrites (like subquery unnesting) are required before physical optimization.

Applying general-purpose LLMs in database systems is challenging due to the specialized context required to optimize these systems. Obtaining and providing necessary information and data is crucial as the lack of sufficient context causes [find one term to replace examples:] 

We demonstrate this approach by using the LLM [to design data analysis and analyze results, reword to read clearly], using AI to automatically discover a rewrite policy that reduces latency by up to X.Y$\times$.

[paraphrase, don't copy reference text directly] To address this, a promising direction is to leverage emergent capabilities in comparative analysis. Our core insight is to ``mind the gap'': LLMs tend to perform well in comparative contexts. [rest of text is unclear, make it read better] By analyzing the delta between successful and regressive rewrites (A/B testing), we transform an open-ended generative task into a constrained pattern-matching task. We demonstrate this approach by utilizing the LLM as a semantic diff' engine to identify latent AST features that drive performance, [update rest of sentence accordingly] using Cursor to evolve the simulator and OpenEvolve to discover a policy that improves throughput by up to X\% and latency by up to Y\%.]

\accheng{add table to summarize results}

without the significant overhead of full-system compilation and data loading


without limiting expressive enough to represent complex policies.
and identifying the correct optimization metrics. 
We iterate through six versions, discovering that successful evolution required providing Cursor with both the baseline implementations and their performance data in the full system. 

This ground truth guided the AI to expose rich system state, specifically scan contexts and I/O latencies, in the simulator, [reword, sounds awk:] effectively bridging the fidelity gap with the full system. 


We initially prompted Cursor to build a simulator based on PostgreSQL's buffer manager [clarify we only based on clock, didn't give access to pbm-sampling or other policies for initial attempts], reasoning that structural fidelity would ensure [sounds awk:] policy transferability. Early versions of the simulator mirrored PostgreSQL's internals, exposing raw buffer descriptors, usage counts, and hash tables. However, this strict replication trapped policy evolution in local optima when starting from Clock. PostgreSQL's buffer manager observes low-level state (usage counts, dirty flags) but lacks the global context, such as active scan progress, needed for intelligent eviction. [don't start sentence with because, don't use em-dash] Because this metadata resides in the [what is executor??] executor rather than the buffer layer, the simulator excluded the state necessary to re-discover strategies like PBM-Sampling, which relies on future access estimates.
Conversely, when we told the AI to relax structural constraints [word better: without context from PBm-sampling and other baselines, the AI relaxed things in a way that led to evolved policies using expensive techniques (e.g.,full buffer pool scans or expensive computations) that were impossible to implement in the full system.] yielded policies that relied on full buffer pool scans or expensive computations. While effective in simulation, these were impossible to port to PostgreSQL's concurrent, latch-protected environment.


[make section more concise WITHOUT CUTTING DETAILS]
\textbf{[more interesting and relevant title?] Initial attempts.}
[reword to read better] We began with a straightforward approach, prompting Cursor to build a PostgreSQL-based simulator focused on hit rates by giving it context of the full system. Our first few versions faithfully replicated the full system implementation, exposing the same data structures: buffer descriptors, usage counts, and hash tables. These simulators seemed promising: if they matched PostgreSQL exactly, then policies evolved in simulation should transfer directly to real PostgreSQL code.

While functionally accurate, this approach buried high-level runtime metadata inside opaque data structures. PostgreSQL's buffer manager operates at the wrong abstraction level for intelligent decisions: it sees low-level state (usage counts, dirty flags, block IDs) but does not have the broader system state necessary for making better eviction decisions, such as active sequential scan progress and execution speed. Although this information exists in the executor and storage manager, it is not aggregated at the buffer layer. By replicating only the buffer layer, our initial simulator trapped evolution to a restricted search space. Consequently, the AI could not even re-discover known strategies, such as PBM-Sampling, which relies on future access estimates to improve upon the default CLOCK algorithm. 

Conversely, when we relaxed the requirement to strictly mirror PostgreSQL's internal structures, this resulted in simulators that produced evolved algorithms relying on scanning the entire buffer pool or expensive computations that, while effective in simulation, were impossible to port to PostgreSQL's concurrent, latch-protected environment.

The key change for successful simulator evolution was providing access to multiple ground-truth baselines: Clock, PBM-PQ (a precursor of PBM-Sampling available in the original paper codebase), and PBM-Sampling. These baselines established the boundaries of a feasible search space, demonstrating which algorithmic techniques could be implemented within PostgreSQL's architectural constraints without over-constraining the design space. This calibration guided the AI to expose rich runtime metadata, such as scan contexts and speed, enabling decision-making based on why a page is accessed. Our final simulator modeled the additional components beyond the buffer manager, exposing sufficient conceptual information (e.g., scan contexts, block groups, access estimates) for evolution.


Our final simulator version required one additional refinement: the optimization objective itself. We initially assumed we should optimize for the cache hit rate, aligning with the VLDB `26 paper~\cite{} simulator. However, this proxy proved insufficient for full-system performance: evolved algorithms achieving high simulator hit rates actually degraded real-world throughput. The problem was that the simulator treated all evictions equally. This ignores dramatic physical I/O cost variances: a synchronous dirty page write (~200$\mu$s) is 10$\times$ slower than a sequential read (~20$\mu$s). Similarly, recovering a random index page (~100$\mu$s) is 5$\times$ more expensive than refetching a sequential scan page.

Cursor was able to identify this gap when we gave it the performance results on the full system. By comparing simulator predictions against real PostgreSQL benchmarks, it discovered that policies with identical hit rates produced different throughput, depending on whether misses triggered cheap sequential reads or expensive random dirty writes. Consequently, Cursor calibrated the objective function to incorporate operation latency. This hardware-grounded context forced evolution to optimize for end-to-end system performance. This again demonstrates our "more is more" insight: by exposing the full system's latency characteristics to Cursor, the AI learned to model hardware-level trade-offs that previous simulator versions lacked. Subsequent evolution led to policies that prioritized evicting clean pages and sequential scan victims over dirty or random-access pages, not because scan pages are less valuable, but because the cost of a "wrong" eviction is far lower, preserving critical I/O bandwidth. We describe the results of our best evolved policy next.

The simulator initially considered only cache hit rate, but this metric alone was insufficient. [...transition to this sentence] because it treats all evictions equally, ignoring physical I/O costs: synchronous dirty writes ($\sim$200$\mu$s) are 10$\times$ slower than sequential reads ($\sim$20$\mu$s). By comparing [clarify what simulator predictions] simulator predictions against full-system performance data of evolved baselines, Cursor identified that policies with identical hit rates yielded different throughput depending on eviction cost. 
This again demonstrates our "more is more" insight: by exposing the full system's latency characteristics to Cursor, the AI learned to model performance trade-offs that previous simulator versions lacked. Consequently, Cursor calibrated the objective function to incorporate operation latency. 
Subsequent evolution led to policies that prioritized evicting clean pages and sequential scan victims over dirty or random-access pages, not because scan pages are less valuable, but because the cost of a "wrong" eviction is far lower, preserving critical I/O bandwidth. 

we must navigate the design space to [reword: find an abstraction] that balances execution speed with the fidelity.

Crucially, the optimal simulator is not known \textit{a priori}. simulator evolution is a search problem distinct from, yet parallel to, policy evolution: we must navigate the design space to find an abstraction that balances execution speed with the fidelity required to correctly rank—rather than perfectly mimic—candidate policies.

[don't say world model explicility, just describe the things as before to tie the idea to world model] refines the world model through iterative execution feedback to automatically discover a rewrite policy that reduces latency by up to 17.8$\times$.

[make more concise WITHOUT CUTTING CONTENT] Applying general-purpose LLMs in database systems can be challenging due to the specialized context required to optimize these systems. Obtaining necessary information is crucial as the lack of sufficient context causes ADRS solution generation to fail (e.g., LLM hallucinations, ineffective solutions). We address this by constructing a domain-specific world model~\cite{} [define world model, what does simulator env mean? reword to be clearer] to simulate the missing environment. Our core insight is to ``create the context'': when direct observation is limited, we co-evolve a simulator to [reword based on clarification above] predict system dynamics and guide the agent. [paraphrase: We demonstrate this approach by using Claude Code] to [update content based on @] orchestrate a data analysis pipeline to discover effective rule combinations for SQL query rewrites and interpret the resulting performance deltas, using AI to automatically discover a rewrite policy that reduces latency by up to 17.8$\times$.

Applying general-purpose LLMs in database systems is challenging due to the specialized context required to optimize these systems. Obtaining and providing necessary information and data is crucial as the lack of sufficient context causes ADRS solution generation to fail (e.g., LLM hallucinations, ineffective solutions, etc.). We address this by exploiting the emergent capability of LLMs to perform differential diagnosis. Our core insight is to ``mind the gap'': while often unreliable in isolation, LLMs exhibit strong reasoning capabilities with comparative analysis. We demonstrate this approach by using Cursor orchestrate a data analysis pipeline to discover effective rule combinations for SQL query rewrites and interpret the resulting performance deltas, using AI to automatically discover a rewrite policy that reduces latency by up to 17.8$\times$.

The default baseline is PostgreSQL's native optimizer executing unmodified queries. PostgreSQL uses cost-based estimation and dynamic programming for plan selection, generating candidate plans based on statistics and indexes and selecting the lowest-cost option. While generally effective for standard queries, this approach struggles with complex analytical queries where structural rewrites (like subquery unnesting) are required before physical optimization. The state-of-the-art algorithm is R-Bot, a retrieval-augmented (RAG) approach that uses LLMs to guide Apache Calcite's rule-based rewriter. R-Bot retrieves relevant rewrite recipes and Q\&A pairs, then leverages a Large Language Model to iteratively select and arrange specific Calcite optimization rules. By using the LLM to drive the Calcite engine rather than relying solely on the database's native planner, R-Bot achieves significant latency reductions on complex workloads compared to standard PostgreSQL execution.

[make more concise WITHOUT CUTTING CONTENT]
\textbf{Initial attempts.} We began by applying OpenEvolve directly to generate query rewrite policies but found that this strategy plateaued quickly. This evolutionary loop compiled LLM-generated variants, benchmarked them against TPC-H queries, and returned a score based on cost estimation improvements for the next iteration (we could evolve directly on Calcite in this use case, so no simulator was needed). This approach failed because the feedback signal was too coarse and the optimization metric was misaligned. The LLM received only an aggregate score, obscuring which specific queries improved and why, effectively forcing it to guess in the dark. Furthermore, by optimizing for internal Calcite cost rather than execution latency, the evolution often produced plans that improved estimates but regressed actual runtime (e.g., improving cost metrics while degrading latency by 48\%). Unlike R-Bot, which performs inference per-query, this approach attempted to evolve a single global policy to handle all queries simultaneously. This overwhelmed the model with conflicting signals across the workload, trapping the evolution in a local optimum unable to beat the SOTA baseline.

We begin by measuring the performance of a set of rule combinations and orders on a pre-defined training set of queries. The \textit{Searcher} module executes an [clarify what this means] adaptive search, testing permutations of optimization rules (from a finite set of templates) on each query and recording the execution latency. This produces a ground truth dataset mapping query features to performant rule sets. [need to mention that while this is NP-Hard, we can use match function from @rbot.md to filter many rule sets, makes serach space more feasible]

\accheng{
entire evolution history is valuable
how to retrieve the history
}

Cursor developed an ADRS framework that searches in pattern space (grounded in data) rather than in code directly: \accheng{this is a loop, need to clarify}
\begin{itemize}
    \item \textbf{Phase 1: Ground truth collection.} We begin by establishing the theoretical maximum performance for a diverse training set (TPC-H, DSB). We execute an offline brute-force search, applying every permutation of optimization rules (up to $k=3$) to each query and measuring the \textit{actual execution latency} on the target database. This produces a ground truth dataset mapping each query to its optimal rule sequence. \accheng{mention that set of rules to try is finite, can filter rules}
    \item \textbf{Phase 2: \accheng{rename, too old generation} Feature engineering.} Next, we extract discriminative features from the query structure to explain the variance in optimal rules. By parsing queries into relational algebra trees, we compute boolean and quantitative features (e.g., \texttt{hasSelfJoin}, \texttt{joinDepth}). Crucially, we employ differential analysis on queries where specific rules succeed versus fail to discover subtle structural determinants (e.g., \texttt{isFilterOnBuildSide}), annotating every query with a rich feature vector. \accheng{we are pattern matching / correlating results to query features}
    \accheng{how do we do correlation? check}
    \item \textbf{Phase 3: Pattern discovery.} We then learn generalized patterns that map these feature vectors to optimal rule sequences. Using a combination of association rule mining and LLM-guided hypothesis generation, we identify correlations (e.g., ``If \texttt{hasScalarSubquery} AND \texttt{!hasSelfJoin}, THEN apply \texttt{FILTER\_SUB\_QUERY\_TO\_CORRELATE}''). We select a minimal set of patterns that maximizes coverage of performance wins while strictly enforcing safety (zero regressions) on the training set.
    \item \textbf{Phase 4: Implementation and evaluation.} Finally, we compile the discovered patterns into deterministic Java code (\texttt{RuleSelector.java}). This optimizer is validated on a hold-out set of unseen queries. If regressions occur, we perform root cause analysis to identify missing features, feeding them back into Phase 2. The result is a production-ready optimizer that runs in $<1$ms (lookup speed) while delivering the performance of the expensive offline search.
\end{itemize}

\textbf{Getting the right data.}
To successfully evolve a better query rewrite algorithm, we needed more \textit{data} on which rules worked for which queries. Cursor realized this by comparing our initial evolution results, which had negligible gains, to the R-Bot baseline achieved order-of-magnitude speedups on the same workload using standard Calcite rules. This discrepancy revealed that the bottleneck was not a lack of effective rules, but a failure of search strategy: R-Bot succeeded by optimizing per-query, while our evolution failed by forcing a single static policy across diverse queries. To bridge this gap, we pivoted from generating policies based solely on latent LLM knowledge to a ``search and classify'' strategy in which we leveraged the AI to to orchestrate data analysis experiments, using the resulting empirical feedback to synthesize better policies.

under the right abstraction.
            \item \textit{More performance metrics} 

We propose leverage agents to manage context  incorporating an exploratory data analysis component in ADRS and leverage LLMs to pattern match on this data (``mind the gap''). 

While this has more recently evolved to include auto-tuning and learned components, the discovery of novel algorithmic approaches has remained a manual endeavor. A new class of AI-driven techniques is poised to automate this process.

they iteratively proposing and refining solutions until a satisfactory one is discovered or the iteration limit is reached, as depicted in Figure~\ref{fig:adrs-architecture}. 

At its core, 

of ADRS lies in its application to the more foundational and complex challenges in database design—those that involve intricate correctness constraints, vast and unstructured search spaces, and deep inter-dependencies between components. 
Moving beyond isolated components to these core problems presents a significant leap in complexity. For example, in workload tuning, the challenge is not to provide guided recommendations on which of RocksDB's hundreds of knobs to turn, but to automate the entire feedback loop of hypothesis, configuration, and verification. 
Similarly, for query optimization, the goal is not merely to use an LLM for query rewriting, as recent work has explored, but to evolve the optimizer's core logic itself, a task that requires navigating a combinatorially vast search space while rigorously maintaining semantic equivalence.
Similarly, for storage and transaction management, the ADRS could evolve entirely new data structures or concurrency control protocols.

\section{Case Study/Eval}

\begin{figure}[h!]
  \centering
  \vspace{-0.7em}
    \includegraphics[width=0.48\textwidth]{figures/llm-txn.png}
  %\vspace{-1.2em}
  \caption{LLM-Txn}
  \vspace{-0.5em}
  \label{fig:llm-txn}
\end{figure}

ADRS are effective in part because LLMs are trained on vast, diverse datasets and can discover novel solutions by identifying patterns from different domains. For instance, the novel MoE load balancing algorithm uses Hamilton's Apportionment from Political Science to efficiently assign replicas. 

[not just cross-domain but also mention benefit of speed: ADRS search until budget runs out, can keep looking for even smallest of wins and automated process, present as two main benefits] The effectiveness of ADRS stems from the ability of LLMs to identify patterns and techniques from diverse domains. For instance, the aforementioned MoE algorithm uses Hamilton's Apportionment from political science to efficiently assign replicas.

[integrate this idea nautrally around here as motivation: This capability addresses the challenges of holistic optimization amidst increasing hardware and workload complexity. Mention that we have to move towards automation because getting too complex, increasingly diverse workloads and systems and hardware to be able to keep up manually]
[too many grandiose words:] These sub-problems are self-contained optimization challenges prime for automated discovery. [sounds less aggresive: ] While prior work attempted to replace these components with learned models~\cite{}, black-box approaches [explain what worst-case guarantees are, use often suffer from high inference overhead and unpredictability] often fail to meet the strict worst-case guarantees required by production environments~\cite{}. 

[work these ideas in as well and make them transition and flow logically]
In particular, ADRS advances the community's vision of instance-optimized databases. While existing efforts focus largely on applying learned components, ADRS can automate [what does this mean? confusing:] the design of internal system logic itself. Finally, ADRS accelerates the development lifecycle, allowing researchers to identify optimizations that would typically require years of manual engineering.

Beyond optimizing specific components, we envision extending ADRS-based optimization to architectural design. For instance, we could synthesize entirely new data structures or concurrency control protocols ``just-in-time'' for the current application workloads. [should this point go earlier?] Furthermore, ADRS accelerates the **development lifecycle by allowing researchers to ``fail fast.'' The framework automates the validation of thousands of candidates, rapidly discarding unstable designs to isolate the rare solutions that are robust enough for deployment.


ADRS is especially exciting for databases because databases are made of heuristics. The modern database system is a composition of highly specialized components, many of which present self-contained optimization problems that are prime targets for ADRS frameworks. Many complex components that are manually tuned or replaced by learned components~\cite{}. However, these struggle due to robustness in practice. By evolving code, we can generate understandable solutions that can be feasibly deployed. 
For example, Datadog has used it to do achieve 10 $\times$ faster performance on XYZ~\cite{}... 

The idea of instance-optimized databases is already popular in the community. ADRS furthers this vision, addressing the concerns of more knobs, holistic optimization, and robustness in particular. Furthermore, ADRS can accelerate the pace at which solutions are developed.
\accheng{what are the key benefits to highlight? robustness? acceleration?}

While these early wins are promising, there is further potential in redesigning components of the database altogether. For example, we could evolve entirely new data structures or concurrency control protocols based on the workload. Optimize ``just-in-time''.

% \accheng{we acknowledge that worst case design is very important in production

% needs to be productionized and battle-tested

% ADRS allows us to fail faster

% query plans in production: get the bad 1\% and have Domas hand-tune

% Domas trying out Claude on query rewrites

% Sql optimizer guy
% }

% Many of these components have well-defined inputs and clear performance metrics. Early successes in industry already validate this approach. For instance, recent work at Meta on caching algorithms with MetaMuse has shown that ADRS can discover novel, high-performance eviction policies for buffer managers. Similarly, ADRS has proven effective in the domain of scheduling, with Databricks leveraging it to manage OLAP query execution and lower latency, and the SMF scheduler for OLTP transactions demonstrating its ability to navigate complex trade-offs in highly concurrent workloads.
% These direct applications confirm that ADRS can already match or exceed human performance on well-scoped, component-level optimization tasks for DB use cases.

For instance, we could synthesize entirely new data structures or concurrency control protocols ``just-in-time'' for the currently active workloads with future ADRS frameworks. [make read better] This adaptivity addresses the challenge of increasing hardware and workload diversity, as static, manually-tuned components can no longer effectively cover the expanding design space.

[need to clarify and add more details to this paragraph]
[add topic sentence stating problem clearly] In database systems, semantic guarantees include data consistency, transaction isolation, and integrity constraints. However, developers often leave these rules implicit within application logic rather than declaring them formally. For example, a banking application may encode a balance invariant within an if-then-else block, or a reservation system may rely on specific isolation levels to prevent double-booking. Writing correct application code has been a notoriously hard problem~\cite{}. A promising direction is to automatically infer these semantic requirements to establish the formal constraints necessary for the ADRS framework, enabling the automated search to optimize database queries. [merge with before WITHOUT cutting details] One possible direction is to employ AI agents to identify and formalize implicit constraints. An agent could use static analysis of application source code to identify data invariants or monitor runtime behavior to infer transactional boundaries. For complex semantics, a coding agent interface might allow the developer to disambiguate requirements through interactive dialogue or hypothetical scenarios. The final output would be a set of formal specifications that serve as the ground truth for verifying generated algorithms. It remains to be seen which combination of static analysis, trace monitoring, and developer interaction provides the most robust definitions for autonomous optimization.

Indexes are crucial data structures that accelerate query processing but must operate under limited storage resources, as they take up memory that [might otherwise be used...] [don't some indexs also slow down queries?].

discuss how we can address these two components of the research process to automate how ADRS can be applied.

Precisely define the problem to solve, provide sufficient context, understand related work.

 evaluation objectives and workloads to use. Implement any relevant baselines.

ADRS iterates until the resource budget is exhausted, discovering optimizations that human researchers might overlook.

% Database systems present a unique opportunity for ADRS application. Modern engines consist of highly specialized components, such as query optimizers, buffer managers, and concurrency control mechanisms, that rely on complex, often manually-tuned heuristics. As hardware architectures diverge and workloads become increasingly diverse, manually tuning these components is becoming intractable. Consequently, the community has already explored automated optimization of data systems to maintain performance and efficiency. This work has mainly centered around replaced specific components with learned models~\cite{}, which has seen seen some success but these black-box approaches struggle with high inference overhead and unpredictable worst-case behavior. 

In contrast, ADRS presents a white-box approach to optimizing the \textit{code} of database systems. ADRS frameworks evolves interpretable source code that can be [update following to be the opposite of the three weaknesses of black-box we mention above: audited, debugged, and deployed without additional runtime dependencies. This approach yields robust solutions that avoid the opacity and overhead of neural networks.]
For example, Datadog used evolutionary algorithms to generate code that achieved 10$\times$ higher throughput~\cite{}. By generating code rather than models, ADRS offers flexibility: it can discover generalizable algorithms applicable across different systems (e.g., robust buffer replacement policies) or specialized logic tailored to specific instances (e.g., workload-specific index selections). Moreover, ADRS accelerates the development lifecycle, allowing researchers to identify optimizations that would otherwise require extensive manual design. ADRS frameworks can automate the validation of thousands of candidates to discover solutions that are performant and robust enough for production. For instance, AlphaEvolve discovered a scheduling policy based on CPU and memory residuals that improved Google's fleet-wide utilization by 0.7\%~\cite{}, demonstrating the potential for significant gains in large-scale systems.
Looking forward, we envision extending ADRS optimization to architectural design. Future systems could synthesize data structures or concurrency control protocols ``just-in-time'' for active workloads. As the complexity of the design space grows with increasing hardware and workload diversity, we view ADRS as a crucial tool to ensure high performance for next-generation databases


In contrast, ADRS evolves interpretable source code that can be audited and battle-tested. This approach can yield robust, deployable solutions, as demonstrated by Datadog's use of evolutionary algorithms to achieve 10$\times$ higher throughput~\cite{}. By generating code rather than models, ADRS advances the vision of instance-optimized databases. 
Moreover, ADRS accelerates the development lifecycle, allowing researchers to identify optimizations that may otherwise require extensive manual design and engineering effort. ADRS frameworks can automate the validation of hundreds or thousands of candidates to discover solutions that are performant robust enough for deployment. For instance, AlphaEvolve discovered a scheduling policy based on CPU and memory residuals that improved Google's fleet-wide utilization by 0.7\%~\cite{}, demonstrating the potential for gains on large-scale data systems.

Moreover, we envision extending ADRS optimization to architectural design. Future systems could synthesize data structures or concurrency control protocols ``just-in-time'' for active workloads. As the complexity of the design space grow with increasing hardware and workload diversity, we view ADRS as a crucial tool to ensure high performance for databases.

The LLM is iteratively prompted to generate a candidate solution (e.g., a piece of code), which is then scored within an evaluation environment. This score and the solution are used as feedback to refine the prompt for the next iteration, guiding the search toward better solutions. Unlike prior machine learning applications in databases, which have primarily focused on black-box tuning or replacing specific components, ADRS treats the system as a white-box, enabling it to reason about and directly generate system code. \lma{Maybe add 1-2 sentences about the benefit of white-box optimization.}

Our evolutionary loop collects the necessary data for generating new policies. \accheng{make this the same as previous figure, we are trying to reduce the cardinatlity of the search space here}

While databases can benefit uniquely from ADRS approaches because they have many heuristics that can be optimized, there are a number of uniquely difficult challenges in applying this approach to databases due to their immense complexity. Using an ADRS framework effectively requires the researcher to first complete the two of the hardest parts of the research process: \textbf{problem formulation} and \textbf{evaluation setup}. Problem formulation involves defining the goal and constraints, understanding related work, and providing sufficient context to develop solution. Databases have many different components and intricacies, so optimizing their performance often requires specialized knowledge, which LLMs may not have as context by default. The needed context may not yet exist (i.e., need to run experiments to generate relevant data).
Evaluation setup involves provide system or simulator, defining performance objectives (e.g., workloads and metrics), and implement baselines. For databases, the challenges are around (i) determining the right metrics and workload and (ii) rapid feedback. 
The iterative nature of ADRS frameworks requires rapid feedback and precise context, which conflict with the scale and complexity of modern data systems. Direct evaluation on full database systems is challenging because it can be prohibitively expensive. Each iteration requires recompilation, data loading, and benchmark execution, which can take too long over hundreds or thousands of iterations. To make search feasible, researchers must rely on \textit{simulators}, but this introduces a trade-off: high-fidelity simulators are difficult to build, while low-fidelity simulators risk guiding the LLM toward invalid optimizations. Furthermore, determining the right metrics and workloads to be used for evolution is challenging. Running all workloads on end-to-end metrics may be too expensive but running a subset of workloads with estimation metric may lead to overfitting or fail to optimize full system.

We can treat problem formulation and evaluation setup as evolvable problems to optimize the process of applying ADRS to databases. 

\textit{Co-evolve the world model} to capture the necessary context.

because end-to-end evaluation is too slow and the search space is too big. Evaluation setup in ADRS involves providing a target system or simulator, defining performance objectives (such as workloads and metrics), and implementing baselines. Direct evaluation on a full database is usually prohibitively expensive, as recompilation, data loading, and benchmark execution take too long for each iteration. ADRS frameworks usually must execute many iterations (e.g., tens to hundreds~\cite{}), so the evaluation in each iteration must be \textit{fast} and \textit{accurate}. Moreover, the search space may be too large (e.g., exhaustive query rewrite is combinatorial problem), so not feasible to run that many iterations.


but simulating database behavior is notoriously hard due to the immense complexity of these systems. This presents a fundamental challenge: high-fidelity simulators are difficult to construct, while low-fidelity ones risk guiding the LLM toward invalid optimizations. [make sentence more concise] simulating database behavior is notoriously hard due to the immense complexity of these systems; intricate interactions between individually optimized layers create a noisy environment that is difficult to capture accurately. 

Second, one can model end-to-end performance (e.g., by train a learned model~\cite{}), mapping system signals to target metrics. However, building such models is expensive and requires extensive training data. Third, evaluation can be accelerated by running only a subset of workloads, though this sacrifices accuracy for speed [add something about how to select subset of workloads manually is difficult, risk over overfitting]. Finally, for problems with a defined set of optimization techniques, one can limit the search space to a subset of these methods. While this reduces the number of required iterations, it must be done carefully [mention manual analysis] to avoid missing potential performance gains.

There are several standard techniques to address the challenge of evaluation but they each come with their own difficulties. First, we can build a simulator, but this introduces a fundamental trade-off: high-fidelity simulators are difficult to build, while low-fidelity simulators risk guiding the LLM toward invalid optimizations. Building simulators of databases is known to be a hard problem because databases have \textit{immense complexity}. These systems comprised of multiple, intricate layers that are usually individually optimized. The interactions between these components create a vast and noisy environment that is hard to simulate and accurately capture end-to-end behavior.  
Second, we can train a model to predict end-to-end behavior. This allows us to map some signal to the metrics we care about. Building this model can be expensive and require extensive training data. Many standard ML techniques here.
Third, we can run only a subset of workloads to enable faster evaluation. This also has a tradeoff between speed and accuracy. 
Fourth, for problems which have a limited set of optimization techniques, we can just try out a subset of these techniques. This would reduce the number of iterations of evaluation required but must be done carefully to prevent missing potential wins.

There are several standard techniques exist to mitigate the cost of evaluation, yet each introduces significant trade-offs and [reword to read better:] require lots of manual labor. 

significantly [reword to sound more genereal, don't focus on manual effort] reduce the manual effort required to adapt ADRS to complex database systems.

Concretely, we leverage the evolutionary loop to not just to discover solutions but also to generate better simulators, models of E2E behavior, workload subsets, and optimization technique subsets. By treating evaluation as an evolvable problem, we optimize the process of applying ADRS to databases.

To realize this potential in practice, there are a number of challenges in applying this approach to databases. While recent work has already demonstrated the promise of ADRS on a number of different systems problems~\cite{}, databases are especially challenging due to their complexity and large search spaces.

The iterative nature of these framework requires rapid feedback and precise context, which conflict with the scale and complexity of modern data systems. Direct evaluation on full database systems is challenging because it can be prohibitively expensive. Each iteration requires recompilation, data loading, and benchmark execution, which can take too long over hundreds or thousands of iterations.
\begin{itemize}
    \item \textbf{Evaluation framework.}  To make search feasible, researchers must rely on \textit{simulators}, but this introduces a trade-off: high-fidelity simulators are difficult to build, while low-fidelity simulators risk guiding the LLM toward invalid optimizations.
    \item \textbf{Evaluation metrics and workloads.} Running all workloads on end-to-end metrics may be too expensive but running a subset of workloads with estimation metric may lead to overfitting or fail to optimize full system. We need a way to 
\end{itemize}

% While the performance problems are usually well-defined for databases (e.g., optimize query latency, reduce I/O utilization, etc.), 


\accheng{evaluation is challenging
DBs are complex
one way is to evaluate every change on full system but this is too expensive
We have simulator and deploy solutions on full system and then evolve simulator
Making evaluation feasible
Good evaluator is fast, high-fidelity: one instantiation of cascading simulator
This is a general pattern
}

\accheng{
67 choose 4
}

% Evaluation is challenging on databases due to their complexity. Each modification on the full system requires a re-compilation, loading database state, and execution of benchmarks. This makes each iterative loop too expensive, so the standard solution is to evaluate solutions on a \textit{simulator} to make evaluation feasible. As such, a key challenge in using ADRS is building a fast and high-fidelity simulator. 

% 2. Lack of context

% 3. Workloads

We describe approaches to addressing each of these challenges in the following sections, which center on use cases in applying ADRS to database performance problems. 

present insights for automating these stages of the research process. Our key insight is that we can co-evolve the evaluator setup in applying ADRS to databases. 

% \section{Insights in Applying ADRS for DBs}
% \label{sec:eval}

% We summarize insights in applying ADRS for databases. We use several use cases, spanning different DB components, to illustrate these insights.

\begin{itemize}
    \item \textbf{Case study \# 1: buffer cache optimization.} 
    \item \textbf{Case study \# 2: index selection optimization.} 
    \item \textbf{Case study \# 3: query rewrite optimization.} 
\end{itemize}

it is [make read better:] currently very difficult to apply these frameworks due to end-to-end evaluation challenges. 
[make flow better, add transition:] ADRS frameworks are only as good as the evaluators guiding them. 

because they are complex and the search space for most problems is very large.

we use Cursor to evolve a simulator that balances execution speed with PostgreSQL fidelity.
we demonstrate how to co-evolve a simulator that balances execution speed with fidelity to PostgreSQL. 
This process relies on our core insight: calibrating against multiple ground-truth baselines is essential for achieving simulator fidelity while preserving the expressivity required for complex policies.

PostgreSQL's buffer manager observes low-level state like usage counts and dirty flags but lacks global context, specifically active scan progress, required for intelligent eviction. This metadata resides in the query executor rather than the buffer layer, so the simulator excluded the state necessary to re-discover strategies like PBM-Sampling which rely on future access estimates. However, when we allowed the AI to relax structural constraints without providing context from existing baselines, it generated simulators that permitted unrealistic techniques, such as full buffer pool scans or expensive computations, that were impossible to implement in the full system.

\textbf{Evaluator.} As described in the pervious section, the simulator models PostgreSQL's buffer manager with realistic I/O latencies based on typical NVMe SSD specifications: 100$\mu$s for random reads, 20$\mu$s for sequential reads, and 200$\mu$s for synchronous dirty page evictions. We test on four workloads: TPC-H (analytical queries with large sequential scans), TPC-C (transactional workloads with random point lookups and frequent writes), CH-benchmark (hybrid OLAP/OLTP), and mixed synthetic workloads. 
It reports latency scores, hit rates, dirty eviction rates, and per-workload access pattern statistics (sequential vs. random, read vs. write ratios).

\textbf{Objective and constraints.} We optimize latency score, which is inversely proportional to average I/O wait time, across the database workloads. Policies must maintain buffer management invariants ( proper locking, reference counting) to be considered valid.
\textbf{Solution generator and selector.} We run OpenEvolve with Claude Sonnet 3.5 for 85-100 iterations. The search completes in about eight hours and costs less than \$30.

how we apply an ADRS to our evolved simulator to automatically discover novel caching policies. We first present the ADRS setup (including benchmark workloads, optimization objective, and evolution configuration) and results. We then describe our results on Postgres with the best evolved policy. 

\textbf{Evaluator.} We use a trace-driven simulator that models PostgreSQL's buffer pool with realistic I/O costs (100$\mu$s for random reads, 200$\mu$s for dirty page evictions). We test on industry-standard benchmarks: TPC-H (analytical queries), TPC-C (transactional workloads), CH-benchmark (hybrid OLAP/OLTP), and mixed workloads.
Each configuration uses 256MB buffer pools with 4x data-to-buffer ratios matching realistic deployments.
The evaluator checks syntax and interface compliance, verifies proper lock handling, and tests valid solutions on the benchmark suite.
It reports latency scores, hit rates, and dirty eviction percentages. Per-workload statistics and access pattern characteristics (sequential vs. random, read vs. write ratios) are included to provide richer context.

\textbf{Objective and constraints.} We evaluate latency score (inversely proportional to average I/O wait time) across a range of database workloads. We require that all buffer management invariants be maintained (proper locking, reference counting) for an algorithm to be considered valid.

\textbf{Solution generator and selector.} We run OpenEvolve with Claude Sonnet 3.5 for 85-100 iterations. The search completes in about eight hours and costs less than \$30.

\accheng{add pseudocode comparison}
\accheng{add figures?}

\accheng{figure on evolving simulator
look at paper WebEvolver: evolve model based on real-world rollouts to predict I have this trace of actions, one of the reasons is to do it faster}

\accheng{if there are different metrics, the simulator will change

simulator can be optimized wrt to system and metric

can we add this as a proof point, organically emerging from these techniques, confirmation of this

nice data point}

\accheng{
Insight: outcome of the evolution is not only the algorithm itself but also the history/data/analyses of evolution
Leverage experience for future workloads/queries and use that to enhance algorithm search
}

\accheng{explore vs. exploit: not on policy itself but the 

high level lesson: run on a policy, get the decision, examine the result and based on this, run additional verification to get more signal on policy

exploratory evaluator: extended evaluator

build a comprehensive evaluator and best use evaluation result, even within policy itself
}

\accheng{insight: how to use the history?
generate data based on optimization space
try to create a model: world model
want to create model that given a queyr, what rules should i apply? want to predict what is the result
want to make decision without ful system eval

present a figure about what
}

For example, if we attempt to directly apply an existing ADRS framework on Postgres for optimizing buffer cache replacement policy, we would need to make a code change in C++, recompile the database (X mins), load data into database for standard benchmarks (e.g., Y mins for TPC-H SF=10), and run the set of queries (e.g., Z mins for workload).

For example, identifying the optimal set of rules for query rewrites is a combinatorial problem. When we try applying ADRS directly, it is ineffective because the framework searches through many uneffective rule combinations.

This has implications for speed, fidelity and generality, as a database researcher must decide how to navigate these trade-offs in developing a suitable evaluator for ADRS frameworks.For speed, if evaluation is too slow/expensive on full system, standard practice is to build a simulator. However, building a database simulator is hard: intricate interactions between individually optimized layers create a noisy environment that is difficult to capture accurately. High-fidelity simulators are difficult to build, while low-fidelity simulators risk guiding the LLM toward invalid optimizations. For fidelity, there is work on modeling end-to-end performance via proxy metrics. This is generally challenging because databases are complex. For search space, can limit to subset of optimization techniques but need domain expertise and is time-consuming. For generality, can use subset of workloads but risks overfitting and losing useful signal. Running all workloads on end-to-end metrics may be too expensive but running a subset of workloads with estimation metric may lead to overfitting or fail to optimize full system.

These challenges can be as hard as coming up with the solutions themsevles. To address this, we present our co-evolutionary approach in the next section to automate parts of the evolution process to more effectively apply ADRS.

There are techniques to achieve speed, fidelity, generality, and coverage but each comes with their own tradeoffs in the database setting. 

- optimization goal
- technique
- insight
- result

[need transistion, make flow better, something like since different problems have different requirements...but make sound better] Different optimization problems present distinct bottlenecks. Optimizing the buffer cache policy requires simulation because need to run on large workloads/benchmarks. Query rewrite can run directly on full system but the challenge is the combinatorial search space of possible rules. 
[make read better, flow well from previous text, flesh out more as necessary] 
As such, rather than proposing a single monolithic architecture, we demonstrate how to tailor the ADRS loop to the specific challenges of different performance problems. Concretely, we present three case studies, spanning different database components.

previously discussed for making evaluation feasible for ADRS. [need to emphasize and explain this point more, different optimization problems have different challenges around speed, generality, fidelity, coverage. give some examples from our case studies.] Since different techniques apply to different problems, we demonstrate this approach over three distinct database performance problems. 

Achieving speed, fidelity, generality, and coverage is hard for databases due to their complexity

\accheng{frame as speed vs. other three properties?}
While standard techniques exist to address speed, fidelity, generality, and coverage, each introduces significant trade-offs in the database context. (1) To improve speed, researchers often employ simulators when full-system evaluation is prohibitively expensive. However, building a database simulator is notoriously difficult, as intricate interactions between layers create a noisy environment that is hard to capture, leading to a trade-off where high-fidelity models are complex to build while low-fidelity ones risk guiding the LLM toward invalid optimizations.
(2) To approximate fidelity, a well-known approach is model end-to-end performance via proxy metrics. However, accurately capturing the behavior of complex database systems through simplified models is challenging and often fails to reflect true performance. 
(3) To balance generality with evaluation speed, we can accelerate the process by running a subset of workloads, but this risks overfitting and losing useful signals, as optimizing for a narrow subset may not translate to the full system. 
(4) Finally, to maintain sufficient coverage while managing the vast search space, one can limit exploration to a subset of optimization techniques. However, this approach requires domain expertise to avoid discarding critical opportunities and is time-consuming to tune manually.

\accheng{subsection with case studies is confusing, 3.0/4.0/5.0 should have bolded phrases: this is the case study where we show this insight, this is the solution, point to 3.2, etc.

not clear that 3.2 is part of the case study

Case Study \#1: --> put these somewhere around header of S3
}

Context Management: Construct What You Need

Workload Selection: Hone the Signal

% \lma{maybe add ``such as in XX, YY, and ZZ tasks.''}

While databases contain numerous algorithms suitable for ADRS optimization, applying this approach is particularly challenging due to the prohibitive cost of evaluating candidate solutions and the massive search space of many problems. Evaluating performance in this domain is inherently complex compared to other software systems. Databases are stateful, highly workload-dependent, and characterized by extensive cross-component coupling, meaning a modification to one system component often impacts the entire engine. Furthermore, leveraging standard database cost models as an evaluation proxy may not always reflect end-to-end performance. However, performing a direct evaluation on a full database during the iterative ADRS search process is often infeasible. Databases are stateful, demanding time-consuming data reloads between runs to ensure reproducible measurements. Recompilation, data loading, and benchmarking introduce significant latency per iteration, and this overhead is prohibitive since ADRS frameworks typically require tens to hundreds of iterations to converge~\cite{}. They are also highly workload-dependent, requiring candidate solutions to be tested against diverse, representative query mixes rather than isolated benchmarks. Beyond evaluation costs, the search space for many database problems is combinatorial (e.g., determining the optimal set of SQL query rewrite rules~\cite{}), making exhaustive exploration impossible within a reasonable timeframe.

Although databases contain numerous algorithms suitable for ADRS optimization, applying this approach is particularly challenging in this domain due to the prohibitive cost of end-to-end evaluation and the large search space of many problems. Direct evaluation on a full database is often infeasible, as recompilation, data loading, and benchmarking introduce significant latency per iteration. This overhead is prohibitive because ADRS frameworks typically require tens to hundreds of iterations to converge~\cite{}. 

Moreover, the search space for many database problems is combinatorial (e.g., determining the optimal set of SQL query rewrite rules~\cite{}), making exhaustive exploration impossible within a reasonable timeframe.

While this has more recently evolved to include auto-tuning and learned components, these methods operate primarily as [clarify what black-box means, treat systems as black box] black-box optimizers. [mention prior work focused on knob tuning or replacing specific components with learned models but these are had to run in practice due to high inference overhead \accheng{at run-time}, unpredictable worst-case behavior, and need for specialized ML infrastructure.] [add transition, make flow better]

we can leverage LLMs to generate executable code by modifying system internals directly. 

This approach yields high performance algorithms for tasks like buffer management, index selection, and query rewrites, while maintaining the low overhead and predictability of native compiled code.

With the advent of Large Language Models (LLMs), we observe a phase shift toward white-box optimization, where models generate executable code to modify system internals directly for superior performance for tasks such as for buffer management, index selection, and query rewrites. A new class of AI-driven techniques is poised to automate this process.

. This white-box approach 
Unlike prior machine learning applications in databases that rely on opaque models, 

While databases contain numerous algorithms suitable for ADRS optimization, applying this approach is challenging due to the prohibitive cost of evaluating candidate solutions and the massive search space of many problems. Evaluating performance in this domain is inherently difficult compared to other software systems because databases are stateful and complex, making direct evaluation prohibitively slow.  The overhead of recompiling, loading data, and benchmarking during each ADRS step makes the hundreds of iterations required for convergence infeasible~\cite{}. While standard cost models offer a faster proxy, they frequently fail to accurately reflect end-to-end performance due to the complex interactions between different database components.
Furthermore, performance is highly workload-dependent, requiring candidate solutions to be tested against diverse query mixes rather than isolated benchmarks.
Beyond evaluation costs, the search space potential optimizations is often combinatorial (e.g., determining the optimal set of SQL query rewrite rules~\cite{}), making exhaustive exploration impossible within a reasonable timeframe.

[theme of techniques is unclear
lacking structural guidance to tie these techniques together
we want to setup to later answer question: Is there something about ADRS that enables us to make search space smaller and evaluation faster that was not possible before?
fix paragraph, make read better and flow better. theme should be: There are different techniques to reduce the evaluation cost but they are problem specific.]
To overcome [what challenges? be specific] these challenges, there are different techniques to reduce evaluation and search costs, but they are problem-specific and typically require considerable manual effort. For instance, when optimizing localized components like buffer managers, one method is to employ simulators to approximate behavior without running the full system~\cite{}. However, constructing high-fidelity simulators is notoriously difficult while low-fidelity alternatives risk misleading the optimization process. Alternatively, for physical design tasks like index selection, we can model end-to-end performance (e.g., via learned cost models~\cite{}), but this requires significant effort in feature engineering and data collection. When dealing with large benchmarks, evaluation can also be accelerated by running only a subset of the workload~\cite{}, but manually selecting representative queries is challenging and risks overfitting, which limits the solution's applicability. Finally, limiting the search space to a subset of optimization techniques can reduce the number of iterations needed (e.g., ~\cite{}) but requires expert analysis to ensure critical opportunities are not excluded~\cite{}.

Consequently, the community has explored automated optimization of data systems to improve performance and efficiency. Prior work has primarily centered around two approaches:  

\accheng{Xiao + Aaron, any comments on industry impact?}
As hardware and workload diversity grows,

While prior work demonstrates that ADRS frameworks excel at Solution Generation, the Evaluation Setup stage currently remains a critical bottleneck in realizing the benefits of ADRS optimization. The automated discovery by ADRS frameworks relies on robust evaluators that can provide fast, accurate, and detailed feedback. ADRS frameworks are only as effective as the evaluators guiding them. Automating evaluation is critical to the long-term success of ADRS. but developing good evaluators is especially challenging for databases.

Historically, spending hours or days to evaluate a single human-designed algorithm was acceptable. However, LLMs can now generate tens to hundreds of novel ideas in minutes. This shift makes the traditional evaluation pipeline the primary bottleneck. Databases are especially challenging and have high evaluation costs due to their complex and stateful nature. For example, directly applying an existing ADRS framework to optimize PostgreSQL's buffer replacement policy would require modifying C++ source code, recompiling the database (X mins), loading data for standard benchmarks (e.g., Y mins for TPC-H SF=10), and executing the full workload (e.g., Z mins). A single iteration could take over X+ minutes. Running tens to hundreds of iterations through a full PostgreSQL benchmark would take days to weeks, making convergence prohibitively slow.

When the problem space is large, [not forced to process, something like naively applying ADRS...make read better] the evaluator is forced to process an overwhelming number of candidates to achieve sufficient coverage. [can combine with previous sentence] Applying ADRS directly to these problems often becomes ineffective, as the framework wastes computational resources searching through vast numbers of ineffective rule combinations. Consequently, the system struggles to identify and focus on the most promising regions of the search space before exhausting its evaluation budget is prohibitively expensive.

When applying ADRS directly, the framework often becomes ineffective as it wastes resources (e.g., searching through vast numbers of ineffective rule combinations), struggling to identify and focus on the most promising regions of the problem space.

[make paragraph read better and flow well. add transitions between sentences as needed. ]
Challenges above exist regardless of ADRS so there have been some standard techniques developed to accelerate evaluation. these techniques are good, they navigate  tradeoff between evaluation speed and quality. evaluation quality means fidelity to e2e performance on full system and convergence [elaborate a bit more]. traditionally, these techniques are applied manually to figure out where in tradeoff to sit. [frmae the following techniques instead as describing them and how they navigate tradeoff rather than negative connotation "sacrifices", just emphasize difficult]
(1) Researchers often employ simulators to avoid expensive full-system evaluation. However, this sacrifices \textbf{fidelity}. Accurately modeling database internals is difficult as complex interactions between different components create a noisy environment that is hard to capture. Low-fidelity models risk guiding the LLM toward invalid optimizations.
(2) Similarly, relying on proxy metrics and using a model to predict end-to-end behavior favors speed over \textbf{fidelity}. Simplified metrics (e.g., cost estimation rather than actual query latency) are easier to measure but often fail to reflect true performance in complex systems.
(3) To improve speed, one can run a subset of workloads. This approach can compromise \textbf{fidelity}: optimizing for a narrow subset risks overfitting and the loss of signals required for the full system.
(4) Finally, limiting exploration to a subset of optimization techniques can reduce the number of iterations needed in the evolution loop but reduces \textbf{coverage}. This technique requires significant domain expertise to ensure critical opportunities are not discarded. [read better and flow well, connect to previous text]
These techniques are important because ADRS requires fast eval, but ideally we could have a way to automate their application.

[rephrase this whole sentence, sounds bad and too dramatic:] The advent of LLMs fundamentally alters this dynamic. [merge with following: ] This capability allows us to use AI to intelligently and automatically navigate the non-trivial trade-off between speed and fidelity.
Since these models can rapidly synthesize executable code, they can generate the parts of evaluators themselves just as they can generate solutions. 

[make read better and keep style as other text, flow well] The advent of LLMs fundamentally alters this dynamic. [doesn't make sense: ] Now that generating code is cheap, we can use AI to intelligently and automatically navigate this non-trivial trade-off between speed and fidelity by automating the construction and refinement of the evaluation environment itself. In the next section, we present co-evolutionary approach to automate key parts of the evaluation process to more effectively apply ADRS to databases.

In this case study, our goal is to evolve a new cache eviction algorithm that improves throughput and latency. The buffer manager uses this policy to determine which database pages remain resident in the limited memory pool, making eviction decisions that minimize costly disk I/O. Formally,
\begin{definition}
(Cache State). A cache state is a set of pages $P$ currently resident in memory, where $|P| \leq N$ and $N$ is the fixed capacity of the buffer pool. Each page $p \in P$ is associated with metadata $M_p$ (e.g., usage count, dirty flag).
\end{definition}

The cache state is determined by the eviction policy:
\begin{definition}
(Eviction Policy). An eviction policy is a function $f: (P, r) \rightarrow p_{victim}$ that, given the current cache state $P$ and a request for page $r \notin P$, selects a victim page $p_{victim} \in P$ to evict.
\end{definition}

Our optimization goal is to minimize the total I/O cost over a sequence of requests $R = \{r_1, r_2, \dots, r_m\}$, where cost is incurred for each miss ($r_i \notin P$). \accheng{need to check this}

methods that can automatically prune search spaces and accelerate evaluation setup.

has traditionally relied on human-driven development of specialized algorithms. This process requires significant manual effort and is slow to adapt to emerging workloads and hardware. To automate performance optimization, recent research integrates machine learning (ML) into data systems. These methods typically treat the underlying engine as a black box, focusing mainly on knob tuning or replacing specific components with learned models that perform inference at query time. However, these learned approaches are difficult to deploy in practice due to high run-time inference overhead, unpredictable worst-case behavior, and the need for specialized ML infrastructure.

We initially applied OpenEvolve to generate query rewrite policies but found that this strategy plateaued quickly. Our evolutionary loop compiled LLM-generated variants, benchmarked them against TPC-H queries, and returned a score based on cost estimation for the next iteration. However, this approach failed because the LLMs did not have sufficient context on what rules worked well for specific queries. Unlike R-Bot, which performs inference per-query, this approach attempted to evolve a single global policy to handle all queries simultaneously. This overwhelmed the model with conflicting signals across the workload, trapping the evolution in a local optimum unable to beat the SOTA baseline.

\textbf{Building our world model: getting the right data.}
Our core insight to evolving an effective policy is that we need to construct the missing context, specifically the ground truth on rule efficacy. Since this data does not exist in the LLM a priori, we designed an autonomous evolution loop to actively generate it. We leverage the AI to orchestrate targeted data analysis experiments, using the resulting empirical feedback to learn and generate high-performance rewrite policies.

We implement an autonomous evolution loop inspired by OpenEvolve:
\begin{itemize}
    \item \textbf{Phase 1: Ground truth collection.} At each iteration, the \textit{Searcher} component executes an adaptive search plan formulated by the AI agent based on prior feedback, targeting specific queries (within a training set) and rule combinations. It runs these rule set permutations on PostgreSQL and records their execution latencies. While finding the optimal rule set is NP-Hard, we limit the search space by constraining permutations to structural templates (e.g., pre-processing $\rightarrow$ main transformation $\rightarrow$ post-processing) and filtering invalid rules using their static matching functions. This process generates a ground truth dataset mapping specific query features to performant rule sets.
    \item \textbf{Phase 2: Pattern analysis.} Next, the \textit{Analyst} component correlates performance wins with query structure. It extracts discriminative features (e.g., \texttt{hasSelfJoin}, \texttt{joinDepth}) and identifies conditions under which specific rule combinations lead to better performance. This phase produces pattern hypotheses (e.g., ``If \texttt{hasScalarSubquery}, apply \texttt{FILTER\_SUB\_QUERY\_TO\_CORRELATE}'') and search directives to guide the next round of testing.
    \item \textbf{Phase 3: Implementation.} The \textit{Implementer} component synthesizes these patterns into a custom rewrite policy in Calcite's \texttt{HepPlanner}. We validate the new optimizer on a hold-out set; if regressions occur, the system performs root cause analysis and feeds new constraints back into Phase 2. 
    \item \textbf{Phase 4: Verification and refinement.} To ensure robustness, the system validates the synthesized code against the full training set and a hold-out test set. If performance regressions are detected, the loop triggers a refinement cycle: the Analyst investigates the failure cases, identifies any ``anti-patterns'', and generates tighter constraints to patch the rule selection logic. This self-correcting mechanism iterates for a specified number of iterations or until the policy achieves zero regressions.
\end{itemize}
The final output is an optimized query rewrite policy in Calcite that uses feature patterns of input queries to deterministically decide which rules to apply. This design enables the database to achieve the performance benefits of expensive offline analysis with negligible runtime overhead ($<1$ms).


We construct a domain-specific world model~\cite{} for optimizing SQL query rewrites. We find that applying existing ADRS frameworks are insufficient for this problem due to the lack of empirical data on effective rule combinations. To address this, we leverage our key insight to construct the missing context where necessary for generating effective solutions. By applying the AI in an evolutionary loop to determine what data is needed and gather it through  targeted experimentation, we enable the discovery of policies that exploit these findings for better performance.

[update sentence: ] We construct a domain-specific world model~\cite{} for optimizing SQL query rewrites. [repetitive, read better, flow better] We find that applying existing ADRS frameworks are insufficient for this problem due to the lack of empirical data on effective rule combinations. 
To address this, we leverage our key insight that evaluating rule combinations across the entire workload is intractable, requiring us to dynamically co-evolve the subset of queries and rules being evaluated. By deploying the LLM in an evolutionary loop to systematically gather data through targeted experimentation, we generate the missing empirical context necessary to discover high-performance rewrite policies.

In this section, we address the challenge of providing sufficient context for ADRS problem-solving on databases. General-purpose LLMs often fail in database optimization tasks due to a lack of specialized knowledge, leading to hallucinations or ineffective solutions. To address this, we construct a domain-specific world model~\cite{}, i.e., a predictive simulator that approximates database behavior and feedback. Our core insight is that we should ``construct the context you need'': when direct access to the underlying problem state is limited, we co-evolve the world model to capture the system dynamics and guide the agent. 

\section{OLD Intro}

\accheng{here are challenges applying ADRS to DBs
challenges are more significant (not necessarily unique) because of DB characteristics...}


\accheng{lack of concrete example throughout
running example: maybe Meta three layers
too fluffy right now, need more evidence
very hard to convince without results

wasn't convinced about the problem: what about the self-driving DBs?
need to layout why the existing approaches fail

works in well-defined silos: what does the search process look like?
discussion of why uniquely challenging is good

compared to OS or HW, DB has already done learned policies for DB
making it sound like learned policy for DBs never done
How have they been able to do so?
The existing challenges with DBs (stateful, complexity) are there whether or not we are applying AI 
}

The design of high-performance database systems has traditionally relied on the meticulous, human-driven development of sophisticated heuristics and algorithms. While this has more recently evolved to include auto-tuning and learned components, the discovery of novel algorithmic approaches has remained a manual endeavor. A new class of AI-driven techniques is poised to automate this process.

This new approach, called as AI-Driven Research for Systems (ADRS), has begun to show promising results in automated algorithm discovery, finding solutions that match or exceed the performance of state-of-the-art, human-designed solutions. 
\begin{itemize}
    \item For example, when applied to caching, an ADRS found an algorithm that beat the best existing baseline by [X\%]. 
    \item Unlike prior machine learning applications in databases, which have primarily focused on black-box tuning or replacing specific components, ADRS treats the system as a white-box, enabling it to reason about and directly generate system code.
    \item An ADRS framework operates by using a Large Language Model (LLM) in a feedback loop. The LLM is iteratively prompted to generate a candidate solution (e.g., a piece of code), which is then scored within an evaluation environment. This score and the solution are used as feedback to refine the prompt for the next iteration, guiding the search toward better solutions. 
\end{itemize}

Despite this promise, applying ADRS to database systems is uniquely challenging because these systems are complex and must satisfy a wide range of operational guarantees.
\begin{itemize}
    \item First, databases are \textit{stateful} systems that must uphold a range \textit{correctness guarantees} across state changes while simultaneously optimizing for varied and often conflicting \textit{performance objectives}. Formulating the optimization goals by specifying correctness constraints and defining workload-dependent performance goals constitutes a significant challenge in practice.
    \item Second, databases have \textit{immense complexity}. These systems comprised of multiple, intricate layers that are usually individually optimized. The interactions between these components create a vast and noisy search space that is difficult to model accurately. For instance, the end-to-end performance of a novel concurrency control protocol arises from its interactions with the transaction manager, logger, and buffer pool. This intricate web of dependencies makes building a fast, high-fidelity evaluation framework a primary obstacle, as simple component-level tests are often insufficient to predict end-to-end system impact.
\end{itemize}

Thus, realizing the full potential of ADRS for databases hinges on solving these two fundamental challenges: (i) formulating the problem precisely and (ii) constructing sufficient evaluation frameworks.

First, precisely formulating the problem is a key challenge in applying ADRS to databases. 
\begin{itemize}
    \item This formulation involves define correctness constraints by automatically extracting implicit application semantics, such as data consistency, transaction isolation, and integrity constraints, which define the space of valid solutions. 
    \item We also need to specify performance objectives, which involves articulating the complex, often dynamic trade-offs between competing metrics like throughput and latency. 
    \item Finally, we need the right abstractions and to provide the appropriate context to ground the search, bridging the gap between a general-purpose LLM and the specialized domain of database systems.
\end{itemize}

Second, building evaluation frameworks for ADRS represents a critical bottleneck. 
\begin{itemize}
    \item The need for rapid feedback to guide the automated search conflicts with the inherent difficulty of accurately simulating complex database systems. We propose addressing this tension with a \textit{spectrum of simulation} that allows ADRS to trade off speed and accuracy.
    \item Furthermore, ADRS frameworks offer the opportunity for end-to-end optimization across the database stack. This requires a \textit{hierarchical framework} capable of managing competing objectives across different system components and reasoning about global performance trade-offs.
\end{itemize}

We demonstrate the initial success of our problem formulation proposal with LLM-Txns case study...

% Furthermore, a natural consequence of ADRS is that there should be a broader shift in the database community to building that are more predictable. Prior design decisions may have emphasized performance, efficiency or resilience at the cost of predictability but now, ADRS can address performance so systems should be more predictable.

In this paper, we argue that fully adopting AI-Driven Research for Systems (ADRS) represents the next fundamental shift in database systems design. We believe this AI-driven methodology is a compelling approach that can move the field beyond human-written heuristics toward automatically discovered, high-performance algorithms. Realizing this vision, however, requires overcoming challenges that we detail in this paper. In the rest of the paper, we  explores these challenges, describe potential solution, and discuss the research implications of this new paradigm.

the hardest parts of the research process, namely \textbf{problem formulation} and \textbf{evaluation setup}, remain unaddressed by ADRS and are the main barriers to effectively applying these frameworks. 
Problem formulation involves understanding related work, defining goal and constraints, providing sufficient context to develop solution.
Evaluation setup involves defining objective, constraints, workloads, provide system or simulator, and implement baselines.

Problem formulation is the key task of researchers. LLMs have shown limited success in helping here. We focus on providing sufficient context, as databases often require specialized knowledge.
\begin{itemize}
    \item \textbf{Context.} While LLMs trained on broad corpus of knowledge, they may not have information about a specific query or need some way to retrieve this knowledge. There has been extensive work on RAG retreival but the needed context may not yet exist (i.e., need to run experiments to generate relevant data).
\end{itemize}

\accheng{need a roadmap of how to lay out these sections}
\accheng{what is the thesis? ADRS opens up exciting research opportunities
we have preliminary results to show ADRS is effective for DBs but there are lots of other problems
take the transformatory angle: this changes how we can do research and here are all the cool things
Goal is to define the right problems
}

% Databases need custom algorithms. Manual design is too slow.
% Runtime ML is impractical (overhead, unpredictability).
% ADRS (offline LLM code evolution) solves the runtime overhead but requires a fast, automated evaluation loop.
% Databases are too heavy to evaluate natively inside a fast loop, and manually building fast proxy evaluators defeats the purpose of automation.
% Our insight: We can use ADRS to co-evolve the evaluation proxy alongside the solution itself.
% We prove this works across three distinct, classic database problems

% \accheng{none of learned systems used at scale, mention the challenges: in usual use, these systems had extreme challenges so they were not practical

% we think we can make it practical

% bring up some of 2.2 challenges}

However, traditional approaches to optimizing system performance rely on manual optimization [make this also account for ML for systems work, which stil requires human to manually train model, etc.], which cannot keep up with the current pace of things.

[make good topic sentence]
We believe ADRS will eventually become the norm for performance research  because of [fill in what it enables]
[make read better and flow well: call back to widening gap we mentioned before. as workload and hardware complexity grow, already outpacing human engineering capacity. the way to address this is by replacing manual optimization with Automated algorithm discovery. connect with below and merge repeitive text as needed]
Previously, the scale of solution generation and evaluation was constrained by the time required for researchers to manually conceptualize and implement each new approach (e.g., replace this component with a learned model). LLMs can overcome this bottleneck by rapidly generating and evaluating hundreds of novel solutions, unlocking a level of optimization that was previously unattainable.
[we need to advance ADRS as it will define how the next generation of high-performance databases are built and optimized.]

[make flow better, read better, add content to paragraph expressing following:
topic sentence: we believe ADRS is rapidly becoming the norm.
ADRS will eventually become the norm
People need to believe this will be the future to care about this paper

need to sell ADRS more

we think the future of DB research is ADRS

restating what we said previously: ADRS will eventually become the norm
People need to believe this will be the future to care about this paper
]

[make flow better, read better, add paragraph expressing following:
we believe ADRS is rapidly becoming the norm.
ADRS will eventually become the norm
People need to believe this will be the future to care about this paper

need to sell ADRS more

we think the future of DB research is ADRS, this is what's blocking that dream

need to layout vision about how DB research will be done in 5/10 years
1. most DB researchers don't know about ADRS
2. people don't know what it will evolve into
b/c people don't understand this dream yet, we should add some of the argument from our other paper

need sense of "upending systems research"

needs 1-2 paragraphs restating what we said previously: ADRS will eventually become the norm
People need to believe this will be the future to care about this paper
]

[this whole paragraph says a couple of points multiple times in different ways. just say main points once and make the logical flow better]
Despite this transformative potential, the current bottleneck in applying ADRS is the [not eval but eval setup, make read better] evaluation phase. [too wordy, combined sentences without cutting content, be more concise and make read better] Evaluation is fundamental to discovering high-quality solutions. Crucially, the success of this approach depends on a robust, user-provided \textit{evaluation setup} to accurately measure the performance of candidate solutions. Ultimately, a discovered solution is only as good as its evaluator, as these measurement components provide the critical feedback signals required to guide the LLM's search process. Effective ADRS pipelines require robust evaluators that return fast, accurate, and highly detailed performance signals. If the systems community can solve this evaluation bottleneck, ADRS will unlock unprecedented capabilities, such as synthesizing custom query optimization rules from scratch, discovering highly specialized data structures, and automatically rewriting core execution engines for new hardware architectures without human intervention. While recent research focuses on improving the solution generation capabilities of ADRS~\cite{}, the evaluation pipeline remains a manual and prohibitive endeavor.

[flesh out next paragraph:
the current bottleneck in applying ADRS is evaluation. say evaluation is fundamental to discovery good solutions. it's already been shown that the solution discovered as only as good as the evaluators becaause evaluators provide the feedback to guide search. need robust evaluators that return fast, accurate, and detailed signals. 
if we can solve evaluation, we get even more amazing things with ADRS (say what these amazing things are concretely).
]
Crucially, the success of this approach depends on a robust, user-provided \textit{evaluation setup} to accurately measures the performance of candidate solutions.
While recent research focuses on improving the solution generation capabilities of ADRS~\cite{}, the evaluation pipeline remains a manual endeavor

[frame parts logically. the components to evaluation are 
workload
search space of solutions
system (modeling = not running on system, running a simulator
run in real system)
we should present techniques as so]
balance evaluation speed and quality. Common approaches include building hand-crafted simulators~\cite{}, training learned performance models~\cite{}, executing representative workload subsets~\cite{}, and artificially restricting the search space~\cite{}. However, directly applying these techniques to ADRS is insufficient. Implementing these workarounds requires massive manual effort and domain expertise. In fact, engineering a high-fidelity simulator, training an accurate performance model, or carefully tuning a workload subset is often as difficult as solving the underlying system problem itself. Ultimately, relying on human intuition to construct these evaluation shortcuts defeats the core purpose of an automated discovery pipeline.

Why Evaluation is the Hardest Part of Applying ADRS to Databases

but...[fill in]. However, [sounds awk, make read better: their reliance on manual application] creates a crucial bottleneck for database systems. [merge two sentences]
Historically, navigating the trade-offs introduced by these techniques required significant effort, often proving as difficult as developing the solutions themselves.
Traditionally, researchers apply these techniques manually, relying on intuition to determine exactly where on the trade-off curve their evaluator should sit.

[add transition from previous paragrpah] Since LLMs rapidly synthesize executable code, they can generate parts of the evaluator just as they generate solutions. Concretely, we can use AI to intelligently and automatically navigate the trade-off between evaluation speed and quality. By dynamically constructing and refining the evaluation environment, we can optimize evaluator design in ways that were previously infeasible. In the next section, we present our co-evolutionary approach to automate key parts of the evaluation process, enabling the effective application of ADRS to databases. [we demonstrate how to do for databases, this can potentially generalize to other domains, ]

We are now at a critical precipice. 

[research is reaching the limits, make read better and flow well]

this [don't use reactive ] reactive development cycle is no longer sustainable [reaching the limits maybe.

[so what? what is the imapct of this?] 

However, these methods largely treat the engine as a black box,  relying on data-intensive learned models for knob tuning or [be clear the learned model is replacing the component and doing inference at runtime] replacing components with learned models that perform inference at query time.runtime inference—which only adjusts the parameters of existing implementations.

Consequently, the gap between required application performance and existing database capabilities is widening because current approaches to optimizing system performance [replace with something about manual, requires significant manual effort] are struggling to keep pace. The design of high-performance database systems traditionally relies on human-driven algorithm development, [don't repeat manual here] which requires substantial time to and manual effort. [add transition, make read better, flow logically] recent research integrates machine learning (ML) to automate performance optimization. [can we make the next two sentences more concise, make the ML for systems part two sentences total] However, these methods largely treat the underlying engine as a black box, focusing on knob tuning or replacing components with learned models that perform inference at query time. Custom-training a model for these tasks requires significant time and data, and these techniques can ultimately only adjust the parameters of existing implementations. Consequently, learned approaches remain difficult to deploy~\cite{} due to run-time inference overhead, unpredictable worst-case behavior, and the need for specialized ML infrastructure.

[add better transition] A new class of AI-driven techniques is emerging to address these practical limitations while automating system design. [make rest of paragraph more concise, read better, flow welll] Specifically, Large Language Models (LLMs) are enabling a phase shift toward white-box optimization. Instead of executing models at runtime, these techniques use LLMs to generate optimized code directly. 

ADRS frameworks operate through an LLM-driven feedback loop. In each iteration, the LLM generates a candidate solution (e.g., executable code), which is evaluated against a predefined benchmark. Promising solutions and their performance metrics are then incorporated into the prompt for the subsequent iteration, guiding the search toward better programs. ADRS frameworks evolve interpretable source code, yielding solutions that are debuggable, deployable, and free of runtime inference overheads. 

leveraging ADRS for automated algorithm discovery at scale [make active voice, sentence too long and wordy, make read and flow better] will be increasingly necessary. 

Therefore,  [advancing sounds weird, should be somethign about applying ADRS to DBs] advancing ADRS for databases is critical, as it will define how the next generation of high-performance databases are built and optimized.

, with their ability to rapidly generate and evaluate many novel solutions, enable 

By rapidly synthesizing hundreds of novel solutions, ADRS unlocks a scale of algorithmic exploration that was previously unattainable, making its advancement critical for defining how the next generation of high-performance databases are built.

[add better transition, we believe sounds awk, make read better] We believe ADRS will eventually become the norm for performance research by enabling automated algorithm discovery at scale. [make paragraph more concise and precise, read better, flow well] As workload and hardware complexity continue to grow, the demands of system optimization are already outpacing human engineering capacity. Previously, the scale of solution generation and evaluation was constrained by the time required for researchers to manually conceptualize and implement each new approach (e.g., replace this component with a learned model). LLMs overcome this bottleneck by rapidly generating and evaluating hundreds of novel solutions, unlocking a level of optimization that was previously unattainable. Therefore, advancing ADRS for databases is critical, as it will define how the next generation of high-performance databases are built and optimized.

replaces a static, brute-force testing harness with a dynamic, LLM-driven process. The AI dictates which specific queries and rule combinations should be evaluated 

[the discussion about "the system" is really confusing. we should talk about ADRS evalution outer loop and ADRS solution generation inner loop clearly to avoid confusing readers in all text]
[better transition] To automate Technique 3, the system acts as an evaluator by strategically selecting a subset of the workload to analyze [how? be specific]. At each iteration, the AI agent formulates an adaptive [what does search plan mean??] search plan based on prior feedback, targeting specific training queries and promising rule combinations. The LLM analyzes previous performance results on different query features and rule combinations to output a targeted set of evaluation to run. For example, if the LLM notices a performance regression on queries with nested joins, it will generate a search plan requesting latency tests for join-heavy queries using a focused subset of join-reordering rules. [what system?] The system executes this selected subset of rules on the target queries [be clear that this could be diff subset of rules for different queries] on PostgreSQL and records the actual execution latencies. This process generates a ground truth dataset mapping specific query features to highly performant rule sets without requiring exhaustive full-system benchmarking across all possible rule combinations and benchmark queries.
[the content in these two paragraph should be combined as the previous sentence applies to both techniques]
To automate Technique 4 and handle the NP-Hard problem of rule ordering, the system dynamically prunes the search space of rule permutations through two mechanisms. First, it constrains permutations to logical structural templates, such as strictly executing pre-processing rules before main transformations, followed by post-processing cleanup. Second, it filters out invalid rules a priori by invoking their static matching functions. For example, the system immediately discards subquery-related rewrite rules if the input query's abstract syntax tree lacks a subquery. This pruning ensures the evaluator does not waste no cycles testing inapplicable or structurally invalid rule sequences.


[remove any repetition with previous text]
After deciding on the pruned sets of rules to apply to specific subsets of queries, the evaluation outer loop executes these experiments on PostgreSQL and records the execution latencies. This process [builds up over iterations, make read better] generates a ground truth dataset mapping specific query features to highly performant rule sets that can be used by the solution generation inner to generate an optimized rewrite policy.

Specifically, we automate workload selection (Technique 3) and pruning the search space (Technique 4). Our evaluation pipeline for this case study uses AI to decide which specific queries and rule combinations to evaluate in each iteration based on an outer feedback loop (Figure~\ref{fig:query-rewrite}). This enables us to systematically gather the empirical data needed to improve the policy while keeping evaluation costs low.

[explain why we need this, link to challenges about evaluation, there is repeition with previous para, combine, make flow better, read better] The primary goal of this evaluation outer loop is to efficiently generate a ground truth dataset mapping specific query features to highly performant rule sets. To achieve this without exhaustive full-system benchmarking, the LLM constructs targeted experiments by explicitly automating workload selection (Technique 3) and search space pruning (Technique 4).

To automate Technique 3, the LLM dynamically curates the workload by analyzing previous performance results to dictate which queries and rules to test next. For example, if the LLM notices a performance regression on queries with nested joins, it will construct latency experiments specifically for join-heavy queries using a focused subset of join-reordering rules. To automate Technique 4 and handle the combinatorial search space, the loop dynamically prunes the space of rule permutations through two mechanisms. First, it constrains permutations to logical structural templates, such as strictly executing [need to explain what pre-processing, main transformations, and post-processing is if we mention it, or just make it easier to understand and don't use specialized terms] pre-processing rules before main transformations, followed by post-processing cleanup. Second, it filters out invalid rules a priori by invoking their static matching functions. For example, the system immediately discards subquery-related rewrite rules if the input query's [never defined this, can we just use a simpler term] abstract syntax tree lacks a subquery. This pruning ensures the evaluator does not waste cycles testing inapplicable or structurally invalid rule sequences.

[mention technique 3 and 4 explicitly, unclear which are the techniques tie to what]
Within this outer loop, the LLM strategically drives both workload selection and search space pruning in constructing targeted experiments to analyze which rules work well for what query features. In each iteration, the LLM analyzes previous performance results across different query features and rule combinations to output a targeted evaluation strategy. For example, if the LLM notices a performance regression on queries with nested joins, it will construct latency experiments for join-heavy queries using a focused subset of join-reordering rules. To automate Technique 4 and handle the combinatorial search space, the system dynamically prunes the space of rule permutations through two mechanisms. First, it constrains permutations to logical structural templates, such as strictly executing pre-processing rules before main transformations, followed by post-processing cleanup. Second, it filters out invalid rules a priori by invoking their static matching functions. For example, the system immediately discards subquery-related rewrite rules if the input query's abstract syntax tree lacks a subquery. This pruning ensures the evaluator does not waste no cycles testing inapplicable or structurally invalid rule sequences.
[we don't explain the goal until down here. we should have the topic sentence be clear what our goal is and how it relates to techniques 3 and 4 upfront, this whole section needs a lot more structure, make read better, improve logical flow] The evaluation outer loop decides which subsets of rules to try on specific subsets of queries and then executes on PostgreSQL and records the actual execution latencies. This process generates a ground truth dataset mapping specific query features to highly performant rule sets

based on rule categories. For example, it only evaluates permutations where basic pre-processing rules (e.g., pushing down filters) are applied before complex structural transformations (e.g., converting subqueries to joins). [how did we discover these templates? these are evolved over time right? need to mention starting point]

Second,  This pruning ensures the evaluator does not waste cycles testing inapplicable or structurally invalid rule sequences.

it constrains permutations to restricts rule orderings to pre-defined execution phases, ensuring that [why would we want to do this?] basic simplification rules are always tested before applying complex, structural transformations.  

dynamically prunes the space of rule permutations through two mechanisms to help determine what rules to apply and in which order to apply them in.  [we talk about workload earlier and dynamic secltion for Technique 3, can we avoid the repeition and restructure as necessary?] Beyond these static pruning mechanisms, the system dynamically curates the evaluation workload at runtime. In each iteration, the AI analyzes previous performance signals to output explicit search directives (e.g., expanding a successful rule sequence to structurally similar queries), ensuring evaluation cycles are continuously focused on the most promising optimizations.

This automated evaluation environment integrates directly into the standard ADRS solution generation loop. The data gathered during evaluation provides the missing empirical context needed to evolve the policy. In a standard evolutionary loop, the LLM receives the latest execution latencies and correlates the performance wins with query structure. It extracts discriminative features (e.g., \texttt{hasSelfJoin}, \texttt{joinDepth}) to generate pattern hypotheses (e.g., ``If \texttt{hasScalarSubquery}, apply \texttt{FILTER\_SUB\_QUERY\_TO\_CORRELATE}''). The LLM then directly synthesizes these patterns into a custom, executable rewrite policy in Calcite's \texttt{HepPlanner}. To ensure robustness, the system validates the synthesized code against the full training set and a hold-out test set. If performance regressions are detected, the loop triggers a refinement cycle where the LLM investigates failure cases and generates tighter constraints. This self-correcting mechanism iterates until the policy achieves zero regressions.

The final output is an optimized query rewrite policy in Calcite that uses the structural features of input queries to deterministically decide which rules to apply. This design enables the database to achieve the performance benefits of extensive offline analysis with negligible runtime overhead ($<1$ms).

Specifically, [these first two steps are not part of the solution generation loop? or are they?] the solution generation LLM receives as context the latest dataset of execution latencies that correlates the performance wins with query structure. It extracts discriminative features (e.g., \texttt{hasSelfJoin}, \texttt{joinDepth}) to generate pattern hypotheses (e.g., ``If \texttt{hasScalarSubquery}, apply \texttt{FILTER\_SUB\_QUERY\_TO\_CORRELATE}''). The LLM then directly synthesizes these patterns into a custom, executable rewrite policy in Calcite's \texttt{HepPlanner}. To ensure robustness, the system validates the synthesized code against the full training set and a hold-out test set. If performance regressions are detected, the loop triggers a refinement cycle where the LLM investigates failure cases and generates tighter constraints. This self-correcting mechanism iterates until the policy achieves zero regressions.

Applying existing ADRS frameworks to optimize query rewrites is ineffective due to a lack of empirical data on effective rule combinations. Since evaluating rule combinations across the entire workload is intractable, we need to dynamically co-evolve the subset of queries and rules being evaluated. By deploying the LLM in an evolutionary loop to systematically gather data through targeted experimentation, we generate the missing empirical context necessary to discover high-performance rewrite policies.

, preventing the loop from revisiting unpromising combinations.  Together, these mechanisms ensure the search space shrinks monotonically: [unclear what this means] every measurement eliminates redundant exploration.


, and the need for specialized ML infrastructure during deployment.

[for the following para, make these edits: first sentence read like a throwaway first sentence

For example, you could state performance a critical objective, but then that would be a good place to say traditional database R\&D involves manual improvement of design and improvement of algorithms + ML blah blah techniques to tune the parameters etc. because I right now it feels like the second sentence directly moves into changing workloads and hardware, it was a little bit too quick

somewhere add this idae but make read better: As database design evolves and optimize for performance, workload and hardware complexity continues to outpace human R\&D capacity.]
Performance remains a critical objective in database system design. Historically, database architectures have evolved to maintain high efficiency while adapting to changing workloads, hardware, and interfaces (e.g. cloud infrastructure). As such, systems are perpetually playing catch-up to meet the escalating demands of modern applications. However, the traditional research and development cycle is reaching its limits\xs{this seems unnecessarily provoking}. 
Contemporary workloads are becoming significantly more challenging, (e.g., autonomous agents that generate an order of magnitude more requests). Simultaneously, the underlying software stack has become increasingly complex (e.g., integration of specialized accelerators and GPU-native processing). 

Consequently, the gap between required application performance and existing database capabilities is widening, as optimizing system performance requires significant manual effort. The design of high-performance database systems traditionally relies on human-driven algorithm development. To overcome these bottlenecks, machine learning (ML) to automate performance optimization. 
However, these methods largely treat the engine as a black box, relying on data-intensive models either to tune existing knobs or to replace core components and perform inference at runtime. Consequently, these learned approaches remain difficult to deploy~\cite{} due to high run-time inference overhead, unpredictable worst-case behavior, and the need for specialized ML infrastructure during deployment.

To overcome these hurdles\xs{nit: you had ``to overcome'' half a paragraph ago},  This new approach/xs{I'd put the name and ADRS in the topic sentence of this paragraph}, 

\xs{this is great phrasing. probably should use it in the first 1~2 paragraphs}


[what does extreme demands mean? make clear and read better] placing extreme demands on evaluation speed and quality. [need transistion and connect, make logical flow better] 

[too wordy] solving this evaluation is a fundamental prerequisite to effectively applying ADRS in practice.

As prior studies demonstrate, ADRS frameworks are only as effective as the feedback guiding them, requiring robust evaluators that return fast, accurate, and detailed signals. While  recent research focuses primarily on improving solution generation~\cite{}, constructing this critical evaluation pipeline remains a manual endeavor. Solving this evaluation bottleneck is a fundamental prerequisite to effectively applying ADRS in practice. [from this paragraph, I'm not quite getting why evaluation is crucially the bottleneck, esp compared with previous human driven R\&D loops. -- you say this in xxx are only as effective as the feedback, which is also true previously with manual approaches. the point of ADRS can do 100x or more iterations without human supervision places more emphasis on eval quality and speed.]

\xs{from this paragraph, I'm not quite getting why evaluation is crucially the bottleneck, esp compared with previous human driven R\&D loops. -- you say this in xxx are only as effective as the feedback, which is also true previously with manual approaches. the point of ADRS can do 100x or more iterations without human supervision places more emphasis on eval quality and speed.}

and\xs{typo here?} 

because they are highly problem-specific. 
Evaluators are structured around three key axes: the system, the workload, and the search space. 

to reduce the required number of iterations, they can restrict the solution search space while minimizing potential lost . [don't repeat what we already said]  
While effective, these techniques are problem-specific and require considerable manual effort to implement. 
Ultimately, these traditional approaches are powerful tools 


\ion{Wasn't always the case that people believed these cost models are not that accurate, especially for filters and joins?} but recent research demonstrates they can fail to accurately reflect end-to-end performance due to intricate component interactions~\cite{}. 

% [somehow combine these two sentences?] 

% To mitigate these overheads, database researchers have developed several standard techniques to balance between evaluation speed and quality, but applying these methods effectively is a [make read better] difficult process.

% [topic sentence needs to say these techniques are hard to apply, allude to last sentence in paragrpah] 
% To mitigate these overheads, database researchers traditionally employ several standard techniques to balance between evaluation speed and quality but requires significant manual effort. 
[the other paragraph that jumped out to me was the one that starts with "to mitigate these workloads" where you talk about existing evaluation trade-off techniques. One, I think, is a bit too long. Two, it wasn't clear to me how complicated things actually are. if you say evaluate only on a subset of workload or restrict search space, that sounds kind of like pretty trivial, but I don't quite get why they're powerful tools and also difficult to apply

And potentially, especially for the middle three sentences, like at the system level, blah blah blah, to restrict the solution search space, feels like that can be significant. Gently shortened.

need to be clear what require manual effort and highly task specific efforts, which bot loop can solve]
[topic sentence too long but want to maintain all key points, make read better ]

\ion{I think we need a figure here. It will make easier to parse this paragraph.} \accheng{label arrows with signals, what these are} 

\accheng{bring up technique discussion here, want to be more principled
not just 4 random techniques but emphasize we cover the whole space}
\ion{Shouldn't also emphasize on the different techniques to evolve the evaluator?} 

In summary, we make the following three contributions:
\begin{itemize}
    \item We demonstrate the application of ADRS to core database components, discovering novel algorithms for buffer management, query rewriting, and index selection and achieving performance improvements over current state-of-the-art baselines.
    \item We propose methodologies to address the challenges of applying ADRS to databases, including simulation, data sparsity, and workload selection.
    \item We discuss the implications of the ADRS approach for database performance optimization and highlight future research opportunities.
\end{itemize}


capable of dynamically adapting to complex workloads and evolving hardware architectures [still need some humans] without relying on manual human engineering.

\xs{make sure here you also include this paper's main contribution -- eval, e.g., ``in particular, armed with xxx''}
[make paragraph read better and flow well, need to add more setnences to the end to flesh out content] 

LLMs to successfully navigate large search spaces and optimize complex, stateful components. Ultimately, automating the evaluation pipeline removes a critical barrier, allowing databases to more rapidly adapt to shifting workloads and modern hardware.

[make read better] There are many exciting potential opportunities with this approach. 
[too wrody, overclaiming , dramatic, make read better] In particular, armed with our co-evolutionary framework to automate the evaluation bottleneck, researchers can now fully realize the potential of this approach. By dynamically balancing evaluation speed and fidelity, this methodology enables LLMs to effectively explore massive search spaces and optimize complex, stateful database components. Ultimately, eliminating the manual engineering required for system evaluation paves the way for fully autonomous databases capable of continuously adapting to arbitrary workloads and novel hardware architectures without human intervention.

% This paper provides a vision of how AI-driven optimization will impact database research. A new class of AI-Driven Research for Systems (ADRS) has demonstrated exciting success in applying LLMs to automate solution discovery and is poised to shift the researcher's role from designing solutions to leveraging these frameworks to search for better solutions. 
% However, applying this paradigm to databases is uniquely challenging.
% The stateful nature of these systems presents challenges in specifying correctness and performance guarantees. Moreover, their immense complexity makes fast, high-fidelity evaluation difficult. In this paper, we argue that realizing the full benefits of ADRS for databases addressing these two core challenges: (i) formulating the problem precisely, which involves translating ambiguous performance goals and implicit application semantics into concrete constraints and objectives, and (ii) building fast, high-fidelity evaluation frameworks to assess and verify generated algorithms. We discuss how addressing these challenges will not only accelerate the pace of discovery but also change how we design, build, and optimize database systems in the future.



The design of high-performance database systems is shifting from manual heuristics toward automated, white-box optimization. AI-Driven Research for Systems (ADRS) enables Large Language Models to generate executable code for system components, yet its application to databases is hindered by the prohibitive cost of end-to-end evaluation and vast search spaces. This paper introduces a framework that automates these evaluations by co-evolving the evaluation process alongside the solutions. Rather than treating simulators, performance models, and workload subsets as static artifacts, we refine them within an evolutionary loop to guide the search toward high-performance code. We evaluate our approach through three case studies: buffer management, query rewriting, and index selection. Our results show that co-evolved algorithms outperform state-of-the-art solutions by up to 2.0$\times$ lower latency. These findings demonstrate that co-evolving evaluation fidelity is an effective strategy for automating database system research.

This paper provides a vision of how AI-driven optimization will impact database research. 

[sentence too long, make more concise, using automate too muhc] 

has demonstrated exciting success in applying LLMs to automate solution discovery and is poised to shift the researcher's role from designing solutions to orchestrating the frameworks that drive automated discovery. 


leveraging these frameworks to search for better solutions. [rewrite below, should mention evaluation challenge first, then that it is especially challenging for databases. to enable ADRS to be applied to databases, we propose...fill this in.
we deomonstrate through through three case studies (buffer management, query rewriting, and index selection) get  algorithms outperform state-of-the-art solutions...
]
However, applying this paradigm to databases is uniquely challenging.
The stateful nature of these systems presents challenges in specifying correctness and performance guarantees. Moreover, their immense complexity makes fast, high-fidelity evaluation difficult. In this paper, we argue that realizing the full benefits of ADRS for databases addressing these two core challenges: (i) formulating the problem precisely, which involves translating ambiguous performance goals and implicit application semantics into concrete constraints and objectives, and (ii) building fast, high-fidelity evaluation frameworks to assess and verify generated algorithms. We discuss how addressing these challenges will not only accelerate the pace of discovery but also change how we design, build, and optimize database systems in the future.


The evolution also revealed a fundamental tradeoff regarding data distribution: a query's optimal rule sequence can occasionally change based on literal parameter values. The system learned to navigate this, keeping rules where the performance wins on one variant heavily outweighed the regressions on another. This resulted in the discovery of a balanced rule selector with zero net regressions across 120 queries that beats R-Bot on both benchmarks.

\subsubsection{ADRS Experimental Setup.} We implement our evaluator outer loop and solution generator inner loop in [Java?], consisting of [XK] lines of code. We use TPC-H and DSB benchmarks with SF=10, following the RBot paper~\cite{}. [mention we use subset of queries (only one variant to avoid overfitting and show that our solution/approach generalizes]
We run [X] iterations of outer loop. Each outer loop does [X] number of queries execution on average.

Since existing ADRS frameworks do not support [add details], we implement a custom ADRS framework heavily inspired by OpenEvolve~\cite{} as our ADRS framework. 
The evaluator reports the geometric mean cost improvement previously described and checks for validity (rule selectors that raise a compile error, produce regressions beyond a threshold, or time out are filtered). We use GPT-4o and run 100 iterations. The search completes in about eight hours and costs less than \$30.

need to mention how many iterations it took for us to get to this result, 

[update the following section based on  calcite/autoevolve-dev/openevolve/tasks/calcite/RuleSelector.java, cross reference with results and wins ]
\textbf{Best evolved policy.} [link back to our described automated evaluator outer loop before and mention how we were able to get the result, make read better and flow logically better, add some more structure in presenting content]
Our best evolved query rewrite policy...
includes a number of key design innovations: (1) tight feature guards that prevent regressions by conditioning on exact query structure (e.g., excluding \texttt{DISTINCT} queries to avoid an 11\% regression on TPC-H query16), (2) multi-rule combinations that pair complementary rules (e.g., \texttt{FILTER\_INTO\_JOIN} + \texttt{JOIN\_TO\_CORRELATE} for 20x speedup on DSB query100), (3) scale-aware conditions that account for behavioral differences between SF=1 and SF=10, and (4) a broadly-applicable expression simplification pattern (\texttt{FILTER\_ REDUCE\_EXPRESSIONS}) that improves 18 query instances not covered by the hand-crafted seed. The evolution also revealed a fundamental tradeoff: conditions tight enough to avoid regressions on one workload may miss improvements on another, leading to the discovery of a balanced rule selector with only one accepted regression across 120 queries that beats R-Bot on both benchmarks.
Figure~\ref{} shows a comparison between R-Bot, the hand-crafted rule selector, and the best evolved rule selector with highlighted key changes.

Correctness is validated continuously, and each final latency data point is calculated using a trimmed mean over these three independent runs.

[fix details for paragraph, cehck machine in remote setup, we use c5.18xlarge, add any other missing, relevant details]
\subsubsection{PostgreSQL Experimental Setup.} 
We implement the best evolved rule selector in Apache Calcite's HepPlanner, integrated with PostgreSQL 17. We run experiments on [c.14xl] EC2 machines with 72 cores, 144 GiB of RAM, and [X] SSD storage. We use PostgreSQL's optimizer cost estimates for evolution and validate with actual execution latency. [how do we verify correctness of rule selector? add one sentence]
Our experiments measure query latency over [X runs, do we have warmup? check] Correctness is validated by comparing row counts between original and rewritten queries. Each data point is the median over five independent runs.

[mention Rbot reflection loop not available, we implement based on description]

\textbf{Query Latency.}
We compare \textit{R-Bot} with two types of baselines, including learning-based methods (\textit{LearnedRewrite}), and origin LLMs (\textit{GPT-4}, \textit{GPT-3.5}).


\paragraph{Query Latency Reduction.} Table 4 shows the query latency of rewritten queries. \textit{R-Bot} outperforms the other query rewrite methods across all the datasets and metrics. The reasons are two-fold.
First, \textit{R-Bot} can judiciously retrieve relevant rule specifications and Q\&As to figure out the rewrite rules pertinent to the input query. For instance, \textit{R-Bot} can apply the exploration rule ``AGGRE\-GATE\_EXPAND\_DISTINCT\_AGGREGATES\_TO\_JOIN'' weakly related to the input query, using retrieved evidences to achieve a 5.6x optimization. However, the other methods fail to identify this critical rule without guidance from rewrite evidences. Besides, we find that \textit{GPT-4} and \textit{GPT-3.5} tend to select only a small number of rules (e.g., 1), which is often sub-optimal. That is because, they exhibit hallucination without rewrite evidences, and thus miss the intricate correlations between rewrite rules and the input query.

Second, \textit{R-Bot} adopts a step-by-step LLM rewrite method, which can leverage rewrite evidences to understand the interrelations among the rewrite rules during rule arrangement. For instance, \textit{R-Bot} can accurately select and arrange multiple rewrite rules (e.g., 6) from analysis of retrieved evidences, so that they can co-operate together to rewrite the input query to an execution-efficient form (e.g., 4.6x accelerated). On the contrary, since \textit{LearnedRewrite} relies on blind exhaustive search, it can hardly find the optimal rule sequence among tremendous possibilities (e.g., only 4.3x accelerated).

\paragraph{Overall Latency Reduction.} We also evaluate overall latency on larger TPC-H 50x and DSB 50x datasets. As shown in Figure 6, \textit{R-Bot} achieves the best latency, demonstrating improvements of 1.82x and 1.68x respectively. The reasons are three-fold. First, \textit{R-Bot} can still optimize the query latency by finding better plans, thus outperforming other methods. Second, \textit{R-Bot} takes some time (e.g., average around 1 min) to retrieve beneficial evidences and iteratively instruct LLM to select and arrange rewrite rules. Thus it can steadily identify the critical rewrite rules (e.g., ``FILTER\_SUB\_QUERY\_TO\_JOIN'') with much higher query latency reduction. Instead, other methods do not spend efforts understanding rewrite evidences, which often causes sub-optimal rewritten queries. Third, compared with results of TPC-H 10x and DSB 10x (see Table 4), we find that \textit{R-Bot} remains similar rewrite latency but demonstrates higher query latency reduction proportional to data scale, which both results in superior overall latency.

In contrast, the evolved policy compiles into deterministic, interpretable Java code. It executes with sub-millisecond overhead and relies on precise feature guards generated during offline evolution, entirely preventing the unpredictable worst-case behavior associated with runtime LLM calls.

[mention RBot results non-deterministic, high inference runtime, weaknesses of black-box approach]

\textbf{TPC-H.}
TPC-H queries feature correlated subqueries and multi-way joins that respond well to subquery decorrelation. Five queries time out in the original (query2, 17, 20, 21, 22), and four of these are resolved by both our rule selector and R-Bot. The difference appears in the remaining non-timeout queries: the evolved rule selector improves 22 of these (up to 3.1x on query10), while R-Bot improves none. The largest single improvement is query22, which drops from \textasciitilde2.75 hours to 6.5 seconds (1519x) via \texttt{AGGREGATE\_REDUCE\_FUNCTIONS} + \texttt{FILTER\_SUB\_QUERY\_TO\_CORRELATE}. Overall, our rule selector reduces average TPC-H latency by 71.6\% (from 74.5s to 21.1s), compared to R-Bot's 51.8\% reduction (to 36.0s), with zero regressions for both.

\textbf{DSB.}
DSB queries are more structurally diverse, involving unions, outer joins, nested subqueries, and complex aggregations. The evolved rule selector improves 32 of 76 instances (42.1\%), while R-Bot improves 10 (13.2\%). The top improvements are query081 (5021s to 1.6s, 3234x) and query054 (478s to 0.2s, 2424x), both resolved by subquery decorrelation rules that R-Bot does not select. The raw evolved output contains 8 regressions, of which 7 are eliminated by tightening feature guards in post-processing; the remaining one (query094\_0, 1.5x slower) is accepted because the same pattern produces a 2.15x improvement on query094\_1. R-Bot produces 2 regressions, including a 31x slowdown on query100. Overall, our rule selector reduces average DSB latency by 87.0\% (from 19.2s to 2.5s), compared to R-Bot's 32.5\% reduction (to 13.0s). These results demonstrate that ADRS can discover robust rule selection policies that generalize across different analytical workloads.

Second, and most critically, \textit{R-Bot} incurs an enormous runtime overhead. [don't start sentence with because] [rest of text has too many adjectives, too verboce, make more concise and direct without cutting content, should readn ad flow well] Because it relies on a black-box approach, \textit{R-Bot} spends an average of over one minute per query performing RAG evidence retrieval and iterative LLM inference calls just to decide on a rule sequence. For the vast majority of operational queries, this massive rewrite latency completely negates any execution speedups. In stark contrast, the evolved policy compiles into deterministic, interpretable Java code. It executes rule selection with sub-millisecond overhead, ensuring that any query execution improvements immediately translate into net overall latency reductions.
Third, the runtime LLM inference utilized by \textit{R-Bot} is fundamentally non-deterministic. The system frequently spends minutes analyzing a query only to hallucinate a sub-optimal or invalid rule sequence, resulting in wasted rewrite time and degraded execution time. By relying on precise, statically compiled feature guards generated during offline evolution, our white-box policy entirely prevents the unpredictable worst-case behavior associated with runtime LLM calls, guaranteeing reliable end-to-end performance.

[update with new insight, undate rest of text accordingly] Our core insight is that ``efficient evaluation requires evolving goals'': the optimal testing strategy shifts from broad exploration to focused validation as the policy matures. Since unguided exploration wastes evaluation cycles, we leverage the AI to set explicit search goals for each iteration (e.g., ``verify if this winning rule helps similar queries'' or ``pinpoint the exact rule causing this regression''). The framework learns to pivot its evaluation focus, moving from discovering new patterns to exploiting successful ones and isolating bugs, maximizing the value of every cycle. We apply this approach by implementing an autonomous evolution loop to optimize SQL query rewriting (\textbf{Case study \# 2)}. Our framework iteratively tests rule combinations, analyzes performance, and synthesizes selection logic to automatically discover a rewrite policy that reduces latency by up to X.Y$\times$.

\xs{here too, love to get the point across that the growing scale of solution iterations necessitates faster, better, repeatable eval} 

automating this pipeline to carefully balance rapid evaluation cycles with high-fidelity performance measurements.

[lot of repetition in this paragraph, cut redundancy, make omre clear, precise, concise, make read better and flow well]
While ADRS frameworks excel at generating solutions~\cite{} and are continuing to improve~\cite{}, the evaluation setup remains a critical bottleneck. These frameworks are fundamentally only as effective as the feedback guiding them, requiring robust evaluators that return fast, accurate, and detailed signals. Since ADRS frameworks can rapidly generates many novel solutions, evaluating these candidates requires fast and accurate evaluation cycles. Consequently, automating this evaluation pipeline is essential for the long-term viability of ADRS. Evaluation is generally difficult in automated system design, requiring a careful balance between rapid feedback and high-quality performance measurements. 

To eliminate this bottleneck, we propose automating the evaluation setup itself. As LLMs can rapidly synthesize executable code, they can generate parts of the evaluator just as they generate solutions. Concretely, we can use AI to intelligently and automatically navigate the trade-off between evaluation speed and quality\xs{nit: this doesn't \textit{quite} seem concrete lol}. By dynamically constructing and refining the evaluation environment, we can optimize evaluator design in ways that were previously infeasible. In the next section, we present our co-evolutionary approach to automate key parts of the evaluation process, enabling the effective application of ADRS to databases. While we demonstrate this methodology within the context of database systems, our approach can potentially generalize to other domains.

[sentence too long but don't lose any ideas] ADRS frameworks have been successful primarily on performance problems for which the generated algorithms do not alter the underlying semantics of the database for easier veritication. However, applying ADRS to more complex problems, such as concurrency control or write-ahead logging, is an open research question. A subtle bug in transaction isolation directly corrupts data rather than just slowing down execution.
To safely evolve these critical components, the evaluation pipeline must move beyond simple performance metrics to integrate rigorous correctness checks. This shift may requires embedding formal verification or exhaustive fuzzing [is the word really fuzzing? not fuzzy testing or something? check]. [add sentence to end on future work in how to automate this]

The primary challenge then becomes balancing absolute safety with search efficiency. It remains to be seen whether automated frameworks can synthesize proven, core transactional logic without rendering the evaluation loop prohibitively slow.

guaranteeing the original semantics remain intact.

[make read better and transistion] The goal is to help application developers write better queries, a notoriously difficult challenge in industry~\cite{}. Applying ADRS directly to these workloads has the challenge of specifications. Unlike internal system components that operate under well-defined guarantees (e.g., [add examples]), developers typically express application correctness constraints implicitly within their code. [give a clearer example] For instance, a financial workload might enforce a balance invariant using application-level conditionals. Safely optimizing these complex queries requires a formal understanding of these unstated requirements. This gap presents an opportunity to use AI agents to reverse-engineer formal specifications directly from source code, documentation, and runtime behavior. For ambiguous logic, the system could interactively prompt developers with hypothetical scenarios to clarify intent. Once these implicit rules are translated into explicit specifications, ADRS frameworks can aggressively optimize the workload, such as safely restructuring entire transactions, while mathematically guaranteeing that the original semantics remain intact.

\textbf{Workload optimization.} [while we focus on system optimization, there is also opportunity for workload optimization. mention goal here is to help application developers write better queries, this is notoriously hard challenge in industry~\cite{}. ]
Applying ADRS directly to user workloads introduces a distinctly different obstacle: missing specifications. System components typically operate under well-defined contracts, but developers frequently leave critical application rules implicit within their code. For instance, a financial workload might enforce a balance invariant using application-level conditionals rather than explicit database constraints. Safely rewriting or optimizing these complex queries requires a formal understanding of these unstated requirements.
This gap presents an opportunity to use AI agents to reverse-engineer formal application specifications. An agent could analyze source code, documentation, and runtime behavior to infer underlying data invariants and transactional boundaries. For ambiguous logic, the system could interactively prompt developers with hypothetical scenarios to clarify intent. Once these implicit rules are translated into explicit formal specifications, ADRS frameworks can aggressively optimize the workload, such as restructuring entire transactions, while mathematically guaranteeing that the original application semantics remain intact.

This shift also [replace: motivates] further modularity in systems. Future architectures could their core components, such as the query optimizer, transaction manager, and buffer pool, through interfaces that would allow ADRS agents to seamlessly swap, rewrite, and evaluate individual components, transforming the database into a platform designed expressly for automated evolution. One promising direction is to extend the concept of structural abstractions, previously introduced as storage engine templates for key-value stores~\cite{cosine}, to general relational systems. [Mention this blog post as well as sign of moving toward modularity: this is well-aligned with recent industry trends...https://www.databricks.com/blog/what-is-a-lakebase]

[don't be so black and white, suggest room for interpretation] We argue that future database systems should prioritize predictable behavior over out-of-the-box efficiency. By providing a stable and deterministic foundation, these systems enable ADRS frameworks to model costs accurately, evaluate candidates reliably, and ultimately generate much higher-performing, workload-specific implementations. 


[write in active voice, make read better, use language of reference text] Success now depends on providing rigorous specifications rather than writing low-level code. As LLMs learn to co-evolve both the solution and the evaluator, humans will increasingly operate as high-level orchestrators. [frame as interesting future work or question] It remains to be seen whether researchers will act as interactive supervisors tightly guiding the evolutionary loop or if future frameworks will synthesize production-ready engines entirely from abstract specifications.

[make much more concise and to the point, make read better and flow better] [paragraph takes way too long to get to main point, shorten significatnly without losing main ideas]
\textbf{The shifting role of the database researcher.} Traditional database engineering requires manually implementing concurrency protocols or complex query optimizer rules. ADRS offloads this tedious implementation and debugging to an automated loop. Consequently, the researcher's role elevates to higher-leverage tasks: formulating precise problems, defining robust cost models, and establishing strict transactional invariants. We can view ADRS as an unbounded fleet of automated system engineers capable of testing thousands of algorithmic variations in parallel. This accelerates discovery by rapidly prototyping ideas and revealing novel architectural directions, even when the generated code requires further refinement.
Furthermore, ADRS explores massive database search spaces much more thoroughly than human developers. While a human might stop tuning an index selection heuristic once it achieves acceptable average-case performance, the AI continuously iterates to exploit non-intuitive, compounding micro-optimizations. The critical skill for future database researchers will no longer be writing low-level system code. Instead, success will depend on the ability to provide rigorous, unambiguous specifications that effectively guide these automated assistants toward production-ready engines.
 As LLMs become capable of co-evolving both the solution and the evaluator, humans will increasingly operate as high-level orchestrators focused on system invariants and workload semantics. It remains to be seen whether developers will act as interactive supervisors tightly guiding the evolutionary loop, or if future frameworks will synthesize production-ready engines entirely from abstract specifications.

 \xs{
S5: if Postgres's optimizer is known to struggle with analytical workloads, it's odd to say "serves as the default baseline". -- since Table 2 only shows OLAP workloads.

it'd possibly make the case stronger if we show the ADRS result is great for both OLTP and OLAP, either by comparing OLTP workloads against postgres baseline or by having ADRS come up with a policy to triage which optimizer to use.} 

\textbf{ML for DBs / LLMs for DBs..}
\accheng{
two categories: 
1. tuning, configs, etc. --> LLM-based tuner, look at Immanuel Trummer work on knob tuning

2. replace with learned component --> query rewrite 
}


While variants like ThetaEvolve~\cite{wang2025thetaevolve} and FLEX~\cite{cai2025flex} explore learning-based adaptations, our work focuses on inference-only evolutionary scaffolds.

Recent work leverages LLMs to automate broader parts of the research process. Building on genetic programming foundations~\cite{langdon2013foundations, koza1994genetic}, FunSearch~\cite{romera2024mathematical} and ELM~\cite{lehman2023evolution} use LLMs as semantic variation operators. Frameworks such as AlphaEvolve~\cite{alphaevolve, nadga2025alphaevolve, novikov2025alphaevolve}, OpenEvolve~\cite{openevolve}, and CodeEvolve~\cite{assumpccao2025codeevolve} use the MAP-Elites algorithm and island models to evolve new algorithms; GEPA~\cite{agrawal2025gepa} employs reflective prompt evolution for better LLM generation; and LLM4AD~\cite{liu2024llm4ad} provides a unified platform for algorithm design. Others include ShinkaEvolve~\cite{shinkaevolve, lange2025shinkaevolve} (sample-efficient evolution), EvoPrompt~\cite{evoprompt, guo2023evoprompt} (genetic prompt optimization), MetaMuse~\cite{ma2025algorithmgenerationcreativeideation} (self-reflective generation), and PolicySmith~\cite{dwivedula2025manmade} (solution selection). Additional mechanisms evolve mutation operators~\cite{fernando2023promptbreeder}, apply reflection-guided dynamics~\cite{ye2024reevo}, use hindsight fine-tuning (SOAR~\cite{pourcel2025self}), or explore context-efficient updates (DeltaEvolve~\cite{jiang2026deltaevolve}) and progress-aware evolution~\cite{yan2026pacevolve}. While variants like ThetaEvolve~\cite{wang2025thetaevolve}, FLEX~\cite{cai2025flex}, and TTT-Discover~\cite{yuksekgonul2026learning} explore learning-based adaptations, our work focuses on inference-only evolutionary scaffolds.
Attempts at end-to-end research automation are also emerging. MLGym~\cite{nathani2025mlgym} offers AI research agent benchmarks, while Code Researcher~\cite{singh2025code} explores agents for large-scale software engineering. Work on self-evolving AI agents~\cite{fang2025comprehensive} and broader systems applications~\cite{liang2025nexthorizon,zhouneuripstalk} is also growing. Darwin~\cite{zhang2025darwin} demonstrates open-ended, self-referential code improvement, automatically evolving stronger coding agents. Glia~\cite{hamadanian2025gliahumaninspiredaiautomated} presents an agentic workflow for systems design, reporting strong results on distributed LLM inference.  Tools like GitHub Copilot~\cite{GitHubCopilot}, Cursor~\cite{CursorAgent2024}, Codex~\cite{OpenAICodex}, and Claude Code~\cite{ClaudeCode2025} accelerate research by helping researchers rapidly prototype ideas, build simulators, and implement baselines. 
They enable rapid translation of high-level concepts into working implementations. 
Recent work also explores using LLMs for performance-critical code~\cite{hong2025autocompllmdrivencodeoptimization}, such as GPU kernel code generation and optimization~\cite{ouyang2025kernelbench}, further illustrating their potential for \SYS/. 

% \textbf{ADRS.} 
% Beyond coding, recent work leverages LLMs to automate broader parts of the research process. 
% Frameworks such as AlphaEvolve~\cite{alphaevolve, nadga2025alphaevolve} and OpenEvolve~\cite{openevolve} use the MAP-Elites algorithm and island models to evolve new algorithms; GEPA~\cite{agrawal2025gepa} employs reflective prompt evolution for better LLM generation; and LLM4AD~\cite{liu2024llm4ad} provides a unified platform for algorithm design. 
% Others include ShinkaEvolve~\cite{shinkaevolve} (sample-efficient evolution), EvoPrompt~\cite{evoprompt} (genetic prompt optimization), MetaMuse~\cite{ma2025algorithmgenerationcreativeideation} (self-reflective generation), and PolicySmith~\cite{dwivedula2025manmade} (solution selection). Glia~\cite{hamadanian2025gliahumaninspiredaiautomated} presents an agentic workflow for systems design, reporting strong results on distributed LLM inference.

% Attempts at end-to-end research automation are also emerging. MLGym~\cite{nathani2025mlgym} offers AI research agent benchmarks, while Code Researcher~\cite{singh2025code} explores agents for large-scale software engineering. Work on self-evolving AI agents~\cite{fang2025comprehensive} and broader systems applications~\cite{liang2025nexthorizon,zhouneuripstalk} is also growing. 
% Darwin~\cite{zhang2025darwin} demonstrates open-ended, self-referential code improvement, automatically evolving stronger coding agents.

% Our work focuses on automated algorithm discovery in systems, where strong evaluators enable the reliable verification needed for productive automation.

overcome the historical challenges of high-latency benchmarking and combinatorial search spaces. Our case studies show that this approach consistently produces white-box solutions that match or exceed human-designed heuristics. More importantly, these results signal a fundamental shift in database research. Instead of relying on opaque runtime controllers or manual engineering, future optimization will increasingly depend on models generating deployable, debuggable source code. As computing environments grow in complexity, the co-evolution of evaluators and solutions provides a scalable path for interpretable system optimization. While we demonstrate this methodology within the context of database systems, our approach can potentially generalize to other domains.

This paper demonstrates that AI-Driven Research for Systems (ADRS) can effectively automate the discovery of high-performance database systems. By co-evolving evaluation artifacts like simulators and workload subsets alongside the candidate code, we overcome the challenges of high-latency benchmarking and combinatorial search spaces. Our case studies in buffer management, query rewriting, and index selection show that this approach produces white-box solutions that match or exceed the performance of human-designed heuristics. These results highlight a shift toward an optimization paradigm where models generate deployable, debuggable source code rather than acting as opaque controllers. The ability to automatically refine the evaluation signal ensures that the discovery process remains both efficient and accurate. As database environments grow in complexity, the co-evolution of evaluators and solutions provides a scalable path for interpretable system optimization without specialized inference infrastructure.

While we demonstrate this methodology within the context of database systems, our approach can potentially generalize to other domains.

% \lma{I think there are also some special algorithms designed for this? Maybe add a sentence on that to distinguish ADRS from simply prompting the LLMs.}

architectures diverge and workloads become increasingly 


[make more concise and direct, too wordy, make read better, especialyl end of paragraph can make much shorter but don't cut content]
In contrast, ADRS presents a white-box approach that optimizes database systems by using LLMs to generate and evolve interpretable source code. This generated code is auditable by developers, predictable in its behavior, and deployable. For instance, AlphaEvolve~\cite{alphaevolve}, and ADRS framework from DeepMind, discovered a scheduling policy that improved Google's fleet-wide utilization by 0.7\%. 
Beyond efficiency, ADRS offers flexibility, discovering both generalizable algorithms for different systems (e.g., robust buffer replacement policies) and or specialized logic tailored to specific instances (e.g., instance-optimized systems~\cite{Kraska2019SageDB,}). By automating the validation of thousands of candidates, ADRS accelerates the development lifecycle, identifying optimizations that manual engineering might miss. , demonstrating potential of these frameworks for production systems. As the capabilities of ADRS frameworks and LLM models improve, we envision ADRS extending beyond component optimization to synthesize entire data structures and protocols ``just-in-time'' for next-generation databases.

For example, Datadog leveraged evolutionary algorithms to generate efficient code that improved throughput by an order of magnitude~\cite{}.

% \lma{I think we want to expand on that a bit. As you mentioned above, there are two types of prior work on ML for DB. One is tuning database configurations (including knobs and physical design (e.g., indexes)). The other is to replace database components (e.g., learned indexes). Then you say these are primarily black-box models. In my opinion, the primary advantage of white-box (code-based) models is that they're easier to explain and deploy (don't need an AI/ML infrastructure). Then you can talk about how they don't have the problem of high inference overhead and unpredictable behavior.} \accheng{thanks, updated}

% \lma{Do we need to mention the instance-optimized here? I think nothing of ADRS for DB is specific to instance-optimized. In fact, I think your buffer pool algorithm can generalize to different databases? So I think we may not need to emphasize instance-optimized here. I think it's just that, as a first attempt, some of our algorithms have stronger generalization ability, while others are less generalizable and more specific to a particular database (i.e., instance-optimized), which are still very valuable.} \accheng{we should discuss this. isn't instance-optimization an advantage for us?} 

Pruning the search space to limit exploration to a subset of optimization techniques can reduce the number of required iterations. While this accelerates convergence, it restricts coverage and requires domain expertise to ensure that critical optimization opportunities are not discarded.

As LLMs can rapidly synthesize executable code, we use them dynamically refine the evaluation environment just as they generate candidate algorithms. We leverage AI to intelligently navigate the trade-off between evaluation speed and quality by optimizing evaluator design (e.g., constructing simulators, developing performance models, selecting workloads, and pruning search spaces) in ways that were previously infeasible. In the next section, we present a co-evolutionary framework to automate key parts of the evaluation process, enabling the effective application of ADRS to databases.

Specifically, we detail how the massive scale of autonomous solution generation requires robust evaluators that return rapid, high-fidelity feedback. We outline why achieving this speed-quality balance is exceptionally difficult for databases due to their stateful architectures and combinatorial search spaces, ultimately requiring automated evaluation environments that traditionally require slow, manual benchmarking.

In this section, we provide background on how ADRS frameworks automate parts of the research process and highlight their potential for databases. We then discuss the main challenges in applying ADRS to databases, namely [problem formulation and evaluation].

% \lma{Do we really want to use ``marginal''? Maybe just say humans may overlook things.}

% \accheng{right now, it's unclear what is prior work

% we need to make clear solution generation is promising, lots of ppl working on

% problem formulation is human-based for now

% evaluation is LLM-able but no one has worked on it yet

% just say we're solving evaluation, doing these things right now because key to long-term success of this method and currently unsolved
% frame it more as a shift rather than this is something cute

% put 2.1 and 2.3
% what is ADRS
% promising for DBs
% evaluation is not solved but useful and why it's particularly hard for DBs
% }


% \accheng{these are pre-ADRS techniques

% make more clear that we're generating code, can make more concise}



% \accheng{have figure or table to clarify what we're trading off for the 4 existing techniques

% how do you do evaluation at a high level?
% workload
% search space of solutions
% modeling = not running anything
% running a simulator
% run in real system

% right now, flow is: standard techniques --> we automate techniques

% we're missing in 2.3 (1) The evaluation is hard. (2)Why is the evaluation harder in the case of DBSs vs other systems? 
% we only talk about (2) currently
% we demonstrate how to do for databases, this can potentially generalize to other domains, maybe say this
% }

%\accheng{unclear about modeling e2e behavior}  %Rather than executing queries, researchers can model end-to-end behavior using analytical proxies, 

% \lma{I think we want a bridge/transition to the next section. Something like why a simulator is important to this problem.}

\accheng{should we talk about a framework here or just our experiences?}

% \lma{I'm actually slightly confused about how the simulator is ``derived from''  the baselines (e.g., CLOCK). In my understanding, the simulator emulates how the database uses the buffer pool policy, but should be independent from the policy itself? What does ``derived from'' the baseline mean? It's a bit unclear to me.}

\accheng{challenges about implementing solution in full system?}
\accheng{correctness?}

% \lma{One thing I think that is not super clear is the relationship between the evolution of the simulator and the policy. Do you first focus on evolving the best simulator? Or do you evolve the simulator and the policy alternatively through multiple iterations? What's your/the recommended workflow?} \accheng{co-evolving, workflow not clear

% cost model, query estimation model}

tests simulator variants, translates discovered policies into C, and analyzes real-world PostgreSQL performance to automatically discover a simulator design that maximizes policy quality. 

We iterate through six versions with Cursor, discovering that without access to baseline implementation logic and performance data in the full system, the generator produced oversimplified simulators that constrained the search space. Access to this information guided the AI to expose rich system state (e.g., scan contexts and I/O latencies) in the simulator, enabling the discovery of policies that exploit these features for better performance.

Since the simulator excluded this metadata, it was impossible to re-discover strategies such as PBM-Sampling that rely on future access estimates. However, when we allowed the AI to relax structural constraints without baseline guidance, we encountered the trade-off of low-fidelity simulators. Cursor generated simulators that permitted unrealistic techniques, such as expensive full buffer pool scans, which were infeasible in the full system.


The outer loop refined the simulator over iterations to balance [X with Y, fill in]
The outer loop relaxed constraints in early versions to encourage more diverse policies but this generated low-fidelity environments that permitted unrealistic techniques like full buffer pool scans that were infeasible in the full system.. Conversely, simplistic models failed to expose the true cost of operations.
Inline with our insight, providing access to multiple ground-truth baselines (Clock, PBM-PQ, PBM-Sampling) was crucial towards evolving an effective simulator. These implementations defined the feasible search space, demonstrating which algorithmic techniques could be implemented within PostgreSQL's architectural constraints without over-constraining the design space. This calibration guided the AI to expose rich runtime metadata, specifically scan contexts and block groups, allowing the final simulator to model necessary components beyond the buffer manager.
By comparing simulated performance against the actual throughput of evolved baselines, the framework identified that the simulator lacked fidelity regarding PostgreSQL's specific concurrency mechanisms. It failed to model ring buffers (which prevent scan pollution), hint-bit dirtying, and the real-world costs of tick contention and per-access overheads. Consequently, the framework refined the simulator to incorporate these architectural realities. This demonstrates our ``more is more'' insight: by exposing the full system's structural constraints, the AI learned to model the performance trade-offs of eviction logic overhead. Subsequent policy evolution shifted away from complex, high-overhead CLOCK modifications. Instead, it produced CV2, a policy that utilizes a lock-free sampling design. This refinement allowed CV2 to evaluate a larger set of candidates (up to 30 samples) to achieve a 64.8\% hit rate while minimizing the lock contention that hindered previous sampling approaches.

The simulator also required refinement to accurately model system overheads, demonstrating that an effective simulator must capture architectural constraints. While early versions of the simulator allowed the inner loop to discover access-count-based CLOCK modifications that improved simulated scores by up to 16\%, these policies failed when translated to C. 

[frame this not as optimization objective but just as part of simulator refinement, we should update this based on whatever simulator changes were required to obtain CV2 from @EXPS, mention the key different iterations we went through and how the refinement worked]
However, when the outer loop relaxed structural constraints without baseline guidance, it generated low-fidelity simulators. These simulators permitted unrealistic techniques, such as expensive full buffer pool scans, which were infeasible in the full system. 
The optimization objective for policy evolution also required refinement, demonstrating that the appropriate simulator is a function of the target metric. While the inner loop initially instructed the AI to maximize cache hit rate, this metric alone was insufficient as it treats all evictions equally, ignoring physical I/O costs: synchronous dirty writes ($\sim$200$\mu$s) are 10$\times$ slower than sequential reads ($\sim$20$\mu$s). By comparing simulated hit rates against the actual throughput of evolved baselines translated to C, the framework identified that policies with identical hit rates yielded different throughput depending on eviction cost. Consequently, the AI calibrated the objective function to incorporate operation latency. This demonstrates our ``more is more'' insight: by exposing the full system's latency characteristics, the AI learned to model performance trade-offs in the simulator that previous versions lacked. Subsequent policy evolution prioritized evicting clean pages and sequential scan victims over dirty or random-access pages. This prioritized eviction is not due to scan pages being less valuable, but due to the cost of a ``wrong'' eviction being lower, which preserves critical I/O bandwidth.

\textbf{More baselines: evolving for the right abstraction.} 
Providing access to multiple ground-truth baselines (Clock, PBM-PQ, PBM-Sampling) was crucial towards evolving towards an effective simulator. These implementations defined the feasible search space, demonstrating which algorithmic techniques could be implemented within PostgreSQL's architectural constraints without over-constraining the design space. This calibration guided the AI to expose rich runtime metadata, specifically scan contexts and block groups, allowing the final simulator to model necessary components beyond the buffer manager.

\textbf{More metrics: evolving for the right metric.} 
Our optimization objective for policy evolution also required refinement, demonstrating that the appropriate simulator is a function of the target metric. While we initially instructed the AI to maximize cache hit rate, this metric alone was insufficient because it treats all evictions equally, ignoring physical I/O costs: synchronous dirty writes ($\sim$200$\mu$s) are 10$\times$ slower than sequential reads ($\sim$20$\mu$s). By comparing simulated hit rates against the actual throughput of evolved baselines, Cursor identified that policies with identical hit rates yielded different throughput depending on eviction cost. Consequently, Cursor calibrated the objective function to incorporate operation latency. This demonstrates our ``more is more'' insight: by exposing the full system's latency characteristics, the AI learned to model performance trade-offs in the simulator that previous versions lacked. Subsequent policy evolution prioritized evicting clean pages and sequential scan victims over dirty or random-access pages—not because scan pages are less valuable, but because the cost of a ``wrong'' eviction is lower, preserving critical I/O bandwidth. We describe the results of our best evolved policy in the next section.

\textbf{Final simulator.} Our final simulator is trace-based and models PostgreSQL's buffer pool with realistic I/O costs (100$\mu$s for random reads, 200$\mu$s for dirty page evictions). It reports a latency score inversely proportional to simulated average I/O wait time (accounting for SSD read latency and synchronous dirty-page write cost) that represent a cost-weighted generalization of hit rate that penalizes expensive misses and dirty evictions. 

\textbf{Co-evolutionary workflow.} This case study demonstrates our approach for simulator c-evolution. Specifically, we apply the following workflow alternating between simulator refinement and policy discovery:
\begin{enumerate}
    \item Generate a simulator candidate using the full-system implementation as context.
    \item Evolve policies using this simulator.
    \item Implement and evaluate the evolved policies on the full system.
    \item Use the performance data as signal to refine the simulator if needed (return to step 1). 
\end{enumerate}
We note that simulator evolution is a search problem, analogous  to policy evolution, yet arguably harder as the ``optimal'' simulator is hard to quantify. This case study demonstrates that an appropriate simulator needs to be tuned with respect to both the specific system and metric(s) to optimize for (see Section~\ref{} for further discussion). 
Iterative co-evolution enables us to navigate the design space to develop a suitable simulator that balances execution speed with fidelity.

[remove metric mention, highlight key points from @] to both the specific system and metric(s) to optimize for. Iterative co-evolution enables the framework to navigate the design space to develop a suitable simulator that balances execution speed with fidelity. We describe the results of our best evolved policy in the next section. 


Figure~\ref{} shows a comparison between the state-of-the-art policy, PBM-Sampling, and the best evolved policy with highlighted key changes

In this section, we describe the results of our best evolved policy. We use OpenEvolve to discover caching algorithms in our simulator from the previous section. 

\subsubsection{ADRS Experimental Setup.} We use OpenEvolve~\cite{} as our ADRS framework. We run the simulator on traces of TPC-C and TPC-H for evolution. The simulator reports the latency score previously described and checks for validity (algorithms that raise a runtime error, exceed a reasonable timeout, or fail to serve all requests are filtered). We use GPT-5.0 and run 100 iterations. The search completes in about eight hours and costs less than \$30.

\textbf{Best evolved policy.}
The best evolved policy includes a number of key algorithmic innovations: (1) fast-path probes that handle 80\% of evictions with O(1) cost, (2) cost-aware Belady scoring that accounts for refetch costs, (3) dual clean/dirty tracking that prioritizes evicting clean pages, and (4) workload-adaptive parameter tuning. The evolution also revealed a fundamental tradeoff: policies optimized for pure OLAP workloads degrade by 35\% on mixed workloads, leading to the discovery of a balanced policy that beats PBM-Sampling on both.
Figure~\ref{} shows a comparison between the state-of-the-art policy, PBM-Sampling, and the best evolved policy with highlighted key changes.


\begin{figure*}[t!]
\caption{Side-by-side comparison of the initial PBM-sampling eviction policy and the evolved combined strategy. Key innovations in the evolved policy are highlighted.}
\label{fig:pbm_evolution_comparison}
\centering

% --- Left Side: PBM Sampling ---
\begin{subfigure}{0.45\textwidth}
    \begin{minted}[
        frame=lines,
        fontsize=\tiny,
        linenos,
        breaklines=true
    ]{python}
def PBM_Sampling(buffers, estimator, N=16):
    samples = []
    while len(samples) < N:
        buf = random_buffer()
        if buf.refcount != 0:
            continue

        # Estimate next access from scan tracking
        next_access = estimator.estimate(buf)
        if next_access == NOT_REQUESTED:
            # No scan needs this page -- evict now
            return buf

        samples.append((buf, next_access))

    # Evict buffer with furthest next access
    # (Belady approximation)
    best = max(samples, key=lambda s: s[1])
    if best.buf.can_evict():
        return best.buf

    # Fallback: return any unpinned buffer
    return random_unpinned_buffer()
      \end{minted}
    \caption{Before: PBM-Sampling Policy}
    \label{fig:pbm-sampling-code}
\end{subfigure}
%
\hfill
%
% --- Right Side: Evolved Combined Strategy ---
\begin{subfigure}{0.45\textwidth}
    \begin{minted}[
        frame=lines,
        fontsize=\tiny,
        linenos,
        breaklines=true,
        highlightlines={2-7,9-13,15-20,27-28,30-31,33-34,37-38,41-42},
        highlightcolor=blue!10
    ]{python}
def CombinedPolicy(buffers, estimator, N=16):
    # FAST PATH 1: Empty buffer (3 probes)
    for _ in range(3):
        buf = random_buffer()
        if buf.refcount == 0 and buf.block_group is None:
            return buf

    # FAST PATH 2: Cold + clean (5 probes)
    for _ in range(5):
        buf = random_buffer()
        if (buf.refcount == 0 and buf.usage_count == 0
                and not buf.is_dirty):
            return buf

    # FAST PATH 3: Orphaned clean (4 probes)
    for _ in range(4):
        buf = random_buffer()
        if buf.refcount == 0 and not buf.is_dirty:
            if not buf.block_group.has_scans():
                return buf

    best_clean = best_dirty = (None, -INF)
    for _ in range(N):
        buf = random_unpinned_buffer()
        t = estimator.estimate(buf)

        # Cost-aware Belady: scan pages cheap to refetch
        cost = 1.0 if buf.scan_count > 0 else 5.0
        score = t / cost

        # CLOCK integration: favor cold pages
        score += (5 - buf.usage_count) * 5.0

        # Multi-scan protection
        if buf.scan_count > 1:
            score -= (buf.scan_count - 1) * 5.0

        # Dirty penalty: avoid sync write cost
        if buf.is_dirty:
            score -= 20.0

        # Dual tracking: separate clean and dirty
        if buf.is_dirty:
            best_dirty = max(best_dirty, (buf, score))
        else:
            best_clean = max(best_clean, (buf, score))

    # Always prefer clean for latency
    return best_clean[0] or best_dirty[0]
    \end{minted}
    \caption{After: Evolved Combined Policy}
    \label{fig:combined-evolved-code}
\end{subfigure}
\end{figure*}


\subsubsection{Postgres Experimental Setup.} We implement the best evolved policy on PostgreSQL 14.0 version, the same as PBM-Samlping. We run experiments on ec2 [c.14xl] machines with 64 cores, 144 GiB of RAM, and 300GB SSD. We use Benchbase~\cite{} as our workload generator. 
Our experiments measure buffer cache hit rate, I/O volume savings, throughput, and runtime. Cache hit rate is measured using PostgreSQL’s built-in statistics. We use the default sample size of 10 blocks and the following PostgreSQL settings. \accheng{TBU} Each data point plotted is the average over three independent runs. The error bars represent 95\% confidence intervals
around the means.

We compare the performance of our best evolved policy on two standard workloads: TPC-C and TPC-H. TPC-C~\cite{tpc-c}, a standard OLTP benchmark, simulates the business logic of e-commerce suppliers with five types of transactions.  We configure TPC-C to run with 100 warehouses (total size of 8GB). TCP-H~\cite{tpc-h}, a standard OLAP benchmark, consists of 22 analytical queries involving sequential scans, bitmap scans, and joins over a supplier-and-orders schema. We run TPC-H at scale factor 10 (total data size of 10GB).

These experiments run TPC-H queries 1 through
16 once each in a random order in each query stream. (TPC-H has 22 queries, but the query plans chosen by PostgreSQL for a few of the later queries result in them taking orders of magnitude longer to run than the other queries. Thus those queries are omitted to keep the experiments’ runs feasible and to avoid having only one access pattern dominate the workload. We use same setup, indexes, and other parameters as the PBM-Sampling paper % [check @new_paper.md Section 6.5 for details]
The buffer cache size is 16 GiB and no cgroup. 

\textbf{TPC-C.}
TPC-C is notably write-heavy and has transactions that can span over 50 items. 
Its requests tend to fall into two categories: either they access a small set of popular keys (i.e., those in the Warehouse and District tables) or a larger range of keys from a distribution with a long tail (Customer, Item, Stock). 
Consequently, TPC-C cannot benefit from the predictive scan benefits in PBM-Sampling: most transactions access a small set of hot keys that are already in the cache (the object hit rate is >50\% with a 10\% cache size in Figure~\ref{fig:w-all-3}c) along with a larger set of cold keys that are unlikely to be cached and contaminate the other keys (hit rate grows slowly as cache size increases). Moreover, transactions tend to access keys in quick succession (e.g., once an order is placed, it is then processed, paid for, and delivered), so recency is especially important in this workload. All algorithms incorporate recency in some form, so performance is similar across these policies, with up to 9K txns/s and 27ms avg. latency. Our best evolved policy performs on par with single-object policies.


[make less wordy and cut redundancy, make read better without cutting content: These implementations define the feasible search space and demonstrate which algorithms worked within PostgreSQL's architectural constraints. This calibration guides the AI to expose rich runtime metadata, specifically scan contexts and block groups, allowing the simulator to model necessary components beyond the buffer manager.]
[add transistion, make clear it was full system performance metrics that led to this discovery] The outer loop also discovered that modeling cache hit rate alone in the simulator was insufficient since this metric treats all evictions equally, ignoring physical I/O costs where synchronous dirty writes ($\sim$200$\mu$s) are much slower than sequential reads ($\sim$20$\mu$s). 

Furthermore, by comparing simulated performance against full system performance metrics, the framework identified that early simulators failed to model specific concurrency mechanisms, such as ring buffers (which prevent scan pollution), as well as real-world overheads (e.g. lock contention). Consequently, the framework refined the simulator to incorporate these architectural realities, forcing the AI to account for various performance trade-offs. This drove policy evolution away from complex, high-overhead CLOCK modifications to our best evolved policy that utilized a lock-free sampling design (described in the next section). 
[The optimization objective for policy evolution also required refinement, demonstrating that the appropriate simulator is a function of the target metric. While the inner loop initially instructed the AI to maximize cache hit rate, this metric alone was insufficient as it treats all evictions equally, ignoring physical I/O costs: synchronous dirty writes ($\sim$200$\mu$s) are 10$\times$ slower than sequential reads ($\sim$20$\mu$s). By comparing simulated hit rates against the actual throughput of evolved baselines translated to C, the framework identified that policies with identical hit rates yielded different throughput depending on eviction cost. Consequently, the AI calibrated the objective function to incorporate operation latency. This demonstrates our ``more is more'' insight: by exposing the full system's latency characteristics, the AI learned to model performance trade-offs in the simulator that previous versions lacked. Subsequent policy evolution prioritized evicting clean pages and sequential scan victims over dirty or random-access pages. This prioritized eviction is not due to scan pages being less valuable, but due to the cost of a ``wrong'' eviction being lower, which preserves critical I/O bandwidth.]

\textbf{Workload optimization.} 
Beyond system design, ADRS can help application developers write better queries, a notoriously difficult industry challenge~\cite{}. However, automating this introduces a specification problem. Unlike internal system components that operate under strict contracts (e.g., serializability or crash recovery guarantees), developers typically express application correctness implicitly within their code. For instance, a financial app might prevent overdrafts using a mid-transaction conditional rather than a declarative database constraint. Safely optimizing these queries requires formalizing these unstated requirements. AI agents can bridge this gap by reverse-engineering formal specifications directly from source code and runtime behavior, interactively prompting developers with hypothetical scenarios to resolve ambiguity. Once translated into explicit specifications, ADRS frameworks can aggressively rewrite the workload, such as restructuring entire transactions, while mathematically guaranteeing that the original semantics remain intact.


\textbf{Naive application: the cost metric illusion.} Since most prior index selection work [clarify what focus means, they just measure improvements wrt cost estimates, check @paper.md] focus on cost estimation~\cite{}, we initially attempt to apply ADRS frameworks to generate solutions using this as the main performance metric but found this led to ineffective polices. This is because cost estimates is not an accurate reflection of query latency in practice. Initially, we attempted to evolve a single global policy by prompting the LLM to minimize the PostgreSQL optimizer's total cost estimate and benchmarking it against standard benchmarks (TPC-H, DSB). This approach plateaued quickly as the cost model relies on static statistics and assumptions that frequently diverge from runtime behavior. For example, the baseline \texttt{db2advis} algorithm achieved a 29.5\% cost reduction but degraded actual latency by 10.7\%. This misalignment occurs since the optimizer overestimates the selectivity of certain predicates (e.g., date ranges on fact tables) while underestimating the overhead of index maintenance and I/O. The unguided LLM search wasted evaluation cycles optimizing for theoretical improvements that failed to materialize in practice, trapping evolution in a local optimum with performance far worse than the SOTA baseline.

Direct application of existing ADRS frameworks to generate index selection policies is ineffective due to the inaccuracy of using a simplified performance model based solely on optimizer cost estimates. While cost estimation is generally used in a lot of index selection work~\cite{} because it enables faster evaluation results, it is not an accurate reflection of actual query performance. 

[update text below as follows: we are automating Technique 2 in this case study (added description below for context). rather than using static performance model of cost estimation, we co-evolve it based on the generated policies, follow reference text

\item \textbf{Technique 2. E2E Performance Modeling}. Modeling end-to-end behavior using simplified metrics (e.g., cost estimation versus query latency) enable faster results but need to accurately reflect full system performance.]
rather than relying solely on the optimizer's cost model, the AI uses actual execution latency to evaluate performance. Existing ADRS frameworks cannot be directly applied as they rely on fast but inaccurate proxy metrics that fail to reflect physical database realities. Accordingly, the evaluation outer loop generates high-fidelity feedback through cascade evaluation (Technique 1) and interleaved measurement (Technique 2).

\textbf{Naive optimization: the cost metric illusion.} Direct application of existing ADRS frameworks to generate index selection policies is ineffective due to the [clarify that we are using performance model with simplified metric of cost estimation. this is generally used in a lot of index selection work~\cite{} because enables faster results but turns out it is not accurate of actual query performance] inaccuracy of the optimizer's cost model. Initially, we attempted to evolve a policy by prompting the LLM to minimize the PostgreSQL optimizer's total cost estimate. This approach plateaued quickly as the cost model relies on static statistics and assumptions that frequently diverge from runtime behavior. For example, the baseline \texttt{db2advis} algorithm achieved a 29.5\% cost reduction but degraded actual latency by 10.7\%. This misalignment occurs since the optimizer overestimates the selectivity of certain predicates (e.g., date ranges on fact tables) while underestimating the overhead of index maintenance and I/O. Consequently, the simulator encouraged the selection of indexes that looked good on paper but performed poorly on disk. The unguided LLM search wasted evaluation cycles optimizing for theoretical improvements that failed to materialize in practice, trapping the policy evolution in local optima.


[reframe the following: there can be noise in performance model / evaluation / performance metrics, which we have to carefully account for. non-deterministic evaluators is known challenge for ADRS~\cite{let-the-barbarians-in}. the outer loop tried various techniques to denoise signal (add examples like taking avg, median, etc.). found that there was big variance (bigger than latency difference between baselines). describe how the outer loop framework identified why there was noise (due to cache, buffers overwritten, different queries seqs, background processes -- snapshotting, etc.). the outerloop tried various things to mitigate this before settling on  had to warmup and measure per query in isolation, same order]
However, a naive execution approach is insufficient because latency measurements are highly susceptible to noise from buffer cache states, cache evictions, and background processes. To mitigate this, the outer loop restricts the evaluation to an interleaved execution pattern. Specifically, the outer loop requires that each query be warmed up and immediately benchmarked before moving to the next query, rather than warming up all queries sequentially. Furthermore, the system immediately runs a warmup execution to load necessary pages into memory before recording the actual benchmarking time, and suppresses background processes that cause latency spikes during the evaluation. This shrinks the measurement noise from areas that are likely to lead to poor fitness signals.

[reframe the following: we tried different combinations of metrics for evolution/combined\_score, we tried cost estimations first, then latency; we tried latency + runtime + storage; other combinations. the outer loop determines metric and the inner loop evolves on metric. then, we measure the performance of evolved policy on the metrics we care about. in the end, we found just using latency was sufficient proxy becasue XYZ...]
This is achieved through a cascade evaluation strategy that progressively filters candidate policies using increasingly expensive but accurate metrics. First, the AI utilizes fast but imprecise cost estimates from the database optimizer to reject constraint violations and isolate clearly ineffective candidate policies. In each iteration, the AI outputs explicit cost thresholds to formulate a targeted evaluation plan. For example, if the LLM notices a candidate policy fails to achieve a minimum cost reduction compared to the baseline, it will immediately discard it.

[reframe and rewrite the text below to clearly describe our evaluation outer loop and how we evolve the performance model to automate technique 2. see the reference text but you can change the structure of your text as needed. make it clear HOW we are automating the performance model and what signals we get from the inner loop. describe our framework, how it automates technique 2, and the output]
\textbf{Automating the performance model.}
To address the evaluation overheads of executing queries to gather latency, we co-evolve the evaluation metric alongside the policy itself. For this case study, the primary goal of this evaluation outer loop is to efficiently generate a reliable ground truth dataset mapping specific index combinations to actual execution latencies. This empirical data is needed to inform the generation of an optimized index selection policy in the solution generation inner loop. Our evaluation pipeline uses AI to construct targeted experiments by automating cascade evaluation (Technique 1) and interleaved measurement (Technique 2).

To automate Technique 1, the LLM dynamically curates the evaluation pipeline by using cost estimates to dictate which candidate policies to test next. The LLM curates these candidates from a designated pool of generated algorithms. The loop applies this insight in practice: the AI rejects constraint violations and isolates clearly ineffective policies using the fast cost metric, and only promotes promising candidates to the slow latency evaluation stage. In each iteration, the AI outputs explicit cost thresholds to formulate a targeted evaluation plan. For example, if the LLM notices a candidate policy fails to achieve a minimum cost reduction compared to the baseline, it will immediately discard it, ensuring each evaluation cycle focuses on promising optimizations.

To automate Technique 2, the loop bounds the noise inherent in latency measurements through two static measurement mechanisms and a third method based on execution ordering. First, it requires a cache warmup for each query before measurement to ensure consistent buffer states. For example, the system immediately runs a warmup execution to load necessary pages into memory before recording the actual benchmarking time. Second, it restricts the evaluation to an interleaved pattern empirically discovered during an initial exploratory phase. Specifically, the outer loop requires that each query be warmed up and immediately benchmarked before moving to the next query, rather than warming up all queries sequentially. Third, background processes that cause latency spikes are suppressed during the evaluation. This shrinks the measurement noise from areas that are likely to lead to poor fitness signals.

it learns to penalize [what is date column? need to provide benchmark and context] date column indexes on large fact tables (which the optimizer inaccurately favors) and prioritize small dimension table indexes that facilitate merge joins. 

[reframe and write the following: the final performance model is...
The solution generation inner loop uses the model for evolution. Specifically, we evolve index selection policies... The final output is an optimized index selection policy that performs well on all the metrics we care about (list)

make read well and flow logically, make sure to mention we're automating technique 2 somewhere
]

Our core insight is [fill in]: 
rather than relying on a static performance model of cost estimation, the evaluation outer loop iteratively refines how to evaluate performance for solution generation inner loop. \accheng{TBU}


- technique
 % \item \textbf{Technique 2. E2E Performance Modeling}. Modeling end-to-end behavior using simplified metrics (e.g., cost estimation rather than actual query latency) enable faster results. The primary challenge is ensuring these proxies maintain fidelity by accurately reflecting true system performance.

- how automate tech

naive: evolve on cost estimation. this is fast because no need to execute, just query planner. this is conventional metric

what we realized is bad proxy, not correlated well to execution latency. in some cases, even negative % (check @index_openevolve/harald-findings/cost-vs-latency.md and add example)

we tried evolving on full latency for all queries. but there is a lot of noise (due to cache, buffers overwritten, different queries seqs, background processes -- snapshotting, etc.). 
tech 1: interleaving -- what we did is that we had to warmup and measure per query 

latency as proxy metric for everything else or we just care about latency the most?

- insight for automate tech


Our optimization target is to minimize the total execution time of the workload under the chosen indexes, i.e., find an optimal index set $I$ that minimizes the total execution latency of the queries in $W$, while satisfying the storage budget constraint $B$. \accheng{need to update this: several metrics we care about}

The most popular algorithm index selection algorithm used in most systems today is, AutoAdmin~\cite{}, which utilizes a greedy search strategy. It iteratively selects the index with the highest estimated cost reduction per unit of storage. While efficient, this heuristic often gets trapped in local optima due to its myopic focus on immediate gains that ignores interactions between index candidates. It also relies on optimizer cost estimates, which frequently correlate poorly with actual execution time. Recent work introduced learning-based approaches (e.g., SWIRL~\cite{}, DRLindex~\cite{}) which use Reinforcement Learning (RL) to explore the search space. Specifically, they model the problem as a Markov Decision Process (MDP) \accheng{check} and train a model to select indexes based on long-term rewards (i.e., the cumulative workload cost reduction). However, the learned model is a ``black box'' and must perform inference at runtime. \accheng{is runtime an issue?} \ak{What is runtime here? I assume these run offline on recent workload samples, in which case inference/slowdowns mean you can run it less often but probably not a dealbreaker?} Our goal in this case study is to evolve a deterministic index selection policy that executes as code during runtime.
[let's just say we pick the best baselines from the paper wrt cost and runtime, mention the one that is actually deployed in practice]

[add topic sentence about overview of state of the art, what does postgres use by default? add that]
A recent comprehensive study~\cite{} compared a wide range of index selection algorithms, revealing mixed findings regarding the trade-offs between heuristic-based and learning-based approaches. The study found that while learning-based advisors can sometimes identify effective indexes for static queries, they suffer from high performance variance, poor robustness to data shifts, and unpredictable behavior when storage budgets increase. Conversely, heuristic-based algorithms remain highly robust and scale well, but they occasionally get trapped in local optima due to their strict reliance on inaccurate optimizer cost estimates.
Based on these findings, we focus on evolving a deterministic, code-based index selection policy that executes natively at runtime, avoiding the unpredictability of learned, black-box models. We benchmark our evolved policy against the four most competitive heuristic baselines identified in the study: \texttt{Extend}, \texttt{DB2Advis}, \texttt{Anytime}, and \texttt{AutoAdmin}. We selected these specific baselines because they represent the current state-of-the-art trade-offs between search efficiency and high estimated cost reduction. Notably, \texttt{AutoAdmin} is  deployed in production systems (e.g., integrated into Microsoft SQL Server's commercial tuning software~\cite{}). 


Attempts at end-to-end research automation are also emerging. 
Darwin~\cite{zhang2025darwin} demonstrates open-ended code improvement, while Glia~\cite{hamadanian2025gliahumaninspiredaiautomated} presents an agentic workflow for systems design. Broader efforts explore research benchmarks and large-scale software engineering agents~\cite{nathani2025mlgym, singh2025code, fang2025comprehensive}. Coding assistants like GitHub Copilot~\cite{GitHubCopilot},  Cursor~\cite{CursorAgent2024}, and Claude Code~\cite{ClaudeCode2025} accelerate research by enabling rapid prototyping of ideas and baselines. Recent work also explores using LLMs for performance-critical code~\cite{hong2025autocompllmdrivencodeoptimization}, such as GPU kernel code generation and optimization~\cite{ouyang2025kernelbench}, further illustrating their potential for ADRS. Most of this prior work focuses on automating solution generation; our focus in this paper in co-evolving the evaluation setup.

% For the first direction, early approaches framed tuning as black-box optimization guided by surrogate models and adaptive sampling~\cite{Duan2009iTuned}. OtterTune~\cite{VanAken2017OtterTune} leveraged historical tuning traces to recommend configurations across deployments. Subsequent systems expanded the learning toolbox with deep reinforcement learning~\cite{Zhang2019CDBTune}, meta-learning for cross-workload robustness~\cite{Li2021ResTune}, and online Bayesian optimization under workload drift and safety constraints~\cite{Zhang2022OnlineTune}. More recent work incorporates textual and domain knowledge directly into the tuning loop. DB-BERT~\cite{Trummer2022DBBERT} extracts tuning hints from manuals using pretrained language models, while GPTuner and $\lambda$-Tune use LLMs to shape search spaces and generate configuration scripts~\cite{Lao2024GPTuner,Giannakouris2025LambdaTune}. Agentic and retrieval-grounded variants further decompose and contextualize the DBA workflow~\cite{Li2025AgentTune,Sun2025Rabbit}.
% Beyond knob selection, self-driving and instance-optimized systems, such as Cosine~\cite{Chatterjee2022Cosine} and SageDB~\cite{Kraska2019SageDB} broaden the scope to physical design and deployment decisions under performance and cost constraints~\cite{,Yu2024BRAD,Sudhir2023Pando,Ding2021MTO}.

% In parallel, another line of work replaces or augments core DBMS components with learned models.
% Learned index structures, beginning with the Recursive Model Index~\cite{Kraska2018LearnedIndex}, and later dynamic variants, such as ALEX~\cite{Ding2020ALEX} and PGM-Index~\cite{Ferragina2020PGMIndex}, approximate data distributions to accelerate lookups, with further refinements and hardware acceleration~\cite{Wu2021LIPP,Kim2024SIA}.
% Learned cardinality estimation models~\cite{Kipf2019MSCN,Yang2019Naru,Hilprecht2020DeepDB} replace hand-crafted estimators with neural density models.
% Query optimization has been framed as a learning problem in systems, such as Neo~\cite{Marcus2019Neo} and Bao~\cite{Marcus2021Bao}, followed by reinforcement-learning and learning-to-rank approaches~\cite{Yang2022Balsa,Zhu2023Lero}.
% Recent work also applies learning and LLMs to query rewrite selection~\cite{Zhou2022LearnedRewrite,Li2024LLMR2,Sun2025RBot} and to concurrency control policies~\cite{Wang2021Polyjuice}.
% Overall, these approaches replace specific heuristics or cost models with learned components while retaining the surrounding system architecture.

because these generated algorithms do not alter the underlying semantics of the database, making verification relatively straightforward. However, applying ADRS to more complex subsystems, such as concurrency control or write-ahead logging, remains an open research question. To safely evolve these critical components, the evaluation pipeline must move beyond simple performance metrics to integrate rigorous correctness checks. This shift may require embedding formal verification or exhaustive fuzz testing directly into the evolutionary search. Future work could investigate how to automate the construction of these complex verification pipelines.

Beyond system design, ADRS also offers significant opportunities for workload optimization. However, automating [what?] this introduces a specification problem. 

To realize this direction, one promising step is to extend the concept of structural abstractions, previously introduced as storage engine templates for key-value stores~\cite{cosine}, to general relational system.

To support rapid evaluation, future databases should prioritize predictability over out-of-the-box performance. Historically, developers build highly coupled architectures to maximize efficiency, but the resulting unpredictability hinders AI-driven search. Providing predictable behavior [replace: provides ] a stable foundation for ADRS frameworks to accurately evaluate candidate solutions. 

A stable foundation enables ADRS frameworks to accurately model costs and evaluate candidate algorithms. This shift requires extreme modularity. We propose extending structural abstractions, like the storage engine templates in~\cite{cosine}, to general relational systems. By exposing core components (e.g., the query optimizer and buffer pool) through rigid APIs, developers transform the database from a static monolith into a manipulable environment. These explicit interfaces allow AI agents to seamlessly swap, rewrite, and evolve individual subsystems.

We could potentially leverage AI agents  to formalize these unstated requirements by reverse-engineering specifications directly from application code. With explicit rules established, ADRS frameworks could safely optimize queries while preserving semantics.

\textbf{Architecting databases for AI.} The emergence of ADRS frameworks motivates a fundamental shift in database design towards predictability and modularity. Historically, developers have built highly coupled, complex architectures to squeeze out maximum baseline performance, often at the cost of system predictability. However, this unpredictability severely hinders AI-driven search. We anticipate future systems may prioritize predictable behavior over out-of-the-box efficiency. This would enable ADRS frameworks to more reliably generate higher-performing, workload-specific implementations. This shift also demands greater modularity in systems. Future architectures could expose their core components, such as the query optimizer, transaction manager, and buffer pool, through interfaces that would allow ADRS agents to seamlessly swap, rewrite, and evaluate individual components, transforming the database into a platform for automated evolution. This structural shift aligns well with recent industry trends toward decoupled data architectures, such as the Lakebase model~\cite{lakebase}. To realize this direction, one promising step is to extend the concept of structural abstractions, previously introduced as storage engine templates for key-value stores~\cite{cosine}, to general relational system.

[combine next two sentences, make read beter and flow logically: We anticipate future systems may prioritize predictable behavior over out-of-the-box efficiency. This would enable ADRS frameworks to more reliably generate higher-performing, workload-specific implementations.]
ADRS also encourages greater modularity in systems. [make more concise and read better] Future architectures could expose their core components, such as the query optimizer, transaction manager, and buffer pool, through interfaces that would allow ADRS agents to seamlessly swap, rewrite, and evaluate individual components, transforming the database into a platform for automated evolution. This structural shift aligns well with recent industry trends toward decoupled data architectures, such as the Lakebase model~\cite{lakebase}. 

Success now depends on providing these automated assistants with clear specifications and well-defined goals. [kind of redunant, merge with above and make read and flow well] As LLMs learn to co-evolve both the solution and the evaluator, humans will increasingly act as high-level orchestrators. A key question for future research is the optimal degree of human involvement in guiding this evolutionary loop.

[elevate unclear, make clear that it frees up time[ elevates the researcher's role to the critical task of formulating the right problems to solve. Rather than writing low-level code, researchers must now provide these automated assistants with clear specifications and well-defined goals. As LLMs learn to co-evolve both the solution and the evaluator, humans will increasingly act as high-level orchestrators. A key question for future research is the optimal degree of human involvement in guiding the evolutionary loop.

Consequently, rather than proposing a monolithic architecture, we adapt the co-evolutionary loop to target the primary evaluation bottleneck of each specific problem.

compared to the real system [clarify this, basically performance results on simulator should reflect performance results on real system]. [add specific, clear, concise sentence about what this meant for the cahe simultor] Our key insight is that ``more is more'': calibrating the simulator against multiple ground-truth baselines is essential for [make sentnece connect to earlier stated goal] exposing the necessary system state while preserving the expressivity required for complex policies.

the tension between speed and fidelity by dynamically automating simulator design (Technique 1). In this context, evolving the evaluator means iteratively refining the simulator's structural constraints (e.g., exposing scan contexts and modeling lock contention) and its internal cost metrics. The optimization goal for the evaluator is to maximize its correlation with full-system PostgreSQL throughput while remaining fast enough to support thousands of policy iterations. 

\textbf{Case study \# 1: buffer cache optimization (Section~\ref{sec:buffer}).} We demonstrate how we can co-evolve the simulator alongside caching policies to achieve [10\%] higher hit rate. This study addresses the tension between speed and fidelity by employing a simulator (Technique 1). Our core insight is that ``more is more'': calibrating the simulator against multiple ground-truth baselines is essential for exposing the necessary system state while preserving the expressivity required for complex policies.

[need to focus on what is the optimization goal that we are evolving for on the evaluation side] to maximize the discovery of performant rule patterns while minimizing evaluation time. [unclear how this sentence links to our goal, this should explain optimization goal that we are evolving for on the evaluation side specific to this case study] For the evaluator, our outer loop iteratively constructs highly targeted experiments to map specific optimization rules directly to matching query structures. Our key insight is ``go off what you know'': to identify promising directions without wasting cycles, the evaluator should exploit prior empirical successes.

We demonstrate how to co-evolve the evaluation workload and search space alongside query rewrite policies to generate solutions that reduce query latency by [200]\%. This study addresses automating Techniques 3 and 4 in selecting the workload subset and pruning the combinatorial search space to ...[rewrite to read well]. For the evaluator, our outer loop iteratively generates highly targeted query workloads to map specific optimization rules to matching query structures. Our key insight is that ``context is key'': actively generating targeted training data allows the framework to prune the search space effectively, focusing the inner loop's exploration strictly on high-impact rule combinations.

We demonstrate how we can evolve the problem context to generate a query rewrite policy that reduces query latency by [200]\%. This study focuses on balancing speed with generality and coverage within a combinatorial search space (Techniques 3 and 4). Our insight is that ``context is key'': actively generating targeted training data allows the framework to prune the search space effectively, focusing exploration on high-impact rule combinations.

% \lma{I feel like the transition to the next section is a bit abrupt. Maybe just be upfront about the organization of this paper, which is that we don't have a single architecture that solves all three problems. Rather, we adapt ADRS in three different scenarios to solve the problems separately. And we discuss the adaptation for each problem, followed by the evaluation of that problem. We can probably even have a section to explicitly set this up.}

\lma{Another thing is that we should make sure the order of the challenges, the order of the case studies, and the discussion of each of them in the subsequent sections are in the same order.}

We show how we can automatically select appropriate workloads and metrics to reduce query latency by [50]\%.
This study tackles achieving fidelity and generality with reasonable latency by refining proxy metrics and workload subsets (Techniques 2 and 3). Our insight is that ``ground truth is king'': evolving the objective function from optimizer cost estimates to actual latency signals prevents the discovery process from overfitting to inaccurate models.

For index selection, our evaluation outer loop iteratively designs a performance model from inaccurate cost estimates that leverage ordered handle non-deterministic results. Our key insight is to ``mind the gap'':the evaluator should actively investigate  [word to read better] the physical discrepancies and measurement artifacts that separate theoretical proxies from true end-to-end performance.

reachehile \textit{R-Bot} achieves total workload speedups of 2.11$\times$ on TPC-H and 1.69$\times$ on DSB, o
s 5.18$\times$ and 6.73$\times$ speedups, , respectively.

non-intuitive, multi-rule synergies that an LLM cannot reliably discover on the fly. 

\lma{from XXs?} 
. Second, our white-box policy avoids limitations inherent to \textit{R-Bot}'s black-box, runtime inference approach. \textit{R-Bot} requires executing an LLM during query compilation, introducing high inference latency and non-determinism. Furthermore, the LLM is susceptible to hallucinations that cause catastrophic regressions (e.g., \textit{R-Bot} degrades DSB \texttt{query100} by 19.6$\times$). 

[mention Rbot uses cost estimation]
- 2.57
- 4.05
- 3.00

\textbf{Query latency.} Our best evolved policy outperforms the baselines across both benchmarks (Table~\ref{tab:query-rewrite-latency}). Our policy achieves significantly higher optimization coverage by discovering complex rule combinations that runtime heuristics miss. Our evolved policy is 2.57$\times$ faster on TPC-H and 4.05$\times$ on DSB compared to R-Bot. 
This is largely because our evaluation outer loop rigorously measures the actual execution latency of various rule combinations to generate a ground-truth dataset for policy evolution while R-Bot uses PostgreSQL's cost estimator during runtime Relying on cost estimates can mislead optimization, resulting in performance regressions (e.g., R-Bot's cost estimator predicted a specific rewrite would improve performance for DSB \texttt{query100}, but it actually degraded by 19.6$\times$). [make paragraph flow better, tie points that relate to each other and make more concise WITHOUT CUTTING CONTENT, make read well]
For instance, the evolved policy discovers performant transformations for queries that previously took over 300s, accelerating TPC-H \texttt{query22} down to 7.3s and DSB \texttt{query054} down to 0.25s. \textit{R-Bot} fails to optimize these queries because it lacks the empirical feedback required to safely navigate the massive search space.

This is largely because our evaluation outer loop rigorously measures latency of various rule combinations to generate a ground-truth dataset for policy evolution while R-Bot uses cost estimation to [fill in... and add example: cost estimator predicted a rewrite was better but actually led to DSB \texttt{query100} by 19.6$\times$).] at runtime. 

Moreover, \textit{R-Bot} is susceptible to LLM hallucinations at runtime, which can cause regressions 

Our policy outperforms R-Bot because our evaluation outer loop rigorously measures the execution latency of various rule combinations to generate a ground-truth dataset for policy evolution. This empirical feedback allows the policy to safely navigate  the massive search space, achieving significantly higher optimization coverage by discovering complex rule combinations that runtime heuristics miss. 

For instance, the evolved policy discovers performant transformations for queries that previously took over 300s, accelerating TPC-H \texttt{query22} down to 7.3s and DSB \texttt{query054} down to 0.25s. In contrast, \textit{R-Bot} fails to optimize these queries since it lacks this data and instead uses PostgreSQL's cost estimator during runtime. Relying on cost estimates can mislead optimization and result in performance regressions (e.g., R-Bot's cost estimator predicted a specific rewrite would improve performance for DSB \texttt{query100}, but it actually degraded execution by 19.6$\times$).

Our best evolved policy achieves the lowest overall latency (rewrite latency plus execution latency) compared to the baselines (Figure~\ref{}), demonstrating the advantages of our white-box approach. Our policy executes as Java code, ensuring sub-millisecond overhead for rule selection. [meention advantages of white-box approach again: ADRS yields solutions that are debuggable, deployable, and free of runtime inference overheads.] As such, we are [X times] faster on TPC-H and [X times] faster on DSB compared to PostgreSQL and [X times] faster on TPC-H and [X times] faster on DSB compared to R-Bot. This is because R-Bot invokes LLMs during runtime, incurring high inference overhead, [add in: to spend an average of over one minute per query performing RAG evidence retrieval and iterative LLM inference calls to select a rule sequence] leading to X slower for GPT-4o and Y slower for GPT-5. For most queries, this rewrite latency [make read better] negates any execution speedups. Furthermore, R-Bot is susceptible to LLM hallucinations [add: analyzing a query only to hallucinate a sub-optimal or invalid rule sequence, resulting in wasted rewrite time]

the runtime LLM inference utilized by \textit{R-Bot} is non-deterministic. The system frequently spends minutes analyzing a query only to hallucinate a sub-optimal or invalid rule sequence, resulting in wasted rewrite time and degraded execution time. 

By relying on precise, statically compiled feature guards generated during offline evolution, our white-box policy prevents the erratic behavior associated with runtime LLM calls, guaranteeing reliable end-to-end performance.

, ensuring that query execution improvements immediately translate into net overall latency reductions. 

The reasons for this are three-fold. First, as discussed previously, the evolved policy consistently finds superior query plans that execute faster than those discovered by \textit{R-Bot}'s runtime heuristics. Second, \textit{R-Bot} incurs runtime inference overhead. Relying on a black-box approach requires \textit{R-Bot} to spend an average of over one minute per query performing RAG evidence retrieval and iterative LLM inference calls to select a rule sequence. For the vast majority of operational queries, this rewrite latency negates any execution speedups. In contrast, 
Third, the runtime LLM inference utilized by \textit{R-Bot} is non-deterministic. The system frequently spends minutes analyzing a query only to hallucinate a sub-optimal or invalid rule sequence, resulting in wasted rewrite time and degraded execution time. By relying on precise, statically compiled feature guards generated during offline evolution, our white-box policy prevents the erratic behavior associated with runtime LLM calls, guaranteeing reliable end-to-end performance.

\lma{missing results.}

\xs{nit: there's some ambiguity when you just say ``optimization'' since in intro/S2 we talk about ``optimizing the Evaluator/evaluation framework'', but here it's actually the OG problem's optimization goal you're referring to.}

our white-box approach avoids limitations inherent to \textit{R-Bot}'s black-box, runtime inference approach. \textit{R-Bot} requires executing an LLM during query compilation, introducing high inference latency and non-determinism. Furthermore, the LLM is susceptible to hallucinations that cause catastrophic regressions (e.g., \textit{R-Bot} degrades DSB \texttt{query100} by 19.6$\times$). 

While effective for standard queries, it struggles with complex analytical workloads requiring structural rewrites (e.g., subquery unnesting). \ak{Clarify this is another competing system, not an LLM system we're building} 

(Figure~\ref{fig:query-rewrite}) \lma{Missing figure.}

[cut redundnacy with text above] To address these evaluation overheads, we co-evolve the evaluation workload and search space with the rewrite policy. For this case study, the primary goal of the evaluation outer loop is to efficiently generate a ground truth dataset mapping specific query features to highly performant rule sets. This empirical data is needed to inform the generation of an optimized rewrite policy in the solution generation inner loop. Our evaluation pipeline uses AI to construct targeted experiments by automating workload selection (Technique 3) and search space pruning (Technique 4). 

by conditioning on exact query structure (e.g., early-exit safety guards that block known regressing structural patterns and explicitly excluding subqueries containing self-joins because standard transformations severely degrade performance on those structures)

Using the empirical datasets generated by our automated evaluation outer loop, the solution generation inner loop synthesizes improved query rewrite policies. 

we used a training set: each query template in the benchmarks has two variants with different literal values, and we restrict the evaluation outer loop to only test on the first variant of each template. We run five iterations of the outer loop to converge on the final policy. During each outer loop iteration, the system executes a highly targeted search plan, evaluating an average of 40-50 query subsets against less than 10 pruned rule combinations per query. [So the second variant of each template is used in the final evaluation? Also, we evolved a single policy per workload, and use that single policy on all the test queries in that workload, right? The train/test setup is not super clear from this description. add model used for both loops: Claude-sonnet-4.5]

\accheng{add model}


Database performance is notoriously difficult to simulate due to intricate component interactions (e.g., buffer eviction triggering storage I/O overheads). This complexity is one of the key challenges in applying ADRS to databases: full system evaluations are prohibitively expensive for iterative feedback, while lightweight simulators rely on proxy metrics that fail to capture critical trade-offs. To address this, we propose co-evolving the simulator alongside the policy.

% , not only due to complex component interactions (e.g., buffer manager vs. storage engine) but also the challenge of articulating precise performance goals. \accheng{good simulator is hard is main thread, can ignore the precise utility function, metrics point below is more important} Users often cannot define the precise utility function that balances competing metrics, such as throughput versus tail latency. These issues make applying ADRS to databases difficult: full system evaluations are often too slow and/or complex for iterative feedback, while lightweight simulators rely on proxy metrics that miss critical trade-offs.

% Our core insight on how to successfully evolve simulators is that ``more is more'': effective simulation requires calibration against more ground-truth baselines from the full system. 

% \lma{I think for each of the problems, we should define them more formally. I.e., what is the input, what is the output, and what is the optimization target? These problems have different variants in the literature. So defining them formally will be clearer. Also, I think we should discuss the actual evolved algorithm in the evaluation as well (maybe you already plan to do so). I feel like just saying we did this or that evolution and got some results is probably not enough. It's more interesting if the evolved algorithm brings some insight.} \accheng{two paragraphs: what is input, what is output, target}

\accheng{in each case study, what the evolution of evaluator means?

what is the optimization goal that we are evolving for?
high level optional but needs to be specific for each example
}


Performance remains a critical objective in database system research, but is becoming increasingly difficult to achieve. \lma{Maybe "Performance has long been a critical objective in database system research, yet delivering it is becoming increasingly difficult."} \ak{This is not obvious, perf relative to increasingly large datasets is lagging, but absolute perf is generally increasing} \lma{I actually agree! This is a bit of a nuanced argument, and we want to be a bit careful in phrasing it.} The growing complexity of modern workloads and hardware is quickly outpacing human research and engineering capacity. Traditionally, the design of high-performance database systems has relied on manual algorithm development. To overcome human bottlenecks, machine learning (ML) to automate performance optimization. \lma{$\leftarrow$ Sentence seems incomplete.} However, these methods largely treat the database as a black box, relying on data-intensive models either to tune existing knobs or to replace core components and perform inference at runtime. Consequently, these learned approaches remain difficult to deploy~\cite{microsoft-autotuning} due to high run-time inference overhead and unpredictable worst-case behavior.
\lma{Maybe cite this tutorial from Microsoft if you don't have a better citation: Autotuning Systems: Techniques, Challenges, and Opportunities.}

\lma{Maybe "engine" $\rightarrow$ "database"} 

10$\times$ faster code for Datadog\xs{any specifics of what code or component?}\ak{and is there a one-word workload specifier just to ground a bit more?}

\lma{Maybe cite your ARDS paper.} 

Given the widening gap between modern application demands and existing database capabilities, 

% \accheng{From the abstract and intro, I couldn't understand how you maintain correctness of the solutions. For example, what if they break transaction isolation? Or is this for tasks so narrowly contained in the code that you can't break stuff?
% 3) Co-evolving the eval is nice but how well does it correlate with performance in the full eval? You didn't have a lot of quantitative data on that in the intro.
% 4) Don’t only cite the ADRS paper as motivation, it's a single non peer reviewed preprint. Cite other work that did similar stuff, like AlohaEvolve and ShinkaEvolve and OpenEvolve, to show that this is a widely explored field. Maybe there are other program optimization things you can cite too.
% add insights to intro}

[too long, no transition before/after] We focus specifically on performance optimization problems in this paper, as candidate solutions can be more easily verified without altering the underlying semantics of the underlying core system. 

[From the abstract and intro, I couldn't understand how you maintain correctness of the solutions. For example, what if they break transaction isolation? Or is this for tasks so narrowly contained in the code that you can't break stuff? add soemthing like..We focus specifically on performance problems in this paper as their solutions tend to be easier to verify since they do not change the semantics of the system.]

\item We discuss the broader implications of the ADRS approach for database performance optimization. \accheng{not sure about third contribution} \lma{Yeah this does not seem to be a typical contribution. Instead, maybe talk about the specific co-evolution methods you developed as the second contribution, and remove this one.} \ak{+1}

\ak{legacy?} 


These techniques treat the system as a black box, primarily centered around two approaches: (i) tuning database configurations, including knobs~\cite{Duan2009iTuned,VanAken2017OtterTune,Zhang2022OnlineTune} and physical design (e.g., indexes~\cite{Chatterjee2022Cosine,Kraska2019SageDB,Yu2024BRAD,Ding2021MTO}) and (ii) replacing specific components (e.g., query optimizers~\cite{Marcus2019Neo,Marcus2021Bao,Yang2022Balsa}) with learned models (e.g., DNNs~\cite{Kipf2019MSCN,Yang2019Naru,Hilprecht2020DeepDB} and more recently, LLMs~\cite{Trummer2022DBBERT,Lao2024GPTuner}). 
\lma{$\leftarrow$ The citations here seem to be a bit mixed up. How about this: These techniques treat the system as a black box, primarily centered around two approaches: (i) tuning database configurations, including knobs~\cite{kanellis2022llamatune,VanAken2017OtterTune,Zhang2022OnlineTune} and physical design (e.g., indexes)~\cite{Chatterjee2022Cosine,Kraska2019SageDB,Yu2024BRAD,Ding2021MTO,ding2019ai}) with surrogate models and more recently, LLMs~\cite{Trummer2022DBBERT,Lao2024GPTuner,Giannakouris2025LambdaTune}), and (ii) replacing specific database components (e.g., indexes~\cite{Kraska2018LearnedIndex,Ding2020ALEX,Ferragina2020PGMIndex}, query optimizers~\cite{Marcus2019Neo,Marcus2021Bao,Yang2022Balsa}), and cardinality estimators~\cite{Kipf2019MSCN,Yang2019Naru,Hilprecht2020DeepDB}) with learned models.}

Historically, spending hours or days to evaluate a single human-designed algorithm was acceptable. However, LLMs can now generate hundreds of novel ideas in minutes, shifting the bottleneck to the evaluation phase. For example, directly applying an existing ADRS framework to optimize PostgreSQL's buffer replacement policy would require modifying C source code, recompiling the engine (~3 mins), loading data for standard benchmarks (e.g., ~30 mins for TPC-H SF=10), and executing the full workload (e.g., ~30 mins). With a single iteration taking over an hour, running many iterations for ADRS convergence could take days to weeks. Furthermore, evaluation can be costly due to the massive search space inherent to many database performance problems. For instance, identifying the optimal set of query rewrite rules is a combinatorial problem~\cite{Sun2025RBot}. Naively applying ADRS to vast problem spaces renders the framework ineffective, as it wastes resources (e.g., evaluating many ineffective rule combinations). We need a way to achieve sufficient coverage without a prohibitively expensive evaluation budget.

\lma{I added some citations here. Feel free to take or replace them. You can probably use some of them in your introduction as well.}

\accheng{@Harald, is minimizing storage an optimization goal? or just constraint?} \hng{it's typically defined as a constraint.}

Our optimization target is to evolve a policy $\pi$ that optimizes for three critical metrics: (1) query latency, which should be minimized to deliver user-facing performance improvements, (2) algorithm runtime, which ensures the advisor can quickly recommend indexes in dynamic environments in which workloads frequently shift, and (3) storage footprint, which guarantees the memory budget $B$ is utilized efficiently. 

By systematically investigating where these gaps originate, such as physical hardware realities ignored by the cost estimator or non-deterministic measurement noise, the evaluation outer loop iteratively refines how to evaluate performance for the solution generation inner loop.

% \setlength{\belowcaptionskip}{-5pt}
\begin{figure}[t!]
  \centering
  % \vspace{-0.3em}
  % \vspace{-1.3em}
  \includegraphics[width=0.48\textwidth]{figures/placeholder-1.pdf}
  % \vspace{-1.8em}
  \caption{Cache hit rates.\ak{This is titled TAOBench but the text says TPC-H?}}
   \label{fig:buffer-1}
  % \vspace{-0.3em}
  \vspace{0.9em}
\end{figure}

Accordingly, our automated evaluation pipeline constructs targeted on the full system...

For TPC-H, the original paper shows the largest hit rate differences for 16 parallel streams at 16GiB for TPC-H, so we present results for this setting. We see that our best evolved policy achieves up to 19.8\% higher hit rate, which translates into 11.4\% I/O volume savings. While PBM-Sampling has higher runtime compared to CLOCK, our best evolved policy has similar runtime while realizing the I/O benefits. These results demonstrate that ADRS can discover robust solutions that work well on a range of different workloads.

\accheng{how do we discuss correctness?}
\accheng{just say current limitation, we do testing, traces, performance part discuss at end}
\accheng{just say we implement in postgres and recompile for the best policy}

\accheng{in each case study, what the evolution of evaluator means?

what is the optimization goal that we are evolving for?
high level optional but needs to be specific for each example
}

To determine the right metric for evolution, we co-evolve the performance model alongside the policy itself. For this case study, the primary goal of the evaluation outer loop is to efficiently determine a reliable performance metric for evolution so that generated solutions outperform on query latency and selection time on the full system. 
To automate Technique 2, the evaluation outer loop constructs a performance model to bridge the gap between estimated cost and the actual performance metrics we want to optimize. To achieve this, the LLM dynamically curates the fitness function by analyzing the correlation between proxy metrics and true execution performance. [add our mind the gap insight] The loop applies this insight in practice: the AI proposes different combinations of evaluation metrics (e.g., only optimizer cost estimates, a weighted combination of cost and latency, latency penalized by storage footprint and runtime, etc.) for the inner loop to use during policy evolution. The outer loop then validates the resulting policies by measuring their actual runtime performance. Through this co-evolution process, we empirically discovered that optimizing solely for latency, once measurement noise is controlled (described below) acts as a sufficient proxy for overall system performance, eliminating the need for complex, multi-metric objective functions that risk confounding the evolutionary signal.

This systematic process was repeated multiple times, reducing measurement noise to provide the inner loop with a stable fitness signal.

Evaluating policies via query latency introduces the challenge of measurement noise. While calculating cost estimation is deterministic, execution latency is variable, and managing non-deterministic evaluators is a known challenge for ADRS frameworks~\cite{let-the-barbarians-in}. To establish a reliable fitness signal, the evaluation outer loop initially experimented with standard statistical denoising techniques, such as taking the average or median across multiple workload executions. These approaches proved insufficient: the measured variance between identical runs was often larger than the actual latency differences between baseline algorithms. By analyzing execution traces, the outer loop identified that this noise stemmed from unstable database states, including volatile buffer cache contents, pages being overwritten by competing queries, and interference from background processes like snapshotting. To mitigate these artifacts, the outer loop iteratively designed an ordered measurement protocol. Instead of executing the entire benchmark at once (which allows competing queries to thrash the cache), the framework warms up each query and measures it in isolation, maintaining the same execution order across all evaluations. 

The final performance model is a rigorous execution pipeline that uses query latency derived from isolated warmup and benchmarking runs as the proxy for end-to-end performance. The solution-generation inner loop uses this to discover novel index-selection policies. By exposing the full system's physical characteristics via this model, the inner loop discovers non-obvious heuristics that contradict standard cost-based logic. For example, it learns to penalize indexes used for broad range queries (such as date ranges) on large tables, which the cost estimator inaccurately favors despite their high execution overhead because it overestimates the selectivity of range predicates and underestimates the resulting I/O overhead. The best optimized index selection policy, described in the next section, performs well on the end-to-end metrics we care about: query latency and selection time.

We only run evolution on TPC-DS~\cite{tpcds} to avoid overfitting and run the final evaluation pm both TPC-DS and TPC-H~\cite{tpch}, confirming that our erformance gains successfully generalize to TPC-H.

queries, leaving 
Although TPC-DS served as the holdout set during evolution, our results confirm that the performance gains successfully generalize to TPC-H.
\hng{@Audrey, pls reformulate if needed. We evolved on TPC-DS but evaluated and got gains on TPC-H}. 

\hng{@Audrey, double-check: clarified what is novel}

%The best evolved index selection policy includes several key algorithmic innovations: (1) cost memoization in which the policy caches the optimizer’s estimated workload cost for each candidate index set. Each set is evaluated at most once by simulating those indexes (e.g., via hypothetical-index support) and querying the planner, which speeds up selection and improves search quality; (2) pre-scoring by benefit/size that ranks candidates by efficiency and drives score-ordered greedy search with real-cost validation; (3) table-importance weighting that boosts dimension-style tables the planner tends to undervalue; and (4) search-space reduction via prefix pruning, top-K seeding, and bounded extension so compute focuses on promising candidates. 

the drop in theoretical cost is immaterial because actual runtime is the definitive measure of performance.[just note this, cost reduction doesn't actually matter] while trading roughly 9 percentage points of cost reduction.

Tese results demonstrate two key takeaways: first, the AI-discovered policy successfully optimize highly complex database schemas; second, an algorithm's ability to minimize theoretical cost estimates is a highly unreliable predictor of actual query execution speed.

[make more understandable] These results show that the learned heuristics transfer to a complex decision-support schema and that cost-reduction rank order is poorly correlated with latency rank order.

\subsubsection{Postgres Experimental Setup.} We implement the best evolved index selection policy on PostgreSQL 14.0. We run experiments on EC2 c5.14xlarge instances with 56 vCPUs, 112 GiB of RAM, and 500GB NVMe SSD. We use Benchbase~\cite{difallah2013benchbase} as our workload generator. Our experiments measure query latency, optimizer cost reduction, and storage utilization. %Latency is measured as the total execution time for the workload after a warm-up run.
Latency is the total (frequency-weighted) execution time of the workload. For each query, we perform one warm-up run followed by benchmark run(s), in interleaved order to limit cache interference.
Each data point plotted is the average over three independent runs, with error bars representing 95\% confidence intervals around the means.
We compare the performance of our best evolved policy against standard baselines (AutoAdmin, Anytime, DB2Advis, and Extend) on two benchmarks: TPC-H and TPC-DS. To keep runtimes manageable, we exclude Q19-Q22 in TPC-H and Q0, Q5, Q56, and Q63 in TPC-DS, which are long-running with minimal index benefit.
We run all benchmarks with a 500MB index storage budget.


\textbf{TPC-DS.}
We evaluate robustness on TPC-DS. The evolved policy achieved the best latency, 6.3\% faster than \texttt{extend} (37,275 s vs 39,791 s), while trading roughly 9 percentage points of cost reduction. Within the same class of iterative-search algorithms (\texttt{extend}, \texttt{autoadmin}, \texttt{anytime}), the evolved policy also has the fastest selection time, 7.5$\times$ faster than the baselines. \texttt{db2advis} is faster but uses a utilization-based one-pass strategy rather than an iterative search, and achieves the worst actual latency among the baselines. These results show that the learned heuristics transfer to a complex decision-support schema and that cost-reduction rank order is poorly correlated with latency rank order.

\textbf{TPC-H.}
For TPC-H, standard cost-based advisors often fail to optimize for actual runtime. The baseline \texttt{db2advis} algorithm achieved 49.7\% reduction in estimated cost but had the worst actual latency among baselines, 7.8\% slower than the \texttt{extend} baseline. This discrepancy arises because the optimizer overestimates the benefit of indexes on high-fan-out dimension tables (e.g., date ranges) while underestimating overhead under cached execution. In contrast, our best evolved policy achieved a 5.8\% reduction in actual latency compared to the best cost-oriented baseline (\texttt{extend}) and the fastest selection time, improving by over 2.2$\times$. It accomplished this by learning to reweight benefit-per-size, prioritize query-cost-weighted candidates, and apply table-importance boosts that correct for the planner's cost--latency gap.


% To automate policy discovery efficiently, we use OpenEvolve to discover an optimized index selection algorithm. 
% This process relies on our core insight: optimizer cost estimates are an insufficient proxy for execution time. We iterate through multiple evolution cycles, discovering that without access to ground-truth latency data, the generator produced policies that optimized for theoretical cost reductions that failed to materialize in practice. Access to execution time guided the AI to penalize specific column types (e.g., date columns) and prioritize others (e.g., join keys), enabling the discovery of policies that improve actual performance.

% \textbf{Naive optimization: the cost metric illusion.}
% We initially prompted Cursor to minimize the PostgreSQL optimizer's total cost estimate. Early versions successfully reduced cost by over 40\%. However, this theoretical improvement trapped the policy evolution in local optima. The optimizer's cost model relies on static statistics and assumptions that frequently diverge from runtime behavior. For example, the baseline \texttt{db2advis} algorithm achieved a 29.5\% cost reduction but degraded actual latency by 10.7\%. This misalignment occurs since the optimizer overestimates the selectivity of certain predicates (e.g., date ranges on fact tables) while underestimating the overhead of index maintenance and I/O. Consequently, the simulator encouraged the selection of indexes that looked good on paper but performed poorly on disk.

% \textbf{Ground truth: evolving for the right metric.}
% Providing access to actual execution latency was crucial towards evolving an effective policy. We calibrated the objective function to prioritize runtime performance over cost estimates. This shift required a rigorous evaluation protocol: we implemented cache warmups and forced \texttt{ANALYZE} calls to ensure consistent measurements. This calibration guided the AI to discover non-obvious heuristics that contradict standard cost-based logic. Specifically, the evolved policy learned to penalize date column indexes on large fact tables, which the optimizer favors, and prioritize small dimension table indexes that facilitate merge joins. This demonstrates our ``ground truth'' insight: by exposing the full system's latency characteristics, the AI learned to model performance trade-offs that the internal cost model missed.

% \begin{figure}[t!]
% \centering
% \vspace{-0.7em}
% \includegraphics[width=0.48\textwidth]{figures/latency_gap.pdf}
% %\vspace{-1.2em}
% \caption{We evolve policies using ground-truth latency to bridge the gap between optimizer estimates and real performance.}
% \vspace{-0.5em}
% \label{fig:latency-gap}
% \end{figure}

% \textbf{Latency-driven evolution.} This case study demonstrates the need for high-fidelity feedback loops. Specifically, we apply the following workflow to bridge the gap between estimated cost and actual latency:
% \begin{enumerate}
% \item Generate a candidate policy using the baseline logic (e.g., greedy expansion).
% \item Evaluate the policy by creating selected indexes on the live database.
% \item Measure actual query latency after cache warmup, discarding the optimizer's cost estimate.
% \item Feed the latency delta back to the LLM to refine the selection heuristics.
% \end{enumerate}
% We note that this approach incurs higher evaluation overhead than cost-based search. However, it is necessary to escape the local optima imposed by the optimizer's inaccuracies. The final evolved policy achieved a 21.2\% latency reduction, validating that true performance gains require optimizing for the physical reality of the database rather than its logical model.

% \subsection{Evaluation}
% In this section, we describe the results of our best evolved index selection policy. We use OpenEvolve to discover selection algorithms that optimize for query latency rather than estimated cost.
% \subsubsection{ADRS Experimental Setup.} We use OpenEvolve~\cite{} as our ADRS framework. We evaluate candidate policies on the TPC-H and TPC-DS benchmarks. The evaluator reports actual query latency after cache warmup and checks for validity (policies that exceed storage budgets or fail to select valid indexes are filtered). We use GPT-4o and run 100 iterations. The search completes in approximately eight hours and costs less than \$30.

% \textbf{Best evolved policy.}
% %The best evolved policy includes several key algorithmic innovations: (1) latency-aware prioritization that penalizes columns with poor cost-latency correlation (e.g., date ranges on fact tables), (2) join-key boosting that prioritizes indexes facilitating merge joins, (3) dimension table focus that adds low-overhead indexes on small tables (e.g., region, nation) often ignored by cost-based advisors, and (4) balanced budget allocation that prevents over-indexing large tables at the expense of broader query coverage. The evolution also revealed a fundamental trade-off: policies optimized solely for optimizer cost reduction (like the baseline \texttt{db2advis}) degraded actual latency by 10.7\%, whereas our balanced policy achieved a 21.2\% latency improvement by sacrificing theoretical cost gains for practical performance.
% The best evolved policy includes several key algorithmic innovations: (1) cost memoization — the policy caches the optimizer’s estimated workload cost for each candidate index set. Each set is evaluated at most once by simulating those indexes (e.g., via hypothetical-index support) and querying the planner, which speeds up selection and improves search quality; (2) pre-scoring by benefit/size that ranks candidates by efficiency and drives score-ordered greedy search with real-cost validation; (3) table-importance weighting that boosts dimension-style tables the planner tends to undervalue; and (4) search-space reduction via prefix pruning, top-K seeding, and bounded extension so compute focuses on promising candidates. Our evolved algorithm reduces actual latency by 6.3\% on TPC-DS and 5.8\% on TPC-H compared to the best baseline, while achieving 53\% lower selection time on TPC-H (3.4 s vs 7.3 s) and doing so within the same memory budget as the baselines.
% %The evolution also revealed a fundamental trade-off: policies optimized solely for optimizer cost reduction (e.g., baseline extend with 49.9\% cost reduction) achieved only 4th-best latency, whereas the evolved v3 policy achieved a 6.3\% latency improvement on TPC-DS and 5.8\% on TPC-H by trading cost reduction for measured workload performance.

\textbf{TPC-H.} [need topic setence: As shown in Figure~\ref{fig:index-selection-eval},... ]
For TPC-H, standard cost-based advisors often fail to optimize for actual runtime. The baseline DB2Advis algorithm achieves a 49.7\% reduction in estimated cost but has the worst actual latency among baselines, executing 7.8\% slower than the Extend baseline. This discrepancy arises because the optimizer overestimates the benefit of indexes on high-fan-out dimension tables (e.g., date ranges) while underestimating overhead under cached execution. In contrast, our best evolved policy achieves a 5.8\% reduction in latency and the fastest selection time, improving by over 2.2$\times$, compared to the best baseline (Extend). [these wins result from...reframe] It accomplishes this by learning to reweight benefit-per-size, prioritize query-cost-weighted candidates, and apply table-importance boosts that correct for the planner's cost--latency gap.

\accheng{title confusing compared to S3}
\lma{yeah "automating" seems a bit awkward here. "co-evolving"?}

Since different evaluation techniques apply to different problems, we illustrate how we use AI to design efficient evaluations by considering three ``classic'' database problems to cover all evaluator axes. 
[make more concise and clear, add the key insight of each from context provided]
For the system axis, we co-evolve the \textit{simulator} alongside the buffer cache policy to automatically discover an algorithm that outperforms the state-of-the-art. Also for the system axis, we co-evolve our \textit{model of end-to-end behavior} to discover a new index selection algorithm that enables both better cost estimation and latency (30\% improvement) compared to existing methods. To address the workload and search space axes, we co-evolve the \textit{subset of workloads and search techniques} to generate a novel query rewrite policy that results in [2.0$\times$] lower latency and runs in over four orders of magnitude faster (<200ms vs. 80 minutes) than the state-of-the-art approach, which makes LLM calls per query. Beyond performance, these results highlight the practical advantage of evolving white-box code: the discovered solutions are interpretable, predictable, and deployable without specialized inference infrastructure.
[Co-evolving the eval is nice but how well does it correlate with performance in the full eval? You didn't have a lot of quantitative data on that in the intro.]

As the complexity of modern workloads and hardware rapidly outpaces human engineering capacity, [doesn't connect, need to mention the problem/challenge] a new class of techniques, termed AI-Driven Research for Systems (ADRS), uses large language models to automate solution discovery. This approach shifts optimization from manual system design to automated code generation. Despite the potential of ADRS, the primary bottleneck in applying this approach is the evaluation pipeline. Since these frameworks rapidly generate hundreds of candidates without human supervision, they depend entirely on fast, accurate feedback to avoid optimizing blindly. Building such evaluators is espeically difficult for complex, stateful database systems. To enable the practical application of ADRS in this domain, we propose automating the design of evaluators by co-evolving them with the solutions. We demonstrate the effectiveness of this approach through three case studies optimizing buffer management, query rewriting, and index selection. Our automated evaluation frameworks enable the discovery of novel algorithms that outperform state-of-the-art baselines (e.g., a deterministic query rewrite policy that achieves up to 6.8$\times$ faster execution). 
proving that automating the evaluation bottleneck [reframe: unlocks the potential for...] highly optimized, deployable code for next-generation data systems.

A new class of techniques, termed AI-Driven Research for Systems (ADRS), uses large language models to automate solution discovery and is [sounds awk] poised to shift the researcher's role from manual system design. [add something about outpacing modern wrokloads etc] The primary bottleneck in applying ADRS is the evaluation pipeline. These frameworks depend on fast, accurate feedback from evaluators to converge on effective solutions. However, building such evaluators is difficult, especially for complex database systems. To enable the practical application of ADRS in this domain, we propose a methodology to automate the design of the evaluation pipeline itself. We demonstrate the effectiveness of this approach through three case studies: buffer management, query rewriting, and index selection. Across all three problems, our automated evaluation frameworks enable discovery of novel algorithms that outperform state-of-the-art baselines, such as a 6.8$\times$ faster execution with a deterministic query rewrite policy.

[better transition] Despite the potential of ADRS, the primary bottleneck in applying this approach is the evaluation pipeline. 
